Zenix: Efficient Execution of Bulky Serverless Applications

Serverless computing, commonly offered as Function-as-a-Service, was initially designed for small, lean applications. However, there has been an increasing desire to run larger, more complex applications (what we call bulky applications) in a serverless manner. Existing strategies for enabling such applications are to either increase function sizes or to rewrite applications as DAGs of functions. These approaches cause significant resource wastage, manual efforts, and/or performance overhead. We argue that the root cause of these issues is today's function-centric serverless model, where a function is the resource allocation and scaling unit. We propose a new, resource-centric serverless-computing model for executing bulky applications in a resource- and performance-efficient way, and we build the Zenix serverless platform following this model. Our results show that Zenix reduces resource consumption by up to 90% compared to today's function-centric serverless systems, while improving performance by up to 64%.

==> Figures/fig-launch.tex <==
{
\begin{figure}[th]
%\begin{center}
%\centerline{
\includegraphics[width=1.05\columnwidth]{Figures/Launch.pdf}
%}
\vspace{-0.3in}
\mycaption{fig-launch}{\sys\ Startup Flow with Real Results.}
{
This example application has two compute elements and one memory element, which is shared by the compute elements.
\sys\ first uses the global (30\ms) and the rack-level (89\ms) scheduler to schedule the first compute and the memory elements.
They then start their own launch process in parallel.
At a later time, \sys\ pre-start the environment for the second compute element.
}
%\end{center}
\vspace{-0.1in}
\end{figure}


==> Makefile <==
ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))
PREFIX=c:\\cygwin\\home\\$(USER)\\grants\\2007-cpa-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac
ALL =  pdf
endif

all: $(ALL)

PDF_TARGETS =main.pdf #zhang-bio.pdf facilities.pdf budget.pdf summary.pdf data-management.pdf zhang-collab.pdf

TEX_STUFF=$(wildcard *.tex) $(wildcard *.sty) $(wildcard *.cls) $(wildcard Figures/*.pdf) $(wildcard Graphs/*.pdf)

.PRECIOUS: .bbl .aux 

pdf: $(PDF_TARGETS)

# pdf: graphs
# 	rm -rf cpa.pdf
# 	pdflatex cpa
# 	bibtex cpa || true
# 	for i in bu?.aux; do bibtex $${i##.aux}; done
# 	pdflatex cpa
# 	pdflatex cpa

GRAPHS=

graphs: $(GRAPHS)

Graphs/%.pdf: Graphs/%.gnuplot.in
	cd Graphs; gnuplot < $*.gnuplot.in

%.aux : %.tex $(TEX_STUFF) 
	pdflatex $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl $(GRAPHS) $(FIGURES)
	pdflatex $*
	pdflatex $*
	pdflatex $*

test_build:
	rm -rf _test_build
	mkdir _test_build
	(cd _test_build; \
	 cvs checkout $$(cat ../CVS/Repository);\
	 cd $$(cat ../CVS/Repository);\
	 make;\
	)	

splitfiles:  main.pdf
	cp main.pdf proposal.pdf
	pdflatex proposaldesc.tex
#	pdflatex proposalsummary.tex
	pdflatex proposalbio.tex
#	pdflatex proposalbiotaylor.tex
	pdflatex proposalrelated.tex
#	pdflatex proposalequipment.tex
#	pdflatex proposalmanagement.tex

#
# copies file to prevent write-after-read problems
# uses date as suffix.
#

zhang-bio.pdf :  zhang-bio.tex $(TEX_STUFF)
	rm -rf zhang-bio.pdf
	pdflatex zhang-bio
	bibtex zhang-bio || true
	for i in bu?.aux; do bibtex $${i##.aux}; done
	pdflatex zhang-bio
	pdflatex zhang-bio

zhang-collab.pdf :  zhang-collab.tex $(TEX_STUFF)
	rm -rf zhang-collab.pdf
	pdflatex zhang-collab
	bibtex zhang-collab || true
	for i in bu?.aux; do bibtex $${i##.aux}; done
	pdflatex zhang-collab
	pdflatex zhang-collab

show_nt: pdf
	- killall AcroRd32 
	cp main.pdf main_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)main_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out $(PDF_TARGETS)





==> design.tex <==
%\input{tbl-techniques-single-col}

\if 0
\section{\sys\ System Design}
\label{sec:design}

%, deferring implementation details to \S\ref{sec:impl}.

%\boldunderpara{Overall Architecture.}~~ 

%The rest of this section presents \sys' detailed system design. %: its scheduling system, runtime execution system, and component adjustment mechanisms. When introducing a design, we add in parenthesis what the design is mainly for. 

This section presents how \sys\ generates and executes resource graphs.
These include 1) an offline profiling system, 2) a customized compiler, 3) elastic memory component materialization, 4) elastic compute component materialization, % even when a (virtual) compute component grows its memory arbitrarily, 
5) scalable scheduling mechanism and performance-efficient scheduling policies, 6) a communication mechanism optimized for dynamically added components' communication, 7) adaptive ways to adjust resource graph, and 8) reliability mechanisms.

%\sys\ consists of three subsystems, a scheduling system, a runtime execution system, and a component adjustment system.
%The rest of this section will introduce each of them. % in the order that an application reaches it while executing.
\fi


\input{offline-v2}
\input{runtime}


==> failure.tex <==
\subsubsection{Reliability and Consistency}
\label{sec:failure}

\boldunderpara{Failure handling.}
Traditional FaaS-based serverless re-executes the entire function when failure happens. This works well when applications are small, but bulky applications can be time- and resource-consuming to re-execute. To avoid re-executing an entire bulky application after a failure, we send the result of every compute component to the rack-level scheduler via reliable messaging (\eg, Kafka~\cite{Kafka} in our implementation).
When a failure happens, \sys\ discards the crashed component and all data components it accesses.
\sys\ locates the latest cut of a resource graph where all the edges crossing the cut have been persistently recorded.
%, all other physical components belonging to the same virtual component, and all this virtual component's communicating components. 
\sys\ re-executes from this cut using the persistently recorded input messages. 

We apply the same failure-handling principle to data components. 
\sys\ does not make data components durable or replicate them, as they only store intermediate state~\cite{klimovic2018pocket}. If any memory region in a data component crashes, \sys\ discards all the compute components that access it and all other memory regions of the same data component. \sys\ then finds the latest reliable resource graph cut to restart.

Resuming from the reliably recorded messages in the above manner is sufficient to guarantee {\em at-least-once} semantics, which is the same as today's serverless systems~\cite{AF_reliable_event_processing_20,GCF_exec_guarantees_2022}. 
%If no restarted component modifies the external state, we can further guarantee {\em observably exactly-once} semantics.
Our failure handling design balances foreground performance and failure recovery performance compared to mechanisms that take more checkpoints~\cite{Burckhardt_2021} or those that restart the entire function chain after a failure~\cite{AWS-Step-Functions,OpenWhisk-composer}.

\boldunderpara{Consistency and synchronization}
Multiple compute components can access the same data component as shared memory. As a generic framework, \sys\ provides basic distributed synchronization primitives instead of a particular consistency scheme. Users can use the \sys\ synchronization primitives like distributed locks to enforce critical sections.
As \sys\ runs on generic RDMA or TCP network, all communication is through messaging, and we do not provide automatic coherence across components. New coherent media like CXL could potentially be used with \sys\ to provide hardware-level coherence, which we leave for future work.

==> fig-app.tex <==
{
\begin{figure*}[th]
\begin{minipage}{2in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/lr-45mb.pdf}}
%\vspace{-0.1in}
\mycaption{fig-app1-45mb}{Memory Consumption of Logistic Regression with 45\MB\ Input.}
{}
\end{center}
\end{minipage}
\begin{minipage}{0.14in}
\hspace{0.14in}
\end{minipage}
\begin{minipage}{2in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/lr-12mb.pdf}}
%\vspace{-0.1in}
\mycaption{fig-app1-12mb}{Memory Consumption of Logistic Regression with 12\MB\ Input.}
{}
\end{center}
\end{minipage}
\begin{minipage}{0.14in}
\hspace{0.14in}
\end{minipage}
\begin{minipage}{2.7in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/lr-peak.pdf}}
%\vspace{-0.1in}
\mycaption{fig-app1-peak}{Peak Memory of Logistic Regression with 12\MB\ Input.}
{}
\end{center}
\end{minipage}
\vspace{-0.15in}
\end{figure*}
}


==> fig-cluster-level.tex <==
\begin{figure}[t]
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/eval_cluster_memory.pdf}}
% \vspace{-0.15in}
\mycaption{fig:eval:cluster-mem}{Cluster Level Memory Utilization}
{
}
\end{center}
\end{minipage}
\hspace{0.005\columnwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/eval_cluster_cpu.pdf}}
% \vspace{-0.15in}
\mycaption{fig:eval:cluster-cpu}{Cluster Level CPU Utilization.}
{
}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\end{figure}


==> fig-code-example.tex <==

{
\begin{figure*}[]
\begin{center}
\centerline{\includegraphics[width=2\columnwidth]{Figures/fig-code-example.pdf}}
\end{center}
% \vspace{-0.2in}
%caption
\captionsetup{width=\textwidth}
\begin{minipage}{\columnwidth}
\begin{center}
\mycaption{fig-micro-swap}{\sys Code example}{}
\end{center}
\end{minipage}
\vspace{0.1in}
\end{figure*}
}

==> fig-example-stack.tex <==
{
\begin{figure*}[th]
%\begin{minipage}{0.54\textwidth}

\begin{minipage}{0.55\textwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-example.pdf}}
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/Figure-example.pdf}}
\vspace{-0.1in}
\mycaption{fig-example}{\sys\ Example.}
{
Example code of application programming with \sys
}
\end{center}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-flow-phyiscal.pdf}}
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/Figure-example.pdf}}
\vspace{-0.1in}
\mycaption{fig-example}{\sys\ Flow.}
{
}
\end{center}
\end{minipage}

% \vspace{-0.15in}

\end{figure*}
}


==> fig-example.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-example.pdf}}
% \centerline{\includegraphics[width=0.75\textwidth]{Figures/Figure-example.pdf}}
\vspace{-0.1in}
\mycaption{fig-example}{\sys\ Code Example}
{
An annotated user program compiled to the \sys internal interface. Data structure a is placed as a memory object and its lifetime is inferred to span over both compute objects.  
}
\vspace{-0.2in}
\end{center}
\end{figure}
}


==> fig-exp-extra-merged.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-4.pdf}}
\end{center}
%captions, 0.25*0.95=0.225
\captionsetup{width=0.225\textwidth}
% \begin{minipage}{\figWidthSix}
% \begin{center}
% \mycaption{fig-micro-warmstart}{Application Warm Start Overhead.}{}
% \end{center}
% \end{minipage}
\begin{minipage}{0.49\columnwidth} % locality
\begin{center}
\vspace{-0.6in}
\mycaption{fig-micro-locality}{Effect of \sys\ Locality Scheduling.}{}
\end{center}
\end{minipage}
\begin{minipage}{0.49\columnwidth} % 
\begin{center}
\vspace{-0.6in}
\mycaption{fig-micro-adjust}{Resource Adjustment.}{More top-right is better.}
\end{center}
\end{minipage}
\vspace{-0.3in}
\end{figure}
}


==> fig-exp-policy.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.97\columnwidth]{Figures/Figure-policy.pdf}}
% \centerline{\includegraphics[width=0.97\columnwidth]{Figures/Figure-policy-line.pdf}}
% \vspace{-0.1in}
\mycaption{fig-policy}{Timeline of Pool Utilization and Application Performance.}
{
Crosses represent aggregated execution. Dots represent disaggregated execution (App2s and App3s).
}
\end{center}
\vspace{-0.25in}
\end{figure}

==> fig-exp-scale-merged.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-micro1.pdf}}
% \centerline{\includegraphics[width=0.97\columnwidth]{Figures/Figure-policy-line.pdf}}
\vspace{-0.1in}
\end{center}
\vspace{-0.2in}
%caption
\captionsetup{width=0.225\textwidth}
\begin{minipage}{0.49\columnwidth}
\begin{center}
\mycaption{fig-micro-swap}{\sys Performance with Swap Component.}{}
\end{center}
\end{minipage}
\begin{minipage}{0.49\columnwidth}
\begin{center}
\mycaption{fig-micro-launch}{Effect of \sys\ Techniques on Run Time.}{}
\end{center}
\end{minipage}
\vspace{-0.1in}
\end{figure}

==> fig-exp12-merged.tex <==
{
\begin{figure*}[th]
\begin{minipage}{\textwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-1.pdf}}
\vspace{-0.2in}
\end{center}
\end{minipage}
%captions, 0.25*0.95=0.225
\captionsetup{width=0.225\textwidth}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-lr-resource}{Memory Consumption for LR with largest input dataset.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-lr-resource-12M}{Memory Consumption for LR with midsize input.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-lr-breakdown}{Execution Time Breakdown for LR.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-tpcds-resource}{Memory consumption of TPC-DS.}{}
\end{center}
\end{minipage}
% \begin{minipage}{\figWidthSix}
% \begin{center}
% \mycaption{fig-tpcds-time}{Execution Time of TPC-DS.}{}
% \end{center}
% \end{minipage}
% \vspace{-0.1in}
\end{figure*}
}


==> fig-exp346-merged.tex <==
{
\begin{figure*}[th]
\begin{minipage}{\textwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-2.pdf}}
\vspace{-0.15in}
\end{center}
\end{minipage}
%captions, 0.25*0.95=0.225
\captionsetup{width=0.225\textwidth}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-tpcds-time}{Execution Time of TPC-DS.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-tpcds-overhead}{Runtime Breakdown of Reduce-By Op.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix} % runtime
\begin{center}
\mycaption{fig-tpcds-memoryscale}{Memory Consumption when Scaling Input Size.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-tpcds-computescale}{Memory Usage (Log Scale) and Performance Speedup.}{}
\end{center}
\end{minipage}
% \begin{minipage}{\figWidthSix}
% \begin{center}
% \mycaption{fig-tpcds-computescale-resource}{Memory Consumption (Log Scale) when scaling compute cores.}{}
% \end{center}
% \end{minipage}
%\vspace{-0.05in}
\end{figure*}
}

==> fig-exp789-merged.tex <==

\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny{5.5}{6.5}}
\makeatother
{
\begin{figure*}[th]
\begin{minipage}{0.75\textwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-3.pdf}}
\vspace{-0.15in}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\notsotiny
\begin{tabular}{l | l }
\textbf{System Configurations} & \textbf{Time} \\
\hline
\hline
OpenWhisk & 773\ms \\
OpenWhisk + Overlay & 1188\ms \\
\sys + Overlay & 1002\ms \\
\sys no overlay & 595\ms \\
%\sys Prewarm Overlay & 556 \\
Full \sys (pre-warm) & 284\ms \\
AWS Lambda & 140\ms \\
AWS Step Functions & 215\ms \\
%Azure Durable Functions & 270\ms \\
\hline
%AWS Lambda & 140\ms \\
%AWS Step Functions & 215\ms \\
%Azure Durable Functions & 270\ms \\
AWS warm & 114\ms \\
OpenWhisk warm & 35\ms \\
\sys\ warm & 10\ms \\
\end{tabular}
\end{center}
\end{minipage}
%captions, 0.25*0.95=0.225
\captionsetup{width=0.225\textwidth}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-tpcds-computescale-resource}{Memory Consumption (log scale) When Scaling Compute Cores.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix}
\begin{center}
\mycaption{fig-micro-elastic}{Memory Elasticity.}{For three different input sizes. %Dashed lines for \sys\ include memory allocated on both memory components and compute components. 
}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix} % 
\begin{center}
\mycaption{fig-micro-launch}{Effect of \sys's Techniques on Run Time.}{}
\end{center}
\end{minipage}
\begin{minipage}{\figWidthSix} % cold
\begin{center}
{\captionsetup{font={stretch=0.85}}\beforecaption\captionof{table}{\label{fig-micro-coldstart}{\bf \footnotesize Cold and Warm Startup Time.}}\aftercaption}
\end{center}
\end{minipage}
% \vspace{-0.15in}
\end{figure*}
}



==> fig-lr-motivation.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.6\columnwidth]{Figures/Figure-LR-Motive.pdf}}
\vspace{-0.1in}
\mycaption{fig-lr-motivation}{Logistic Regression~\cite{carreira2019cirrus} Major Object Memory Consumption.}
{
Each color represents a major data object.
}
\end{center}
\vspace{-0.2in}
\end{figure}


==> fig-motivation-old.tex <==
\begin{figure}[t]
\label{fig-lr-motivation}
\begin{minipage}{\columnwidth}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/Figure-merge-0.pdf}}
\vspace{-0.1in}
% \mycaption{fig-motivation-exp}{Input-and-Function Dependent Memory Consumption Patterns.}
% {Two functions in video processing~\cite{copik2021sebs} have distinct features.}
\end{center}
\end{minipage}
%captions, 0.25*0.95=0.225
% \captionsetup{width=0.65\columnwidth}
\begin{minipage}{\columnwidth}
\begin{center}
\mycaption{fig-motivation-exp}{Memory Usage Examples.}
{(a) (b) are two stages in a video processing application~\cite{copik2021sebs} with three input videos. (c) shows memory consumption of major data structures in a Logistic Regression application~\cite{carreira2019cirrus}.}
\end{center}
\end{minipage}

% \begin{minipage}{0.33\columnwidth}
% \begin{center}
% \mycaption{fig-lr-motivation}{}
% {
% 
% }
% \end{center}
% \end{minipage}
%\vspace{-0.25in}
% \begin{minipage}{0.65\columnwidth}
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{Figures/video-processing-extract-gif.pdf}}
% \vspace{-0.05in}
% \mycaption{fig-motivation-exp}{Input-and-Function Dependent Memory Consumption Patterns.}
% {Two functions in video processing~\cite{copik2021sebs} have distinct features.}
% \end{center}
% \end{minipage}
% \begin{minipage}{0.34\columnwidth}
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{Figures/Figure-LR-Motive.pdf}}
% \vspace{-0.1in}
% \mycaption{fig-lr-motivation}{Logistic Regression~\cite{carreira2019cirrus} Memory Consumption.}
% {
% Each color represents a major data object.
% }
% \end{center}
% \end{minipage}
% \vspace{-0.2in}

\end{figure}

==> fig-runtime.tex <==
{
\begin{figure}[t]
\begin{center}
%\centerline{
\includegraphics[width=0.85\columnwidth]{Figures/Architecture.pdf}
%}
\vspace{-0.1in}
\mycaption{fig-arch}{\sys\ System Architecture.}
{ \zhiyuan{Hightlight? the memory/comptuation implementaion?}
}
\end{center}
%\vspace{-0.1in}
\end{figure}


==> fig-workflow.tex <==
{
\begin{figure*}[th]
%\begin{minipage}{0.54\textwidth}
\begin{center}
\centerline{\includegraphics[width=0.95\textwidth]{Figures/Workflow.pdf}}
%\vspace{-0.1in}
\mycaption{fig-workflow}{\sys\ Workflow.}
{
This example demonstrates the workflow of \sys. The user annotates her program with two remote and two split annotations. The \sys\ compiler then generates a graph of virtual components.
At the run time, \sys\ materializes {\em Mem1} as one physical memory component, {\em Mem2} as two physical memory components on two memory servers, two instances of {\em func3} and single instances of {\em func1} and {\em func2} on two compute servers.
%After this application is first triggered, \sys\ allocates computing resources for the elements in the compute pool and the memory pool.
At a later time, \sys\ could decide to aggregate {\em func1}, {\em func2}, and {\em Mem2} and run them on a balanced server. At yet another time, \sys\ could decide to re-disaggregate the components.
%After a few invocations, \sys\ finds an opporunity to merge the green and the blue compute elements with the mem1 element.
%It then runs these merged elements in a server in the balanced pool.
%Later on, if the balanced pool runs out of resources, \sys\ could pick these merged elements as the victim and disaggregate them again (the back arrow).
}
\end{center}
\vspace{-0.15in}
\end{figure*}


==> impl.tex <==
\section{Implementation}
\label{sec:impl}

We now briefly discuss our implementation of \sys. 
Currently, \sys supports programs written in Python, the most commonly used programming language in serverless~\cite{Datadog_2021}. 

\subsection{Profiling and Compiling}

\boldpara{Compiler support.}
Most of our implementation could be extended to other language including native languages. For Python, we also implement a specific optimization that could potentially apply to other non-native languages as well.
Specifically, when we place variables and data structures in remote memory, the Python runtime will need to serialize and deserialize the data before/after handing them to/from the network~\cite{skyway-asplos18,gerenuk-sosp19}. Serialization and deserialization have high performance overhead. To minimize this overhead, we develop various memory-optimized data structures (such as NumPy arrays, lists, maps, etc.) that build on native arrays. Such data structures are simple wrappers around native bytes and hence do not need the costly serialization/deserialization process.
%much more efficient to transfer than data structures in Python libraries. 

\subsection{Runtime Implementation}
We implemented \sys's runtime system on top of Apache OpenWhisk~\cite{OpenWhisk}.
In total, \sys\ includes $\mathtt{\sim}$15K SLOC: 8K lines of Scala to extend Openwhisk's scheduler and executor, and 4K lines of C together with 1.8K lines of Python for runtime and libraries.


\input{fig-app}

We reuse as many existing OpenWhisk infrastructure pieces as we can to reduce development cost, \eg, we reuse its CouchDB metadata store to store element code and profiling metrics, its Invoker code to launch containers, and its Kafka messaging system for dependent element communication. 
%We utilize the CouchDB instance to store element code, resource profiles, and other metadata. We re-use most of the Invoker code in order to launch function containers. 


Finally, a major change is the addition of our own library in the container runtimes. This library performs three tasks: 1) managing user-level swapping using Linux \ufd, 2) setting up and performing RDMA communication between co-running containers, and 3) handling \texttt{pull\_stat} calls by performing resource profiling. %All these three tasks are hidden from user applications.
%Included with the container runtimes in \sys is a special library which enables containers to communicate with one another. This library is implemented.... \zhiyuan{fill}





==> intro-2.tex <==
\section{Introduction}
\label{sec:intro}

Serverless computing, commonly offered in the form of FaaS (Function-as-a-Service), is a type of cloud service that allows users to deploy and execute their application programs (\ie, functions) without managing servers.
%(or more specifically, any software or hardware infrastructures beneath their applications).
%Initially introduced for cloud providers to exploit unused data-center resources, 
Serverless computing has quickly gained huge popularity in recent years because of its benefits to cloud users: minimal IT burdens 
%to focus on their core business products 
and paying for only when their applications are triggered.

%\hx{Shall the following paragraph focus on why ``memory'' disaggregation is needed? Also, I felt that this paragraph should appear before the previous paragraph. Talk about the reason first and then why existing techniques can't handle it.}
%We set out to first answer the research question of \textbf{\textit{why disaggregating resources for serverless computing?}}
Despite the many benefits, today's FaaS-based serverless computing still has several key limitations.
%and we believe that they are major reasons that prevent serverless computing from enabling a richer set of applications.
First, the amount of resources a function can use is limited.
%For example, AWS Lambda~\cite{XXX} limits each function to use at most 10\GB\ of memory and run for at most 15 minutes.
Resource limits forces users to rewrite their large-scale applications like data analytics as smaller pieces that are small enough to fit in a function
and/or to use an external service to host its extra resource need. \hx{force users to rewrite? or they just cannot run large-scale applications at all? We should probably better say ``resource limits prevent users from running large applications'' rather than "forcing them to rewrite". }
\yiying{Well, in theory, shouldn't every program could potentially be rewritten in a way that it's broken up into smaller pieces that could fit in a resource limit, and having intermediate data stored somewhere else?}
Second, there are only few fixed CPU-to-memory ratios that users can choose, but user workloads can have many different CPU and memory usages.
As a result, either some CPU or some memory resource is wasted~\cite{arxiv}.
Third, a function's resource amount is fixed across invocations, but different input to a function could result in different resource needs~\cite{arxiv}\zacb{For the third point, this doesn't really describe a limitation of serverless computing? It just describes a property of function invocations. What's the actual point trying to be made? It seems just like another consequence of limited function resources}.
This lack of elasticity would result in function failure in the worst case when some invocations exceed the preset per-function resource amount.
%, \eg, Google Cloud Functions offer six combinations of CPU frequency and memory sizes
Finally, all resources must be allocated and deallocated at the same time even if they exhibit different lifetimes.
On the one hand, a function needs to be provisioned with the peak resource use, but not the entire function needs to use the peak amount. 
As a result, either the cloud provider~\cite{azure_functions_pricing} or the user needs to pay for the unused resources~\cite{aws_lambda_pricing,google_functions_pricing}. %, because cloud providers cannot easily exploit the unused resources.
On the other hand, certain resources such as intermediate data cannot live beyond the execution of a function, 
which makes sharing them across functions harder~\cite{klimovic2018pocket,XXX}.
%Finally, as many recent works have demonstrated~\cite{Pocket,XXX}, it is hard to efficiently manage function intermediate data, or ``states'',
%and to efficiently share them across functions. 
%it even more likely to have unused resources.
%In addition, because 
%Together, these limitations prevents users from running 
%although FaaS billing has become more fine-grained in terms of time unit (\eg, AWS Lambda recently changed billing granularity to 1\ms), 
%Finally, user functions are limited to use only CPU and memory but not other types of resources such as GPU, 
%preventing more workloads like deep learning from migrating to serverless computing.

The root cause of these limitations is today's ``function-centric'' serverless model.
%A function is a fix-sized box defined by the cloud provider,
%and cloud users have to adapt their applications into these provider-defined functions, 
%usually with performance loss, increased cost, and developmental cost.
%We argue that a better serverless computing model should work towards user applications, not the other way round.
%
A function is a rigid, fix-sized box that couples CPU and memory resources and is allocated, scheduled, terminated, and billed as an inseparable unit.

To solve this fundamental problem, we propose a new serverless-computing model that is \textit{``resource-centric''}.
Our key idea is to disaggregate serverless applications into different units based on their \textit{resource features} and to schedule and execute these units independently in corresponding \textit{resource pools}.
%Resource disaggregation solves exactly this problem. 
Resource disaggregation enables the independent scaling of different resource types, thereby allowing arbitrary resource ratio (\eg, CPU-to-memory size ratio). 
When pooling resources together, applications can allocate as much resource as needed, essentially lifting today's FaaS function resource limits.

We are not the first to apply the resource disaggregation idea on serverless computing. In fact, today's FaaS-based serverless computing systems already sit on a disaggregated architecture, where a storage pool like AWS S3 is managed independently from the pool that executes serverless functions.
This separation is indeed what enables today's functions to be {\em autoscaled}: more/fewer functions are allocated as application loads change without the need to change the storage layer.
%Much of FaaS serverless computing's success is a result of its {\em autoscaling} feature: more/fewer functions are allocated as application loads change. This autoscaling feature is enabled by an increasingly popular data-center architecture: the disaggregation of storage and computational systems. This disaggregation allows the independent scaling and management of a storage system (\eg, AWS S3) from a computational service (\eg, AWS Lambda).

%A. Disaggregation are proved to bring benefits to non-serverless programs. B. In this case, it brings some benefits as well as some performance overheads. for example, it can enable larger programs but still have performance downgrade in some cases. C. When bringing disaggregation into serverless, we face the same tradeoff choices but a different set of capacities: auto-scaling, locality etc, which enables new design space exploration for us. D. we will explore how to apply the benefits of disaggregation onto serverless. Starting from a ideal model for disaggregation, but in real implementation we leverage existing serverless arch and do not reinvent the whole flow.  E. Elements can provide benefits of serverless (fine-grained scaling and locality) while (make a fine-grained elements) fit into the current serverless scheduling arch. F. Which should be enough to proof the disaggregation benefits and future improvements on the arch will solve some performance overhead.

This paper takes a step further by exploring the disaggregation of computation (processing) and memory in the serverless-computing setting, thereby enabling a fully disaggregated serverless computing paradigm. Resource disaggregation (memory disaggregation in particular) is an active research area that has attracted extensive academia works~\cite{Shan18-OSDI,semeru-osdi20,AIFM,fastswap,INFINISWAP,XXX} and initial industry adoption~\cite{FACEBOOK-BRYCECANYON,Ali-SinglesDay,XXX}. Existing resource disaggregation works apply to a non-serverless-computing setting. It is unclear how disaggregation could fit in to serverless computing, as serverless computing has stark difference from traditional computation model for its auto-scaling and event-triggering features.



%The next question that follows is \textbf{\textit{how resources should be disaggregated for serverless computing?}}
Existing resource disaggregation solutions separate an application only by its resource types, 
\eg, into a compute component, a memory component, and a storage component.
For serverless computing, disaggregating only by resource types is not enough, as doing so cannot solve the last limitation of today's serverless function mentioned above.
We propose to consider three dimensions when disaggregating serverless applications: resource type, resource amount, and resource lifetime.
The resource amount and lifetime dimensions allow us to solve the last limitation.
%Finally, after disaggregation, applications can decouple the lifetime of memory and computation. 
For example, a piece of intermediate data could live beyond the end of its producer when it is disaggregated, allowing other computation units to access it; if later on the application does not need this data anymore and uses a smaller data structure, disaggregating these two data pieces would reduce  memory consumption.
The resulting application can be represented by a graph of {\em element}s, each representing a piece of application code or data structure with a distinct triad, \textit{$<$resource type, resource amount, lifetime$>$}.
%For example, a CPU (compute) element runs in a CPU (compute) pool, and a memory element runs in a memory pool.
Edges in an element graph represent task flow and data flow. 
One element can trigger one or more elements with directed edges (\ie, task flow) and multiple elements running at the same time can communicate with each other with undirected edges (\ie, data flow). 
%With this model, we essentially turn serverless computing from \textit{``function centric''} to \textit{``resource centric''}.
%Multiple elements can be used to capture resource consumption changes in a user application.
%Separating an application based on resource amount allows fine-grained right sizing. 
%For example, if the initial phase of an application uses a huge data structure, the next phase uses only a few variables, and the last phase uses a median-sized data structure, we could use a huge memory element, no memory element, and a median-sized element for these phases while using a single compute element for the entire duration.
%In contrast, today's FaaS would use one function with huge memory for the entire duration.
%As a result, disaggregation reduces the total resource consumption and thus user costs.




%\textbf{\textit{How to efficiently support resource disaggregation?}}
Based on the abover model, we propose \textbf{\textit{\sys}}, a framework that efficiently executes user applications in a resource-disaggregated manner.
Users supply a graph of code pieces to \sys, each of which is a \textit{compute element} (\ie, an element of the resource type CPU).
\sys\ statically generates \textit{memory element}s from these code pieces either by our automatic compiler tool or by user explicit calling our memory-element interface. 
%, with an easy-to-use interface \sys\ provides (we discuss how users could potentially generate elements, with some of \sys's compiler support in \S\ref{XXX}).
At the run time, \sys\ schedules, autoscales, and executes element graphs in the unit of element.
Using resource-based elements instead of functions as the run-time unit raise many new challenges that today's serverless computing frameworks cannot solve.
We designed a \textit{disaggregation-native} run-time system that incorporates many technical innovations at different layers to solve these challenges.
%uses an element as the unit of scheduling, execution, and auto-scaling, and elements with different resource types run on different disaggregated resource pools. 

%\textbf{\textit{What are the new technical challenges?}}
%\sys\ innovates on several fronts to confront key technical challenges raised by disaggregating serverless functions. 
First, disaggregation inevitably introduces more inter-element communication. Such communication needs to sustain much higher load and achieve much lower latency than today's function-to-function communication.
For example, a compute element could frequently access a memory element and expect such accesses to be close to native memory performance.
We propose an RDMA-based, direct element-to-element communication mechanism.
On top of it, we build a library that transparently caches remote memory data locally and performs serialization and deserialization for languages like Python. 
Furthermore, we propose a locality-aware and resource-pool-aware scheduling system that schedules elements as close to each other as possible if they have high communication need.

Second, the startup time of elements could have a bigger impact on application performance when elements run shorter than typical traditional functions.
We propose a pre-warming scheme that warms up the execution environment for each element in an ``almost just-in-time'' manner.
Furthermore, we developed a mechanism to establish and manage RDMA connections without the need for a proxy network, as the latter significantly increases the startup time.
In addition, to efficiently launch and execute memory elements, we propose to use a single execution environment for all memory elements on a physical server and to isolate them into different RDMA protection domains.

Finally, an element should be elastic and auto-scaled.
We auto-scale memory elements by allocating more {\em physical} memory chunks for a memory element when its size grows.
The allocation and accessing of multiple memory chunks are all transparent to user applications, and different memory chunks can sit on different physical servers, thereby allowing user applications to use as large memory as they want.
We also transparently track the lifetime of elements and terminate them when their lifetime end.

%Finally, when disaggregating applications using three dimensions, the resulting element graphs could be huge and pressure the scalability of the scheduling system.
%We organize the scheduler itself as a two-level distributed system to make the scheduling more scalable.



%\textbf{\textit{When and how not to disaggregate?}}
Despite disaggregation's various benefits and our solutions to its technical challenges, certain performance loss is still inevitable when there are many elements that communicate with each other frequently.
To solve this problem, our idea is to merge, or \textbf{\textit{aggregate}}, elements.
Specifically, we transparently merge compute and memory elements that suffer from high communication performance overhead into one execution environment that run on a \textit{balanced pool}.
The balanced pool does not disaggregate different types of resources, and each server has both beefy CPU and ample memory.

To fully exploit the benefits of element aggregation while hiding its complexity from user applications, we developed new run-time and compiler support.
The run-time system transparently executes two elements in a single container and converts remote accesses to local ones, while the compiler merges multiple elements' code into one which is then executed as any other elements.

To decide when and what to aggregate/disaggregate, we design a policy based on the utilization of each resource pool, the performance overhead of element communication, and element resource utilization.
%merge same lifetime
We also developed a monitoring system to collect per-element run-time profiles.
We design our policy and monitoring to be simple and lightweight. 
As a tradeoff, at runtime, an element could use more resources than the prediction.
In worst case, an element can use more memory than what the server hosting it has.
To handle such cases, we developed a user-space swap system to transparently swap not-recently-used local memory to the remote memory pool.

We implemented \sys\ on top of OpenWhisk~\cite{OpenWhisk}.
%Currently, \sys\ only supports Python, but our approach could be easily extended to other languages.
We evaluated \sys\ with a set of microbenchmarks and three real-world applications: simple machine-learning training, distributed query with the TPC-DS benchmark, and video processing.
We compared \sys\ with vanilla OpenWhisk, AWS Lambda, AWS Step Functions~\cite{AWS-Step-Functions}, and PyWren~\cite{jonas2017occupy_pywren}.
Our real-workload evaluation results demonstrate that \sys\ could save memory of up to 1.96\X\ while improving performance by up to 28\% compared to existing systems.
In addition, \sys\ enables workloads that are larger than today's FaaS limits without any developer involvement.
We will make \sys\ publicly available upon the publication of this paper.
% Serverless computing is a new type of cloud service that has gained a lot of traction recently. The main idea of serverless computing is to free cloud users from managing servers so that they could focus on their core business logic. Because of this, more types of (non-IT) users could now enjoy cloud computing.

%Serverless computing is a recent computing paradigm introduced and now supported by most major public cloud providers. Serverless computing, as the name suggests, removes the need for cloud users to manage virtualized operating systems infrastructure. This allows companies to focus less on the infrastructure challenge of operating their services and more on the features that they provide to the users. Another positive consequence of serverless computing is more efficient billing and resource utilization. Instead of needing to allocate computing cores and memory which may go unused due to patterns in user activity \cite{liu2011measurement} serverless users are billed only when requests to applications are received and for the resources used while processing the request. One more benefit of serverless computing is the ability for cloud providers to have more efficient scheduling and placement policies of applications which can more effectively use the resources within the data center.

%As promising as the serverless paradigm may seem it is not without its drawbacks. There are a few main limitations which prevent more users from shifting their applications to serverless infrastructure. First is that current serverless offerings from cloud providers such as AWS, Google Cloud, and Microsoft Azure all limit serverless application functions to relatively small amounts of computing resources. Typically no more than a few cores and generally less than 15GiB of memory. These values are far less than what is available in traditional reserved virtual machine offerings. Second is that serverless functions are not designed for storing state between function invocations. They are supposed to be designed in a stateless way to offer easy horizontal scaling, but this places limits on the types of applications which may be converted to serverless workloads. Lastly, serverless functions are not designed to communicate directly between one another. This results in high communication latencies between chains of serverless functions that may make up larger processing pipelines.

%In this work we aim to solve the hardware resource limitation and communication latency issues of serverless computing by proposing a new end-to-end architecture for serverless functions to run on disaggregated hardware. This work presents the system and performs an in-depth performance analysis to show the feasibility of such an architecture and why serverless is a good fit for disaggregated platforms.

==> intro-3.tex <==
%\yiying{All, I have three versions of Intro. The most recent one is the current Section 1. The oldest version is Section 3. Let me know which version is better (or none of them is good) and/or how to improve.}

\section{Introduction}
\label{sec:intro}

\if 0
our target is to support larger applications in a serverless style and be resource-efficient. 

Novelty/contributions:

1. converting programs to resource graphs via profiling and compiling

2. dynamic materialization of components (based on history and status of execution, we decide whether or not to merge components (e.g., executing memory local vs. remote))

3. runtime control plane optimizations and scheduler
\fi




Serverless computing, commonly offered as Function-as-a-Service (FaaS), is a cloud service that allows users to deploy and execute their applications without managing servers.
%(or more specifically, any software or hardware infrastructures beneath their applications).
%Initially introduced for cloud providers to exploit unused data-center resources, 
% Serverless computing has gained significant popularity in recent years because of its benefits to cloud users: minimal IT burdens and paying only when their applications run.
Serverless computing's popularity stems from its benefits to cloud users, including minimal IT burdens and pay-per-use pricing.

Serverless computing was originally designed for running short, small-scale functions such as HTML serving, and its usage in public clouds has followed this pattern. For example, 50\% of functions running took less than 3 seconds to execute, and 90\% took less than 1 minute, according to a study of Azure Function's usage in 2019~\cite{shahrad2020serverless}. %AWS Lambda used to limit a function's maximum memory to 3,008\MB\ and maximum run time to 5 minutes before 2020~\cite{aws_lambda_pricing}. 
In recent years, thanks to its benefits, there has been an increasing desire to run more types of larger applications on serverless~\cite{lambda-ml-inf,XXX}. In response, AWS Lambda has increased its per-function resource limit from 3,008\MB\ and a maximum run time of 5 minutes to 10\GB\ and 15 minutes in 2020~\cite{aws_lambda_increase}. 
 
\boldunderpara{Limitations of FaaS for Larger Applications.} Although FaaS resource limits increase enable the execution of larger applications, 
today's FaaS-based serverless systems has fundamental limitations for running medium- and large-scale applications in a resource-efficient way. 
First, today's serverless systems allocate all resources for a function when it starts and keeps the same amount of resources until the function finishes.
When larger and longer applications execute as functions on serverless, their different execution phases often have different resource needs (\eg, pre-processing tokens vs. attention computation in large-language-model inference).
With today's serverless, users have to provision functions for peak usages but end up not using the peak resources all the time.
Second, a function's resource reservation is fixed across invocations in today's serverless offerings. Yet, different inputs to a function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}, which is more likely to happen with the more complex medium- to large-scale applications.
This lack of elasticity would result in resource waste or in the worst case, function failure, if an invocation exceeds the resource reservation.
Third, providers offer fixed, limited sets of function CPU-to-memory ratios. 
Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}, and these issues are more severe as applications become larger.
Finally, programmers today have to rewrite existing medium- to large-scale applications to run on FaaS, usually by manually splitting a program into functions, by using a storage layer like S3 or in-memory storage~\cite{klimovic2018pocket,} to share data across functions, and by expressing functions in an application as a DAG with an orchestration layer~\cite{AWS-Step-Functions,azure_durable_functions}. 

%Because of these benefits, efforts have been made to port large-scale applications such as data analytics~\cite{XXX} and machine learning~\cite{XXX} to serverless computing, even though serverless computing is designed and optimized for running short, small-scale functions. These prior efforts demonstrate the feasibility and benefits of running large-scale applications in a serverless manner, but they have two major issues.

\if 0
Despite many benefits, today's FaaS-based serverless computing still has several key limitations.
%and we believe that they are major reasons that prevent serverless computing from enabling a richer set of applications.
First, function CPU-to-memory ratios are fixed by providers. 
Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}.
Second, a function's resource reservation is fixed across invocations, but different inputs to the same function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}.
This lack of elasticity would result in resource waste or in the worst case, function failure, if an invocation exceeds the resource reservation.
%, \eg, Google Cloud Functions offer six combinations of CPU frequency and memory sizes
%\zhiyuan{maybe add: in a single execution}
Third, all resources are allocated from the provider at the beginning of a function and kept as long as the function lives.
Thus, users have to provision functions for peak usages but end up not using the peak resources all the time.
%As a result, either the cloud provider~\cite{azure_functions_pricing} or the user needs to pay for the unused resources~\cite{aws_lambda_pricing,google_functions_pricing}. %, because cloud providers cannot easily exploit the unused resources.
Meanwhile, data generated during function execution cannot live after execution ends, 
which makes sharing such data across functions difficult and slow~\cite{klimovic2018pocket,sreekanti2020cloudburst}.
Finally, the maximum amount of resources a function can use is limited, which can force users to rewrite their large-scale applications like machine-learning inference~\cite{lambda-ml-inf} as smaller pieces that can fit in functions. 
%and/or to use an external service to host its extra resource needs. 
\fi

These limitations are caused by today's \textit{function-centric} serverless model, where a function is the unit of resource allocation and scaling. This model works well when functions are small but would cause resource wastage when functions become larger.
We argue that larger serverless applications call for more fine-grained resource allocation and scaling.

%Our observation is that the root cause of these limitations is today's \textbf{\textit{function-centric}} serverless model.
%A function is a rigid, fixed-size box that couples computing resources as an inseparable unit throughout a function's execution and across the function's invocations.
%If there is any mismatch between an application's resource need and a cloud provider's pre-defined function sizes,
%users will suffer from resource wastage, performance penalty, and/or program rewriting burden. 

%We argue that we should forgo the function-based execution model and 
We build \textbf{\textit{\sys}}, a serverless computing platform that executes medium- to large-scale applications in a resource-efficient way with fine-grained resource allocation and scaling. %To achieve fine-grained resource allocation and scaling, we 
Our main idea is to decompose an application into different pieces according to the application's execution resource needs. Specifically, we decouple code pieces and data objects with different resource amounts (number of vCPUs, memory size) %different resource {\em type}s (\eg, CPU vs. memory), different resource {\em amount}s (\eg, a memory object of 100\MB\ vs. one of 1\GB), 
and different lifetime. These decoupled pieces form a {\em resource graph} according to their control flow and data flow. 
Nodes in a resource graph represent either a piece of application code (what we call a {\em compute component}) or one or more data objects (what we call a {\em memory component}). %A user application can be viewed as a {\em resource graph}, 
Each component has three associated resource features: %differs in at least one of the three resource features from other components: 
\textit{resource type, resource amount, and span}. %We expect one resource 
We impose no limit on the amount or time span of a component (within user's budget cap), and these values can vary across invocations or even within an invocation. 
% (\eg, when \sys\ auto-scales up a memory component).
%Under the hood, our compiler and libraries map user applications to a \textbf{\textit{resource graph}} that \sys\ executes. 
% One component can trigger other components, run in parallel with other ones, or communicate with other ones. 
A component can trigger, run in parallel with, or communicate with other components.
% (\eg, a compute component access data in a memory component).
%\noteryan{This section makes it seem like two components can not have identical resource requirements. It's not immediately clear, at least from this section, why this is. (IE: a parralelizable algo evenly split into individual equally partitioned nodes).}.
%based NumPy library). 
%A \sys\ compiler generates a resource graph and components in it from annotated user programs or from \sys\ library calls; 
%our run-time system dynamically determines the amount and span of a component based on its actual run-time resource needs.

\input{fig-motivation-exp}

To obtain the resource graph for a user program, we first profile the program's execution with sampled inputs to acquire object sizes, per-code-block CPU usage, and memory access intensity. We then compile the code to separate out code pieces with different CPU consumption as different compute components and larger or shared objects as memory components.

Our proposed resource graph allows excellent flexibility for capturing user applications' fine-grained resource needs. However, it introduces a major technical challenge to cloud providers:
\emph{allowing arbitrary resource features (type, amount, span) of components could lead to inefficient resource usage} where available resources are ``stranded''. % (\ie, available resources that cannot be used by any applications). %\noteryan{This is a bit vague on the definition and cause of stranding. I would either expand on what you mean by stranding, or at least cite a paper that discusses bin-packing problems here.}
Resource stranding happens when a server has some free resource, %(\eg, 256\MB\ of memory), 
but it cannot be used by any workloads because all workloads need more than the free amount %(\eg, if the smallest component to be scheduled is 512\MB) 
or because another type of resource is not free. % (\eg, no free CPU cycles). 
%Stranded resources can amount to 25\% when the load is high in today's cloud VM instances~\cite{Pond}.
%Arbitrary resource type, amount, and span could lead to even more resources being stranded.
%Stranded resources on a server cannot be utilized until a workload releases resources. With arbitrary component time span, resource can be stranded for long.
If there are only one or few allocation sizes, then resource stranding can be largely avoided. This is the approach taken by today's FaaS. Unfortunately, such allocation limits are the exact cause of FaaS' problems.
% from being used by any jobs and thus cannot be charged to any user. \notehx{what is the logic here (from `stranded' to `can't be charged')}
%\notegeoff{I also found it hard to understand what you meant by "reading" here.  it seems like the current fixed resource allocation model leads to more stranding than having a flexible resource allocation model.}
%To avoid this problem, today's serverless platforms impose fixed CPU-memory ratio and size/run-time limits on functions~\cite{bilal2021,job-packing}, which unfortunately is the cause of various problems discussed earlier. 

We solve the resource-stranding problem with two system-level ideas, while allowing components in a resource graph to have arbitrary resource features. Our first idea is to {\em disaggregate} resource types by allocating CPU-type components in a CPU-centric server pool and memory-type components in a memory-centric server pool. 
By allocating only one type at a time in that type's pool, we can avoid the need to find a server that has available free amount of every resource type~\cite{multi-bin-packing,multi-bin-packing-2}, while not imposing any ratio on CPU and memory.
%Without disaggregation, scheduling a component needs to find a server that has free space for each  we can avoid the type of resource stranding that is caused by multi-dimensional bin packing while allowing arbitrary CPU-memory ratio. %\notehx{so the fundamental benefit is to make charging easier?}
%\notegeoff{two separable aspects of Scad are (1) more flexibile and dynamic resource allocation model of cpu and memory over time, and (2) a disaggregated system architecture.  as a reviewer, I would argue that (2) does not necessarily follow from (1) --- you can get benefits from a more flexible model even with a standard server architecture.  so my suggestion is to add in an argument for why it makes sense to implement the new model using a disaggregated architecture (e.g., easier provisioning, scheduling; better resource utilization; reliability?; etc.  it may take up too much space in the intro to do it, so perhaps Sec 2 or 5 would be a better place.}

%\notezhiyuan{balance between program and execution time, also the amount problem? hide resource mapping}
%Solving the resource-stranding problem then reduces to efficiently scheduling a component in a single-typed pool.
The above disaggregation approach solves the resource type problem, but resource stranding can still happen within a single pool since a component can still have arbitrary amount and span and we allow a component to grow in size.
%an arbitrary amount and span of a component of one resource type. 
To address this problem, we introduce our second idea: \textit{``materializing'' an arbitrary sized (virtual) component} of a type with multiple \textit{fixed-size physical components} of that type. 
%\notegeoff{this is just allocation pool binning like malloc?}
Virtual components capture arbitrary resource needs of an application, while physical components are the actual execution units that have only a few fixed sizes, similar to how memory pages help avoid external fragmentation for arbitrarily-sized virtual memory areas. 
%\notehx{I also don't see a connection here. Why physical components have to be fixed sized? Isn't this counter-intuitive since you already use disaggregated cpu and memory?}
%Scheduling smaller and fixed-size physical components is easy and avoids resource stranding.
To further provide tight resource utilization, we dynamically create and terminate physical components in an {\em on-demand, auto-scaled} manner for each invocation.
%\noteyiying{shall we say something about our diff to mem page?}
%For example, a virtual memory component can grow from 10 128\MB\ physical components to 20 128\MB\ physical components during its execution, and another invocation of the same virtual component could lead to only 1 64\MB\ physical component. \notehx{is this similar to how virtual/physical memory works? virtual components are what get exposed to users? what is a `component` exactly?}

Our resource disaggregation and physical component materialization ideas solve the resource stranding problem, but they bring two challenges: performance overhead caused by network delays between physical components and system scalability to handle decomposed components. %When optimizing for low cost, our goal is to retain the performance of today's serverless computing.
%\notehx{Doesn't this problem already exist? as long as you disaggregated memory/cpu, you would suffer from network delays?}
We solve these problem from several perspectives.
First, we use a hierachical scheduling system with locality-aware scheduling policy to improve scheduler scalability and to reduce communication delay. %perform locality-aware scheduling to place frequently communicating components close to each other. 
%as close to each other as possible, in addition to cold-start-aware scheduling and pre-warming techniques.
Second, we separate control-path operations like network connection establishment from performance critical paths. %\noteryan{The idea of hiding operations behind critical path sounds odd in my head. I would probably say separate control path operations from performance-critical path.}
%Second, we build an efficient RDMA-based communication system that judiciously exploits an indirect channel for fast connection setup, while allowing direct component-to-component communication after the setup.
Third, we %compile user programs to directly access memory components with 
use a memory-like internal interface to directly access memory components and avoid serialization/de-serialization. 
Fourth, we cache/buffer read/write data in a small local cache, and we batch network accesses.
Finally, if performance overhead is still high after the above optimizations, we merge, or {\em aggregate}, components that have high communication overhead and run them together in one execution environment in a separate server pool. %{\em balanced pool}.
%implement a customized RDMA stack to further improve performance over our TCP stack. 
%and use several remote-memory access optimizations such as local caching, access batching, and zero copy. % to further improve performance.

%In the worst case where performance overhead is still high after the above optimizations, we propose to merge, or {\em aggregate}, components that have high communication overhead and run them together in one execution environment in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources. We dynamically aggregate and disaggregate components to tune the tradeoff between performance and efficient resource utilization.

%In addition to enabling new long-running, resource-intensive serverless workloads, Scad maintains or improves the efficiency of today's short-lived workloads that are not split. 
%For these, Scad is equivalent to today’s stateful serverless systems, but with added support for autoscaling state. 
% Thus, Scad’s scheduling overhead and overall performance are also similar to today’s serverless systems for short-lived workloads.
%To demonstrate these, 

We implemented \sys\ on top of OpenWhisk~\cite{OpenWhisk}
% .
%\sys\ efficiently schedules and launches components in their corresponding resource pools, automatically scales components in an on-demand, elastic manner, and transparently accelerates the communication across components that are partitioned by the network.
%Currently, \sys\ only supports Python, but our approach could be easily extended to other languages.
and evaluated it with a set of microbenchmarks and two real-world applications:  machine-learning model training and data analytics with a TPC-DS benchmark.
We compared \sys\ to OpenWhisk, AWS Lambda, AWS Step Functions~\cite{AWS-Step-Functions}, Orion~\cite{Orion-osdi22}, %Azure Durable Functions~\cite{azure_durable_functions,Burckhardt_2021}, 
and PyWren~\cite{jonas2017occupy_pywren}.
Our machine-learning results show that \sys\ reduces resource consumption by 40\% to 84\% compared to OpenWhisk while only adding 1.3\% performance overhead.
Our TPC-DS results show that \sys\ reduces resource consumption by 16\% to 31\% and counter-intuitively, improves performance by 15\% to 28\% compared to PyWren, thanks to our more efficient remote-data accessing mechanism and our better scaling of compute resources.
%Our results demonstrate that \sys\ reduces application resource consumption by  up to 6.1\X\ while improving application run time by up to 28\% compared to existing systems.  \notegeoff{since Scad uses remote memory, a reviewer might be surprised that the system improves performance.  so you might couch it in terms of something like, "Even though ... remote memory ..., Scad is able to improve performance because data does not need to be serialiazed/unserialized between components..."}
%\yiying{Zhiyuan, what exactly is the 28\% number? Total run time of an application?} \zhiyuan{Yes its execution time}
%In addition, \sys\ enabled workloads that are larger than today's FaaS limits without any developer involvement.










\if 0

To enable this vision, we judiciously exploit two ideas, {\em disaggregation} and {\em aggregation}.

\boldunderpara{Disaggregation.} Our first idea is based on resource disaggregation, a popular data-center architecture which separates resources into different pools.
Today's disaggregation systems disaggregate user applications based on their resource types (\eg, separating compute from memory)~\cite{Shan18-OSDI,semeru-osdi20,AIFM}.
%The criteria for disaggregation in a serverless computing setting, however, should not just be resource type as in traditional disaggregation systems.
To fit the elasticity of serverless computing, we propose to also disaggregate based on (1) resource amount and (2) span of execution (\ie, phases or relative time windows within an application's execution time).
%\yiying{Shall we give an example here? It's a bit hard to talk in abstract terms, but I don't know how to properly give a (short) example here.}
Specifically, we disaggregate a serverless application into {\em component}s, each representing either a piece of application code (\ie, compute component) or a data structure (\ie, memory component) with a distinct triad, \textit{$<$resource type, resource amount, span$>$}.
%\yiying{not sure if we should still keep the triad here.}
Components with different resource types run on different disaggregated resource pools. %\textcolor{red}{\sout{(\eg, a memory component runs in a memory pool)}}.
A user application can be described as a {\em resource graph}, where one component can communicate with or trigger other ones.
%An component is the unit of scheduling, execution, and auto-scaling. 
%For example, a compute component runs in a compute pool, and a memory component runs in a memory pool.
%Users supply a graph of components to \sys\ for their application, with an easy-to-use interface \sys\ provides.
%components of an application form a graph, which represents both the task flow and the data flow. 
%One component can trigger one or more components (\ie, task flow) and multiple components running at the same time can communicate with each other (\ie, data flow). 
%Users supply resource graphs to \sys, with an easy-to-use interface \sys\ provides.

%Resource disaggregation has the potential of fulfilling both these two required changes, as it allows users to separately define execution units with different resource features and allows providers to easily manage and execute such units.
%Disaggregation allows users to precisely and freely define the resources they deem fit for their applications, thereby 
Serverless-specific disaggregation has several key benefits. 
First, it enables the independent scaling of different resource types, thereby allowing arbitrary resource ratios (\eg, CPU-to-memory ratio). 
Second, instead of provisioning for the peak resource usage, we can use multiple components to capture resource consumption changes in a user application.
Third, when pooling resources, applications can allocate and use resources beyond what a single node can provide. 
%Users however can specify cost rate limits to prevent incurring unexpected charges.
Finally, when serverless applications want to access or share data that cannot fit into the local environment, allowing them to use a memory interface to access disaggregated memory could potentially yield better performance than accessing a storage layer via a storage interface as in today's serverless systems.
% \zhiyuan{Tightly connected components can avoid communication and computational overhead introduced by restructuring application into resource limited functions.}
Together, the first two features improve {\em resource efficiency}, and the latter two improve {\em performance}.
% \zhiyuan{Together improves {\em resource efficiency}, and {\em performance}.}
%essentially lifting today's FaaS function resource limits.
%, thereby saving the total cost to run the application.
%Right-sizing resources for different phases of an application results in less total resources and thus lower cost.
%For example, if the initial phase of an application uses a huge data structure, the next phase uses only a few variables, and the last phase uses a median-sized data structure, we could use a huge memory component, no memory component, and a median-sized component for these phases while using a single compute component for the entire duration.
%In contrast, today's FaaS would use one function with huge memory for the entire duration.
%As a result, disaggregation reduces the total resource consumption and thus user costs.
%Finally, because components can have different lifetimes, applications can decouple the lifetime of data (memory components) from computation (compute components). %and use the memory component interface to easily manage intermediate data. 
%For example, a memory component representing intermediate data can live from the start of its first producer to the end of its last consumer.

\zhiyuan{Merge this part to execution. should we follow the same structure here? (profiling, compiling, execution)}
\boldunderpara{Aggregation.} Despite its benefits,
disaggregation inevitably incurs increased network communication.
% network communication is intrinsic to disaggregation can affect performance.
%This problem could become more severe when users unnecessarily split their applications into very fine-grained pieces. 
Moreover, when disaggregating an application into smaller units, each of them could potentially incur scheduling and startup overhead.
%The overhead of both items could be significant in a serverless setting.
To reduce or eliminate these overheads, our second idea is to merge, or {\em aggregate}, components and when possible, run them together in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources.
Aggregated components can run locally
% in one execution environment
in one environment on one server, avoiding the network communication overhead, startup time, and scheduling burden.
%Aggregation can go beyond even what today's single-function limit, allowing the merging of potentially several functions in a DAG.
%They can also be scheduled and launched as one unit, reducing the system overhead.

%Overall, disaggregation allows an serverless application to be executed in fine granularity thereby being \textbf{more resource efficient \zhiyuan{and solve resource-related performance problem}} than today's serverless solutions. Aggregation allows an application to go beyond the limit of today's FaaS functions thereby avoiding the otherwise needed network communication and \textbf{improving performance}. \zhiyuan{improve performance overhead introduced by disaggregation?}

\fi

\if 0
Both disaggregation and aggregation bring new challenges under the serverless computing setting.
First, disaggregation inevitably introduces more inter-component communication. Such communication needs to sustain much higher load and achieve much lower latency than today's function-to-function communication.
Second, an component should be elastic and auto-scaled.
Third, the startup time of components could have a bigger impact on application performance when components run shorter than typical traditional functions.
Unfortunately, none of today's serverless computing platforms are designed or can properly handle disaggregation and aggregation.

\boldunderpara{\sys.} We built {\em \sys} ({\em Serverless Computing with Aggregation and Disaggregation}), a resource-centric serverless computing framework that dynamically aggregates and disaggregates components based on resource utilization and application behavior. 
Users can port their applications to \sys by annotating the original programs %(\eg, adding split points in a program) 
or by using libraries that \sys provides. %(\eg, a remote-memory-based NumPy library). 
Under the hood, our compiler and libraries map user applications to a component-based interface that \sys\ executes.
\sys\ can run all applications supported by today's serverless platforms and many that are not. %\yiying{not very sure if this is the best way to say it..}
Applications whose resource usage patterns vary during the execution
% whose usage patterns are input-dependent,
and/or use vast amounts of resources can especially benefit from \sys.
% \zhiyuan{Changed here}
%\yiying{give some example applications here?} \zhiyuan{i'd say do not emphysis on phases here? Programs suffers limited, coupled and variance resource usage patterns can especially benefit from \sys.}

Despite these many benefits, disaggregation and aggregation in a serverless setting bring two major challenges.
%in resource scaling and component management, as elaborated below: 

%Different from traditional disaggregation systems, in the serverless setting, \sys\ needs to not only disaggregate resources based on new criteria but also efficiently start and automatically scale the disaggregated components.
%Moreover, \sys\ should dynamically disaggregate and aggregate components in an efficient and adaptive manner.
%Making disaggregation and aggregation work in a serverless setting is not easy, as every disaggregated component needs to start up quickly and automatically adapt to changes in resource demands (\ie, auto-scaling).
%Moreover, disaggregated components need to communicate efficiently. 
%Moreover, as \sys\ allows users to define components, inevitably user definitions can be imprecise or even wrong. 
%For example, a user may split their application into too fine-grained components. 
%Often times an application’s resource features are highly
%dependent on input and cannot be pre-determined. Thus, \sys\ should be able to {\em morph} an resource graph into different shapes by disaggregating and aggregating different components dynamically.
%To achieve these goals, \sys\ follows two design principles.
%Although resource disaggregation and serverless computing are each fairly well understood, it is 
%\hx{The following two paragraphs need more work; they do not read smoothly along the flow. How is it related to disaggregation/aggregation?  We shouldn't create another branch that is off of the main presentation flow.  Can we not talk about ``ideas'' again? We already talked two main ideas before.  All we need to do in this paragraph is to show how \sys instantiates these two ideas rather than introducing new ideas. }
%\hx{Relate each of these principles to the big picture of aggregation/disaggregation. For example, ``to efficiently implement aggregation/disaggregation, \sys uses two design principles'' or something like that. It is hard for me to see the transitioning/relationship. }

First, \emph{how to deal with dynamic resource scaling and aggregation that components must undertake} at the run time to achieve our targeted performance and resource benefits. For instance, a memory component may contain an array that grows dynamically, possibly requiring space beyond what the server that hosts it can offer. As another example, \sys\ may need to aggregate a compute and a memory component to improve their communication performance. To enable flexible resource adjustment, we decouple {\em virtual} and {\em physical} components. Virtual components, which capture application features and are generated statically by compilers, remain unchanged throughout the execution. Physical components, on the contrary, are dynamically added, released, or merged at run time in response to load changes. As a result, there can be one-to-one, one-to-many, or many-to-one relationships between virtual and physical components. These relationships are managed dynamically by \sys, enabling elasticity in a straightforward manner. 
%A virtual component can be {\em materialized} to one or more physical components at runtime.
%These physical components can be dynamically added or removed based on load changes, and they can exist on different servers.
%Meanwhile, multiple virtual components could also be aggregated and executed as one physical unit.
%The location, amount, and even the existence of physical components are hidden from the user.
%For example, a virtual memory component could be materialized as multiple physical memory components that potentially sit on different servers,
%while multiple virtual components could also be aggregated and executed as one physical memory.
%This decoupling allows \sys's runtime system to make different scheduling and execution choices while preserving application-specific features. 
%Moreover, it enables the dynamic elasticity of components.
%This decoupling is possible due to the serverless computing model: users supply application code and leave the provisioning and execution to providers.

Second, \emph{how to efficiently handle the two relationships in resource graphs: data communication and task triggering}.
Different from traditional disaggregation systems which focus on optimizing the run-time communication performance (data plane),
in a serverless setting, we also need to efficiently start up the communication across {\em dynamically instantiated} components (control plane).
We build an RDMA-based communication system that judiciously exploits an indirect channel for connection setup, while allowing direct component-to-component communication after the setup.
Different from today's serverless task-flow systems, our resource graph can contain many more components, demanding efficient scheduling and failure handling.
We propose a two-level scheduling system that launches components in a just-in-time, asynchronous, and reliable manner.
%\sys's second design principle is to decouple the {\em data flow} from the {\em task flow}.
%A data flow captures how data is accessed or transferred across components, while a task flow captures how components trigger the start of other components.
%\sys\ separates the design of data flow and task flow, with the former targeting fast, direct communication and the latter targeting fast startup and fault tolerance.
%For example, we implemented an RDMA-based component-to-component communication system for the data flow
%and a two-level scheduling system that launches components in a pre-warmed, asynchronous, and reliable manner. 
\fi


\if 0
Overall, this paper makes the following contributions:

\vspace{-\topsep}
\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
    \myitemit{The identification of various resource-related limitations of today's FaaS-based serverless computing.}
    \myitemit{The proposal of resource-centric serverless computing.}
    \myitemit{The first system that integrates serverless computing with resource disaggregation, with solutions like aggregation to make the integration practical.}
    \myitemit{A demonstration of how to decouple data and task flows.}
%    \myitemit{Solutions like aggregation to make disaggregation practical.}
%    \myitemit{The implementation and evaluation of \sys.}
     \myitemit{New scheduling and component launching mechanisms and policies designed for resource-centric serverless computing.}
     \myitemit{An RDMA-based, transparently virtualized, direct communication system that could be used in serverless settings beyond resource-centric serverless computing.}
    \myitemit{A demonstration of how to make applications written in managed languages like Python performant in a disaggregated serverless environment.}
    \myitemit{Three serverless computing applications ported to \sys.}
\end{itemize}

%We will make \sys\ publicly available upon the publication of this paper.
\fi


==> intro-old.tex <==
%\yiying{All, I have three versions of Intro. The most recent one is the current Section 1. The oldest version is Section 3. Let me know which version is better (or none of them is good) and/or how to improve.}
\section{Introduction}
\label{sec:intro}

Serverless computing, commonly offered as Function-as-a-Service (FaaS), is a cloud service that allows users to deploy and execute their applications without managing servers.
%(or more specifically, any software or hardware infrastructures beneath their applications).
%Initially introduced for cloud providers to exploit unused data-center resources, 
% Serverless computing has gained significant popularity in recent years because of its benefits to cloud users: minimal IT burdens and paying only when their applications run.
Serverless computing has gained tremendous popularity in the past few years thanks to its benefit of minimal IT burdens, pay-per-use pricing, and automatic scaling (auto-scaling)~\cite{serverless-growth-1,serverless-growth-2}.

Initially, serverless computing was designed for running short, small-scale functions like simple HTML serving. 
%Accordingly, AWS Lambda used to limit a function's maximum memory to 3,008\MB\ and maximum run time to 5 minutes before 2020~\cite{aws_lambda_pricing}. 
In recent years, there has been an increasing desire to run large, complex applications such as video processing~\cite{excamera,ao2018sprocket},
%\notemohammad{Ref 9 is from 2018 and Ref 21 is from 2017! These cannot back the argument that "there has been an increasing desire ...", since they are from 5-6 years ago.}
%\noteyiying{added new refs in 2022 and 2023 for the AWS and Databricks ones}
scientific computing~\cite{numpywren,serverlessseqcompar19}, machine-learning tasks~\cite{carreira2019cirrus,AWS-SageMaker-Serverless,Azure-ML-Training-Serverless}, data analytics~\cite{Databricks-SQL-Serverless,AWS-Redshift-Serverless}, and relational databases~\cite{AWS-Aurora-Serverless,Azure-SQL-Serverless-Announce} in a serverless style, as these applications are also event-triggered and can benefit from pay-per-use pricing, auto-scaling, and reduced IT burdens. These applications 1) run longer or consume more memory than typical FaaS function size limits, 2) exhibit resource usage variations across different phases of computation, 3) require different amounts of resources with different inputs.
We call applications that have one or more of these features {\em bulky applications}.


This paper answers two key research questions: 1) {\em What should auto-scaling mean for bulky applications?} 
2) {\em How to properly execute bulky applications in a serverless style?}
\notezhiyuan{very good summary! one question: what do serverless style means? it should cover auto scale, no-provisioned server, anything else?  Maybe: How to properly execute bulky applications in a serverless style? 1) What should auto-scaling mean for bulky applications? 2) (Should be performance?) }

Today's FaaS-based serverless platforms use function as the unit for auto-scaling and resource allocation. As user request load increases (\ie, more triggering events happening), more functions are allocated and launched.
This function unit works well for small-scale applications but creates three fundamental issues for bulky applications.
First, FaaS platforms allocate all resources for a function invocation when it starts and maintains them until it ends.
As bulky applications usually have different resource consumption phases during their execution, provisioning for peak usage would cause significant resource waste during non-peak time.
%(\eg, reading compressed images, decompressing them, and detecting faces in them). 
Second, a function's size is fixed across invocations in today's FaaS offerings. Yet, different inputs to a bulky application often have different resource requirements~\cite{bilal2021,mvondo2021ofc}, resulting in resource waste if provisioning for peak input usage or application failure when under-provisioning.
Third, FaaS scales application computation by launching parallel executions of a function. However, function as the scaling unit could be too coarse-grained, as bulky applications can have different parallelism needs across their execution and separate CPU and memory scaling needs. %Launching parallel instances of an entire bulky application is an overkill and causes resource waste.
In sum, today's \textit{function-centric} serverless model, where a function is the unit of resource allocation and scaling, is a poor fit for running bulky applications. %in a serverless style.

\notezhiyuan{Last point still do not make sense? should be resource bundle, or performance}

\if 0
%\notezhiyuan{Resource scaling instead of auto scaling?}
Today's practice to run bulky applications in the serverless style is to manually split or rewrite a program as a set of functions, by using a storage layer like S3 or in-memory storage to share data and communicate across functions~\cite{klimovic2018pocket,mvondo2021ofc,romero2021faa,wang2020infinicache,pu2019shuffling,sreekanti2020cloudburst}, and by expressing functions in an application as a DAG with an orchestration layer~\cite{AWS-Step-Functions,azure_durable_functions}. 
%, and its usage in public clouds has followed this pattern. For example, 50\% of functions running took less than 3 seconds to execute, and 90\% took less than 1 minute, according to a study of Azure Function's usage in 2019~\cite{shahrad2020serverless}. %AWS Lambda used to limit a function's maximum memory to 3,008\MB\ and maximum run time to 5 minutes before 2020~\cite{aws_lambda_pricing}. 
%In recent years, thanks to its benefits, there has been  
Meanwhile, to respond to the increasing need for running bulky applications, AWS Lambda, AWS's FaaS service, has increased its per-function resource limit from 3,008\MB\ to 10\GB\ and a maximum run time from 5 minutes to 15 minutes in 2020~\cite{aws_lambda_increase}. 
%\notemohammad{This from 3 years ago. I wonder if the fact that this has not been increased since then raises more questions.}

%We argue that the two practices today (manual splitting of applications and increasing function sizes) have fundamental limitations that prevent the wider adoption of serverless computing for bulky applications. 
%\boldunderpara{Limitations of FaaS for Larger Applications.} 
%Although FaaS resource limits increase enable the execution of larger applications, today's FaaS-based serverless systems have fundamental limitations for running medium- and large-scale applications in a resource-efficient way. 

%On the one hand, 
Today's function-centric serverless frameworks like FaaS have two fundamental resource-efficiency issues, and running bulky applications with increased function sizes will only result in more resource wastage.
First, today's serverless systems allocate all resources for a function when it starts; this amount stays the same during the function's execution.
%\notemohammad{"until the function finishes" -> it is also common for those resources to be kept alive after execution to mitigate cold starts.}
However, bulky applications usually have different resource consumption phases during their execution (\eg, reading compressed images, decompressing them, and detecting faces in them). 
%\noteyiying{is this a good example? if so, we should say which phase in this pipeline is more or less resource hunger.}
%\notemohammad{"(\eg, decoding a video, detecting faces in it, and then encoding it)" > This is not a great example, and someone who has not worked with that specific benchmark would have a hard time grasping this.}
%With today's serverless, users have to provision functions for peak usages but end up not using the peak resources all the time.
Second, a function's size is fixed across invocations in today's serverless offerings. Yet, different inputs to a function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}, which is more likely to happen with bulky applications.
This lack of elasticity results in resource wastage or, in the worst case, function failure if an invocation exceeds the resource reservation.
%Finally, providers offer fixed, limited sets of function CPU-to-memory ratios. Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}, and these issues are more severe as applications become larger.


%\notezhiyuan{Maybe no effort part? just focus on the limit and inefficient. mention inefficient not only caused by uers but also }
On the other hand, manually porting applications into DAGs of functions heavily burdens developers, as they need to split existing programs manually and repeatedly test that each split piece fits within a function's resource limit. Moreover, manually generated DAGs could be resource-inefficient, as programmer-determined application splitting could be too fine-grained, resulting in huge function-communication/startup overhead, or too coarse-grained, resulting in resource wastage within a function.
\zhiyuan{To be presented as a single DAG}
\fi
%Because of these benefits, efforts have been made to port large-scale applications such as data analytics~\cite{XXX} and machine learning~\cite{XXX} to serverless computing, even though serverless computing is designed and optimized for running short, small-scale functions. These prior efforts demonstrate the feasibility and benefits of running large-scale applications in a serverless manner, but they have two major issues.

\if 0
Despite many benefits, today's FaaS-based serverless computing still has several key limitations.
%and we believe that they are major reasons that prevent serverless computing from enabling a richer set of applications.
First, function CPU-to-memory ratios are fixed by providers. 
Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}.
Second, a function's resource reservation is fixed across invocations, but different inputs to the same function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}.
This lack of elasticity would result in resource waste or, in the worst case, function failure if an invocation exceeds the resource reservation.
%, \eg, Google Cloud Functions offer six combinations of CPU frequency and memory sizes
%\zhiyuan{maybe add: in a single execution}
Third, all resources are allocated from the provider at the beginning of a function and kept as long as the function lives.
Thus, users have to provision functions for peak usages but end up not using the peak resources all the time.
%As a result, either the cloud provider~\cite{azure_functions_pricing} or the user needs to pay for the unused resources~\cite{aws_lambda_pricing,google_functions_pricing}. %, because cloud providers cannot easily exploit the unused resources.
Meanwhile, data generated during function execution cannot live after execution ends, 
which makes sharing such data across functions difficult and slow~\cite{klimovic2018pocket,sreekanti2020cloudburst}.
Finally, the maximum amount of resources a function can use is limited, which can force users to rewrite their large-scale applications like machine-learning inference~\cite{lambda-ml-inf} as smaller pieces that can fit in functions. 
%and/or to use an external service to host its extra resource needs. 
\fi

%These limitations are caused by today's \textit{function-centric} serverless model, where a function is the unit of resource allocation and scaling. This model works well when applications are small but would cause significant resource waste when applications become larger and bulkier.
%To work around FaaS's limitations, programmers today have to rewrite existing medium- to large-scale applications to run on FaaS, usually by manually splitting a program into functions, by using a storage layer like S3 or in-memory storage~\cite{klimovic2018pocket,} to share data across functions, and by expressing functions in an application as a DAG with an orchestration layer~\cite{AWS-Step-Functions,azure_durable_functions}. 
%We argue that larger serverless applications call for more fine-grained resource allocation and scaling.

%\notezhiyuan{resource flexibility}
As applications get bulkier, we believe their resource allocation and scaling granularity should be made smaller than an application. Moreover, instead of having fixed granularity, the granularity should follow and adapt to each execution run of a bulky application. With this fine-grained, internal resource scaling and execution idea, we propose a \textbf{\textit{resource-centric}} serverless model for bulky applications and build \textbf{\textit{\sys}}, a new framework for efficiently executing bulky applications in a serverless style. Figure~\ref{fig-faasraas} and Figure~\ref{fig-overall} illustrate \sys's overall idea and architecture.
%\sys\ includes a profiler, a compiler, and a runtime system, as shown in Figure~\ref{fig-overall}. 


%Users deploy their applications as original programs with optional annotations; they do not need to set any resource size but can optionally cap the maximum they are willing to pay.
% \notezhiyuan{may delete the limitation part. I think its a patch not our main point}
%\sys\ sets no resource limit to an application but allows users to set a constraint on the maximum amount of resources they are willing to pay for.
%Event-triggered applications with different resource and scaling requirements within the same invocation or across invocations would benefit particularly from \sys, but \sys\ still supports other types of serverless applications, such as those currently run on FaaS. 
%\sys\ still supports small serverless applications and large applications with constant resource needs. For the former, \sys\ works similarly to FaaS; for the latter, \sys\ works similarly to traditional VMs. \noteyiying{instead of defining bulky applications, I'm just saying what types of applications would benefit from us and what we can support}
%\notezhiyuan{we now have no evaluation of this. Still I think its a patch, should not be in the intro}

\if 0
At the core of \sys\ is the concept of resource-centric computing graph, or {\em resource graph}, which captures the internal resource requirements and their relationships of an application.
%\notezhiyuan{should not be stable? we are missing that the component could scale based on across different inputs. which is not connected to later part.}
%\noteyiying{I can't think of a better word than stable. Stable CPU doesn't mean same CPU across invocations. It just means that the utilization stays the same in one execution. I think this should be fine.}
Nodes in a resource graph represent either a piece of application code with stable CPU usage (\ie, a {\em compute component}) or one or more data objects with similar lifetime (\ie, a {\em data component}).
%\notezhiyuan{A reousrce graph could outline the resource requirements and sharing relatinship of in an application}
%A user application can be viewed as a {\em resource graph}, 
%Each component has two associated resource features: %differs in at least one of the three resource features from other components: 
%\textit{resource type, resource amount, and lifetime}. At least one feature differs from other components for the code piece or data objects to be a unique component. %We expect one resource 
%We impose no limit on the amount or lifetime of a component (within user's budget cap), and these values can vary across invocations or even within an invocation (\eg, a memory component . 
% (\eg, when \sys\ auto-scales up a memory component).
%Under the hood, our compiler and libraries map user applications to a \textbf{\textit{resource graph}} that \sys\ executes. 
% One component can trigger other components, run in parallel with other ones, or communicate with other ones. 
A component can trigger, access, or communicate with other components, and these relationships form the edges of a resource graph.

\sys\ captures resource graphs based on an application's historical executions. 
%\notezhiyuan{maybe move the profiling part to later after we motivate why we need to capture history?}
%The resource graph is our model for capturing an application's historical resource features and is the basis of our runtime scheduling and auto-scaling.
%\notezhiyuan{detailed explaination. the reousrce sharing pattern and amount enables us to see components as estimate the resoource needs, instead of isolated executions, enabling our following key implementation.}
It performs lightweight profiling on sampled user invocations to capture the resource usage of code ranges and data object sizes, based on which we generate the resource graph of an application with the \sys\ program analyzer and compiler. 
\sys\ captures the per-component peak resource usage for all user runs, which we use to set the expected size of each component.
%Based on profiling results, \sys\ identifies compute and data components and generates compute-components' code using our compiler.
%samples user invocations of an application for performing our lightweight profiling. Based on profiled resource-usage patterns, \sys\ compiles user programs into resource graphs. %For example, we group large objects with similar lifetimes into a data object and then analyze programs to turn  
%When knowing the resource features of an application through its resource graph, a runtime system can proactively schedule and scale CPU and memory resources in the right amounts that meet the needs of an application's different execution phases.

%We argue that we should forgo the function-based execution model and 
 %To achieve fine-grained resource allocation and scaling, we 


%To obtain the resource graph for a user program, we first profile the program's execution with sampled inputs to acquire object sizes, per-code-block CPU usage, and memory access intensity. We then compile the code to separate out code pieces with different CPU consumption as different compute components and larger or shared objects as memory components.

%\notezhiyuan{maybe change the order and the key words. see slack msg.}
Executing captured resource graphs in a resource-efficient and performance-efficient way presents several challenges: 1) To provide generic support for bulky applications, we impose no size limit on any component in a resource graph. Thus, a component can exceed a server's available resources.
2) The best way to execute a resource graph depends on the cluster resource availability. For example, components can be co-scheduled on the same server when resources are ample.
3) As our profiling results are from past sampling runs, a future run can have inputs not profiled before. Thus, our generated resource graphs may diverge from the actual application resource needs.
\fi

%To confront these challenges, we propose the {\em adaptive materialization} of resource graphs by forming an {\em execution graph} based on an application's resource graph, the runtime resource availability, and each invocation's actual resource demands. %where \sys\ determines the location and execution methods of each component. 

\notezhiyuan{Better definition focusing on transforming. Use three separate cases? cross-server, cross invocation, lifetime.}
\notezhiyuan{Materialization is tightly coupled to performance? we could do all connected by IPC implementaion.}
\notezhiyuan{This fine-grained approach may face the same problem as functions: high inter-communication overhead and scheduling overhead. An ideal case would be, when resoruces available on one machine, it should be executed as if its a single monolith function. If more resoruces are needed, it should be able to dymaically utilize the resoruce on other servers. }
\notezhiyuan{This is a requirements from the innner-requirement of serverless.}
The main idea behind \sys\ is \textbf{\textit{adaptive serverless}}, where the resource allocation and execution of a bulky application adapts to its internal resource requirements and cluster resource availability.
% \zhiyuan{
%This means at runtime the same bulky applications could be executed as a single local process, a utilizing remote memory or even a distributed process span over multiple servers.
% }
\noteyiying{what you added is redundant as the content below. we need to keep intro short}
%\zhiyuan{For example,}
\sys\ first tries to execute a bulky application as one process in a single server. When no single server can host it, \sys\ executes it on multiple servers.
\notezhiyuan{How to execute on multiple servers?}
As the application's resource needs change throughout its execution, \sys\ decreases or increases the corresponding amount on the same server(s) if possible. However,
% as we do not reserve resources to minimize resource waste, 
increasing CPU or memory resources on a server is not always possible. In this case, \sys\ launches increased computing or memory resources on another server while maintaining the already launched resources at the initial server to avoid migration costs. If no single server can host the added resources, \sys\ allocates the needed resources from multiple servers.

Adaptive serverless executes bulky applications in a resource-efficient and, thus, cost-efficient way.
However, several key technical challenges must be solved to make this approach viable. 

%whenever possible and expresses all data accesses as native memory instructions. If the server has enough resources for running the subsequent compute components, these components will execute in the same process as the previous component, avoiding the overhead of any execution environment launch time. 
%If a compute and a data component can fit in a single server, \sys\ schedules them together, with data accessed through native memory instructions. 
%In resource-constraint scenarios, \sys\ would schedule data components away from compute components and transparently orchestrate data accesses via network communication. 
%For large data components, \sys\ may also allocate multiple memory regions from multiple servers. %We also apply adaptive materialization for triggering compute components, scheduling triggered components in the same container if the server has enough resources and on another server otherwise.
%\notezhiyuan{not underestimated, maybe just say runtime resource requirements}
%Furthermore, to handle resource demands that diverge from previous profiling results, \sys\ dynamically adds physical resources to a component on demand. 

%\input{tab-intro}
\input{fig-faasraas}

\notezhiyuan{Connecting to this? The challange of execution. (not adaptive?) => Requirement is fast response}


First, \sys\ needs to capture internal resource features in a bulky application so that \sys\ can quickly and properly make autoscaling decisions during the application's execution.
Instead of imposing runtime monitoring overhead and allocating purely on demand, our solution is to capture resource features prior to the execution with a combination of user hints and coarse-grained profiling history.
Users express where resource changes may happen by annotating their source programs and using \sys's library; profiling history guides the resource amounts within each unchanged phase.
Internally, \sys\ record these pieces of prior information as a {\em resource graph}, as shown in Figure~\ref{fig-overall}. At runtime, \sys\ makes {\em proactive} resource scheduling decisions based on an application's resource graph and cluster resource availability. \sys\ handles inaccurate prior knowledge by making on-demand resource adjustments. Compared to a pure on-demand approach, \sys\ largely avoids the performance overhead of execution and network environment setup.

Second, adaptive serverless implies that different parts of an application may execute on the same or different servers at runtime.
\sys\ should efficiently support both local and remote executions.
Our approach is to {\em pre-compile} both versions (\eg, local execution uses native memory accesses; remote execution uses RDMA). Doing so allows \sys\ runtime to quickly choose a compilation that fits the runtime needs.

%can scale cpu and memory separately if needed

\input{fig-overall}

Finally, good application performance requires proper run-time support at different layers. At the scheduling layer, \sys\ employs a two-level scheduler architecture that performs coarse-grained scheduling at a global node and fine-grained allocation at the rack and server level. \sys\ adopts a {\em just-in-time} scheduling policy that makes scheduling and execution decisions just before the resources are needed. 
%of a component and launches it when its previous component is running. For compute components, \sys\ performs automatic CPU and memory scaling in an on-demand and transparent fashion. For data accesses and data components, \sys\ compiles a native and an API-based remote version for the \sys\ scheduler to choose between quickly, and we allocate local or remote memory space in an adaptive and auto-scaled way. 
For memory accesses, \sys\ supports and dynamically chooses native local memory accesses, object-based remote memory accesses, and transparent remote memory swapping.
For network communication, we propose a new control plane for fast connection establishment in a serverless style. Finally, \sys\ handles failure by partial re-execution of failed components and consistency by providing synchronization primitives.

\if 0
\notezhiyuan{I think we cannot implement the policy with this. maybe just remove the straight forward part.}
A straightforward way to implement the above policies is to determine an entire execution graph and reserve all resources needed. However, resource reservation causes significant wastage.
\notezhiyuan{The motivation should be 1) the resoruce avaliable 2) requirement for each input are both flexible. Should map to motivation point 2)3). The question should be When/How to do this adaptive materialization. }
Instead, we perform {\em just-in-time} materialization by scheduling the following component(s) in a resource graph when the current component executes. Just-in-time materialization avoids resource wastage, adapts execution plans based on real-time cluster resource utilization and component execution locations, and overlaps the start-up time of the next component's environment with the current component's execution.
\notezhiyuan{These are implementation detials, maybe not here or lead by a word saying this is an optimization. }
For \sys\ runtime to quickly choose a materialization way, we compile multiple versions of components in a resource graph offline (\eg, one compilation that co-locates a data and a compute component with native memory accesses and one non-colocated compilation with network accesses).
%A straightforward way of realizing adaptive materialization is to determine the entire execution graph when a user event triggers an application and reserve the resources for the execution graph. This approach has two issues. First, reserving resources for the entire application's duration causes significant resource wastage. Second, determining the resources needed by an entire execution graph before its execution is hard. 
\fi

%Altogether, resource graphs allow the \sys\ runtime to have prior knowledge of component relationships and their estimated sizes, with which it can make good locality-based scheduling decisions. Adaptive materialization allows for \sys\ to adjust to runtime cluster environment and application resource needs. Our designs at different layers of \sys\ enable the efficient execution of these ideas.
%\noteyiying{not sure where to best put the above sentences. having them here for now}
%Altogether, \sys\ adapt run-time resource allocation based on profiled application resource patterns and cluster resource availability, thereby achieving both resource efficiency and performance efficiency.

We evaluate \sys\ with a set of microbenchmarks and three real-world applications: a machine-learning task, data analytics queries from the TPC-DS benchmark, and video processing pipelines.
We compared \sys\ to two FaaS frameworks (OpenWhisk~\cite{OpenWhisk}, AWS Lambda~\cite{AWS-Lambda}), four serverless DAG frameworks (AWS Step Functions~\cite{AWS-Step-Functions}, PyWren~\cite{jonas2017occupy_pywren}, ExCamera~\cite{excamera}, gg~\cite{fouladi2019laptop}), one serverless resource tuning system (Orion~\cite{Orion-osdi22}), and two VM-based execution methods (remote-memory swapping~\cite{FastSwap}, VM migration~\cite{XXX}).
Our machine-learning results show that \sys\ reduces resource consumption by 40\% to 84\% compared to OpenWhisk while only adding 1.3\% performance overhead.
Our TPC-DS results show that \sys\ reduces resource consumption by 73\% to 85\% and improves performance by 54\% to 64\% compared to PyWren.
Our video process results show that \sys\ reduces resource consumption by 33\% to 90\% and improves performance by 33\% to 47\% compared to gg on Openwhisk.

We will make \sys\ publicly available upon acceptance.
%Our results demonstrate that \sys\ reduces application resource consumption by  up to 6.1\X\ while improving application run time by up to 28\% compared to existing systems.  \notegeoff{since Scad uses remote memory, a reviewer might be surprised that the system improves performance.  so you might couch it in terms of something like, "Even though ... remote memory ..., Scad is able to improve performance because data does not need to be serialiazed/unserialized between components..."}
%\yiying{Zhiyuan, what exactly is the 28\% number? Total run time of an application?} \zhiyuan{Yes its execution time}
%In addition, \sys\ enabled workloads that are larger than today's FaaS limits without any developer involvement.




\if 0
Our resource disaggregation and physical component materialization ideas solve the resource stranding problem, but they bring two challenges: performance overhead caused by network delays between physical components and system scalability to handle decomposed components. %When optimizing for low cost, our goal is to retain the performance of today's serverless computing.
%\notehx{Doesn't this problem already exist? as long as you disaggregated memory/cpu, you would suffer from network delays?}
We solve these problem from several perspectives.
First, we use a hierachical scheduling system with locality-aware scheduling policy to improve scheduler scalability and to reduce communication delay. %perform locality-aware scheduling to place frequently communicating components close to each other. 
%as close to each other as possible, in addition to cold-start-aware scheduling and pre-warming techniques.
Second, we separate control-path operations like network connection establishment from performance critical paths. %\noteryan{The idea of hiding operations behind critical path sounds odd in my head. I would probably say separate control path operations from performance-critical path.}
%Second, we build an efficient RDMA-based communication system that judiciously exploits an indirect channel for fast connection setup, while allowing direct component-to-component communication after the setup.
Third, we %compile user programs to directly access memory components with 
use a memory-like internal interface to directly access memory components and avoid serialization/de-serialization. 
Fourth, we cache/buffer read/write data in a small local cache, and we batch network accesses.
\fi

%In the worst case where performance overhead is still high after the above optimizations, we propose to merge, or {\em aggregate}, components that have high communication overhead and run them together in one execution environment in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources. We dynamically aggregate and disaggregate components to tune the tradeoff between performance and efficient resource utilization.

%In addition to enabling new long-running, resource-intensive serverless workloads, Scad maintains or improves the efficiency of today's short-lived workloads that are not split. 
%For these, Scad is equivalent to today’s stateful serverless systems, but with added support for autoscaling state. 
% Thus, Scad’s scheduling overhead and overall performance are also similar to today’s serverless systems for short-lived workloads.
%To demonstrate these, 









\if 0

To enable this vision, we judiciously exploit two ideas, {\em disaggregation} and {\em aggregation}.

\boldunderpara{Disaggregation.} Our first idea is based on resource disaggregation, a popular data-center architecture which separates resources into different pools.
Today's disaggregation systems disaggregate user applications based on their resource types (\eg, separating compute from memory)~\cite{Shan18-OSDI,semeru-osdi20,AIFM}.
%The criteria for disaggregation in a serverless computing setting, however, should not just be resource type as in traditional disaggregation systems.
To fit the elasticity of serverless computing, we propose to also disaggregate based on (1) resource amount and (2) span of execution (\ie, phases or relative time windows within an application's execution time).
%\yiying{Shall we give an example here? It's a bit hard to talk in abstract terms, but I don't know how to properly give a (short) example here.}
Specifically, we disaggregate a serverless application into {\em component}s, each representing either a piece of application code (\ie, compute component) or a data structure (\ie, memory component) with a distinct triad, \textit{$<$resource type, resource amount, span$>$}.
%\yiying{not sure if we should still keep the triad here.}
Components with different resource types run on different disaggregated resource pools. %\textcolor{red}{\sout{(\eg, a memory component runs in a memory pool)}}.
A user application can be described as a {\em resource graph}, where one component can communicate with or trigger other ones.
%An component is the unit of scheduling, execution, and auto-scaling. 
%For example, a compute component runs in a compute pool, and a memory component runs in a memory pool.
%Users supply a graph of components to \sys\ for their application, with an easy-to-use interface \sys\ provides.
%components of an application form a graph, which represents both the task flow and the data flow. 
%One component can trigger one or more components (\ie, task flow) and multiple components running at the same time can communicate with each other (\ie, data flow). 
%Users supply resource graphs to \sys, with an easy-to-use interface \sys\ provides.

%Resource disaggregation has the potential of fulfilling both these two required changes, as it allows users to separately define execution units with different resource features and allows providers to easily manage and execute such units.
%Disaggregation allows users to precisely and freely define the resources they deem fit for their applications, thereby 
Serverless-specific disaggregation has several key benefits. 
First, it enables the independent scaling of different resource types, thereby allowing arbitrary resource ratios (\eg, CPU-to-memory ratio). 
Second, instead of provisioning for the peak resource usage, we can use multiple components to capture resource consumption changes in a user application.
Third, when pooling resources, applications can allocate and use resources beyond what a single node can provide. 
%Users however can specify cost rate limits to prevent incurring unexpected charges.
Finally, when serverless applications want to access or share data that cannot fit into the local environment, allowing them to use a memory interface to access disaggregated memory could potentially yield better performance than accessing a storage layer via a storage interface as in today's serverless systems.
% \zhiyuan{Tightly connected components can avoid communication and computational overhead introduced by restructuring application into resource limited functions.}
Together, the first two features improve {\em resource efficiency}, and the latter two improve {\em performance}.
% \zhiyuan{Together improves {\em resource efficiency}, and {\em performance}.}
%essentially lifting today's FaaS function resource limits.
%, thereby saving the total cost to run the application.
%Right-sizing resources for different phases of an application results in less total resources and thus lower cost.
%For example, if the initial phase of an application uses a huge data structure, the next phase uses only a few variables, and the last phase uses a median-sized data structure, we could use a huge memory component, no memory component, and a median-sized component for these phases while using a single compute component for the entire duration.
%In contrast, today's FaaS would use one function with huge memory for the entire duration.
%As a result, disaggregation reduces the total resource consumption and thus user costs.
%Finally, because components can have different lifetimes, applications can decouple the lifetime of data (memory components) from computation (compute components). %and use the memory component interface to easily manage intermediate data. 
%For example, a memory component representing intermediate data can live from the start of its first producer to the end of its last consumer.

\zhiyuan{Merge this part to execution. should we follow the same structure here? (profiling, compiling, execution)}
\boldunderpara{Aggregation.} Despite its benefits,
disaggregation inevitably incurs increased network communication.
% network communication is intrinsic to disaggregation can affect performance.
%This problem could become more severe when users unnecessarily split their applications into very fine-grained pieces. 
Moreover, when disaggregating an application into smaller units, each of them could potentially incur scheduling and startup overhead.
%The overhead of both items could be significant in a serverless setting.
To reduce or eliminate these overheads, our second idea is to merge, or {\em aggregate}, components and when possible, run them together in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources.
Aggregated components can run locally
% in one execution environment
in one environment on one server, avoiding the network communication overhead, startup time, and scheduling burden.
%Aggregation can go beyond even what today's single-function limit, allowing the merging of potentially several functions in a DAG.
%They can also be scheduled and launched as one unit, reducing the system overhead.

%Overall, disaggregation allows an serverless application to be executed in fine granularity thereby being \textbf{more resource efficient \zhiyuan{and solve resource-related performance problem}} than today's serverless solutions. Aggregation allows an application to go beyond the limit of today's FaaS functions thereby avoiding the otherwise needed network communication and \textbf{improving performance}. \zhiyuan{improve performance overhead introduced by disaggregation?}

\fi

\if 0
Both disaggregation and aggregation bring new challenges under the serverless computing setting.
First, disaggregation inevitably introduces more inter-component communication. Such communication needs to sustain much higher load and achieve much lower latency than today's function-to-function communication.
Second, an component should be elastic and auto-scaled.
Third, the startup time of components could have a bigger impact on application performance when components run shorter than typical traditional functions.
Unfortunately, none of today's serverless computing platforms are designed or can properly handle disaggregation and aggregation.

\boldunderpara{\sys.} We built {\em \sys} ({\em Serverless Computing with Aggregation and Disaggregation}), a resource-centric serverless computing framework that dynamically aggregates and disaggregates components based on resource utilization and application behavior. 
Users can port their applications to \sys by annotating the original programs %(\eg, adding split points in a program) 
or by using libraries that \sys provides. %(\eg, a remote-memory-based NumPy library). 
Under the hood, our compiler and libraries map user applications to a component-based interface that \sys\ executes.
\sys\ can run all applications supported by today's serverless platforms and many that are not. %\yiying{not very sure if this is the best way to say it..}
Applications whose resource usage patterns vary during the execution
% whose usage patterns are input-dependent,
and/or use vast amounts of resources can especially benefit from \sys.
% \zhiyuan{Changed here}
%\yiying{give some example applications here?} \zhiyuan{i'd say do not emphysis on phases here? Programs suffers limited, coupled and variance resource usage patterns can especially benefit from \sys.}

Despite these many benefits, disaggregation and aggregation in a serverless setting bring two major challenges.
%in resource scaling and component management, as elaborated below: 

%Different from traditional disaggregation systems, in the serverless setting, \sys\ needs to not only disaggregate resources based on new criteria but also efficiently start and automatically scale the disaggregated components.
%Moreover, \sys\ should dynamically disaggregate and aggregate components in an efficient and adaptive manner.
%Making disaggregation and aggregation work in a serverless setting is not easy, as every disaggregated component needs to start up quickly and automatically adapt to changes in resource demands (\ie, auto-scaling).
%Moreover, disaggregated components need to communicate efficiently. 
%Moreover, as \sys\ allows users to define components, inevitably user definitions can be imprecise or even wrong. 
%For example, a user may split their application into too fine-grained components. 
%Often times an application’s resource features are highly
%dependent on input and cannot be pre-determined. Thus, \sys\ should be able to {\em morph} an resource graph into different shapes by disaggregating and aggregating different components dynamically.
%To achieve these goals, \sys\ follows two design principles.
%Although resource disaggregation and serverless computing are each fairly well understood, it is 
%\hx{The following two paragraphs need more work; they do not read smoothly along the flow. How is it related to disaggregation/aggregation?  We shouldn't create another branch that is off of the main presentation flow.  Can we not talk about ``ideas'' again? We already talked two main ideas before.  All we need to do in this paragraph is to show how \sys instantiates these two ideas rather than introducing new ideas. }
%\hx{Relate each of these principles to the big picture of aggregation/disaggregation. For example, ``to efficiently implement aggregation/disaggregation, \sys uses two design principles'' or something like that. It is hard for me to see the transitioning/relationship. }

First, \emph{how to deal with dynamic resource scaling and aggregation that components must undertake} at the run time to achieve our targeted performance and resource benefits. For instance, a memory component may contain an array that grows dynamically, possibly requiring space beyond what the server that hosts it can offer. As another example, \sys\ may need to aggregate a compute and a memory component to improve their communication performance. To enable flexible resource adjustment, we decouple {\em virtual} and {\em physical} components. Virtual components, which capture application features and are generated statically by compilers, remain unchanged throughout the execution. Physical components, on the contrary, are dynamically added, released, or merged at run time in response to load changes. As a result, there can be one-to-one, one-to-many, or many-to-one relationships between virtual and physical components. These relationships are managed dynamically by \sys, enabling elasticity in a straightforward manner. 
%A virtual component can be {\em materialized} to one or more physical components at runtime.
%These physical components can be dynamically added or removed based on load changes, and they can exist on different servers.
%Meanwhile, multiple virtual components could also be aggregated and executed as one physical unit.
%The location, amount, and even the existence of physical components are hidden from the user.
%For example, a virtual memory component could be materialized as multiple physical memory components that potentially sit on different servers,
%while multiple virtual components could also be aggregated and executed as one physical memory.
%This decoupling allows \sys's runtime system to make different scheduling and execution choices while preserving application-specific features. 
%Moreover, it enables the dynamic elasticity of components.
%This decoupling is possible due to the serverless computing model: users supply application code and leave the provisioning and execution to providers.

Second, \emph{how to efficiently handle the two relationships in resource graphs: data communication and task triggering}.
Different from traditional disaggregation systems which focus on optimizing the run-time communication performance (data plane),
in a serverless setting, we also need to efficiently start up the communication across {\em dynamically instantiated} components (control plane).
We build an RDMA-based communication system that judiciously exploits an indirect channel for connection setup, while allowing direct component-to-component communication after the setup.
Different from today's serverless task-flow systems, our resource graph can contain many more components, demanding efficient scheduling and failure handling.
We propose a two-level scheduling system that launches components in a just-in-time, asynchronous, and reliable manner.
%\sys's second design principle is to decouple the {\em data flow} from the {\em task flow}.
%A data flow captures how data is accessed or transferred across components, while a task flow captures how components trigger the start of other components.
%\sys\ separates the design of data flow and task flow, with the former targeting fast, direct communication and the latter targeting fast startup and fault tolerance.
%For example, we implemented an RDMA-based component-to-component communication system for the data flow
%and a two-level scheduling system that launches components in a pre-warmed, asynchronous, and reliable manner. 
\fi


\if 0
Overall, this paper makes the following contributions:

\vspace{-\topsep}
\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
    \myitemit{The identification of various resource-related limitations of today's FaaS-based serverless computing.}
    \myitemit{The proposal of resource-centric serverless computing.}
    \myitemit{The first system that integrates serverless computing with resource disaggregation, with solutions like aggregation to make the integration practical.}
    \myitemit{A demonstration of how to decouple data and task flows.}
%    \myitemit{Solutions like aggregation to make disaggregation practical.}
%    \myitemit{The implementation and evaluation of \sys.}
     \myitemit{New scheduling and component launching mechanisms and policies designed for resource-centric serverless computing.}
     \myitemit{An RDMA-based, transparently virtualized, direct communication system that could be used in serverless settings beyond resource-centric serverless computing.}
    \myitemit{A demonstration of how to make applications written in managed languages like Python performant in a disaggregated serverless environment.}
    \myitemit{Three serverless computing applications ported to \sys.}
\end{itemize}

%We will make \sys\ publicly available upon the publication of this paper.
\fi


==> intro-zhiyuan.tex <==
%\yiying{All, I have three versions of Intro. The most recent one is the current Section 1. The oldest version is Section 3. Let me know which version is better (or none of them is good) and/or how to improve.}
\section{Introduction}
\label{sec:intro}

Serverless computing, commonly offered as Function-as-a-Service (FaaS), is a cloud service that allows users to deploy and execute their applications without managing servers.
%(or more specifically, any software or hardware infrastructures beneath their applications).
%Initially introduced for cloud providers to exploit unused data-center resources, 
% Serverless computing has gained significant popularity in recent years because of its benefits to cloud users: minimal IT burdens and paying only when their applications run.
Serverless computing has gained tremendous popularity in the past few years thanks to its benefit of minimal IT burdens, pay-per-use pricing, and automatic scaling (auto-scaling)~\cite{serverless-growth-1,serverless-growth-2}.

Initially, serverless computing was designed for running short, small-scale functions like simple HTML serving. 
%Accordingly, AWS Lambda used to limit a function's maximum memory to 3,008\MB\ and maximum run time to 5 minutes before 2020~\cite{aws_lambda_pricing}. 
In recent years, there has been an increasing desire to run large, complex applications such as video processing~\cite{excamera,ao2018sprocket},
%\notemohammad{Ref 9 is from 2018 and Ref 21 is from 2017! These cannot back the argument that "there has been an increasing desire ...", since they are from 5-6 years ago.}
%\noteyiying{added new refs in 2022 and 2023 for the AWS and Databricks ones}
scientific computing~\cite{numpywren,serverlessseqcompar19}, machine-learning tasks~\cite{carreira2019cirrus,AWS-SageMaker-Serverless,Azure-ML-Training-Serverless}, data analytics~\cite{Databricks-SQL-Serverless,AWS-Redshift-Serverless}, and relational databases~\cite{AWS-Aurora-Serverless,Azure-SQL-Serverless-Announce} in a serverless style, as these applications are also event-triggered and can benefit from pay-per-use pricing, auto-scaling, and reduced IT burdens. These applications 1) run longer or consume more memory than typical FaaS function size limits, 2) exhibit resource usage variations across different phases of computation, 3) require different amounts of resources with different inputs.
We call serverless applications with one or more of these features {\em bulky serverless applications}, or bulky applications for short.

Today's practice of running bulky applications in a serverless style is function DAGs~\cite{AWS-Step-Functions,jonas2017occupy_pywren,excamera,azure_durable_functions,OpenWhisk-composer,zhang2020kappa,gg}, where users construct a DAG of functions and set the size of each function in the DAG. This approach creates several resource-waste and performance issues.
First, a function's size is fixed across invocations. Yet, with different inputs,
%to a bulky application often have different resource requirements~\cite{bilal2021,mvondo2021ofc}, resulting in 
there will be resource waste if provisioning for peak input usage or application failure if under-provisioning.
Second, different functions in a DAG execute in different environments (\eg, containers on one server or different servers). 
Communicating between environments and setting up the environments can become a major performance overhead, especially when breaking a bulky application into many functions.
On the other hand, reducing the number of environments by making functions bigger would cause resource waste, as a function has the same resource allocation throughout its execution; resources allocated for the peak execution needs are wasted during non-peak time of the function.
Finally, functions in a DAG store and access intermediate state in a disaggregated layer, usually over a key-value-like interface~\cite{klimovic2018pocket,XXX}.

\if 0
This paper answers two key research questions for building serverless systems for bulky applications: 1) {\em What should auto-scaling mean for bulky applications?} 
2) {\em How to properly execute bulky applications in a serverless style?}
\notezhiyuan{very good summary! one question: what do serverless style means? it should cover auto scale, no-provisioned server, anything else?  Maybe: How to properly execute bulky applications in a serverless style? 1) What should auto-scaling mean for bulky applications? 2) (Should be performance?) }

Today's FaaS-based serverless platforms use function as the unit for auto-scaling and resource allocation. As user request load increases (\ie, more triggering events happening), more functions are allocated and launched.
This function unit works well for small-scale applications but creates three fundamental issues for bulky applications.
First, FaaS platforms allocate all resources for a function invocation when it starts and maintains them until it ends.
As bulky applications usually have different resource consumption phases during their execution, provisioning for peak usage would cause significant resource waste during non-peak time.
%(\eg, reading compressed images, decompressing them, and detecting faces in them). 
Second, a function's size is fixed across invocations in today's FaaS offerings. Yet, different inputs to a bulky application often have different resource requirements~\cite{bilal2021,mvondo2021ofc}, resulting in resource waste if provisioning for peak input usage or application failure when under-provisioning.
Third, FaaS scales application computation by launching parallel executions of a function. However, function as the scaling unit could be too coarse-grained, as bulky applications can have different parallelism needs across their execution and separate CPU and memory scaling needs. %Launching parallel instances of an entire bulky application is an overkill and causes resource waste.
In sum, today's \textit{function-centric} serverless model, where a function is the unit of resource allocation and scaling, is a poor fit for running bulky applications. %in a serverless style.

\notezhiyuan{Last point still do not make sense? should be resource bundle, or performance}
\fi

\if 0
%\notezhiyuan{Resource scaling instead of auto scaling?}
Today's practice to run bulky applications in the serverless style is to manually split or rewrite a program as a set of functions, by using a storage layer like S3 or in-memory storage to share data and communicate across functions~\cite{klimovic2018pocket,mvondo2021ofc,romero2021faa,wang2020infinicache,pu2019shuffling,sreekanti2020cloudburst}, and by expressing functions in an application as a DAG with an orchestration layer~\cite{AWS-Step-Functions,azure_durable_functions}. 
%, and its usage in public clouds has followed this pattern. For example, 50\% of functions running took less than 3 seconds to execute, and 90\% took less than 1 minute, according to a study of Azure Function's usage in 2019~\cite{shahrad2020serverless}. %AWS Lambda used to limit a function's maximum memory to 3,008\MB\ and maximum run time to 5 minutes before 2020~\cite{aws_lambda_pricing}. 
%In recent years, thanks to its benefits, there has been  
Meanwhile, to respond to the increasing need for running bulky applications, AWS Lambda, AWS's FaaS service, has increased its per-function resource limit from 3,008\MB\ to 10\GB\ and a maximum run time from 5 minutes to 15 minutes in 2020~\cite{aws_lambda_increase}. 
%\notemohammad{This from 3 years ago. I wonder if the fact that this has not been increased since then raises more questions.}

%We argue that the two practices today (manual splitting of applications and increasing function sizes) have fundamental limitations that prevent the wider adoption of serverless computing for bulky applications. 
%\boldunderpara{Limitations of FaaS for Larger Applications.} 
%Although FaaS resource limits increase enable the execution of larger applications, today's FaaS-based serverless systems have fundamental limitations for running medium- and large-scale applications in a resource-efficient way. 

%On the one hand, 
Today's function-centric serverless frameworks like FaaS have two fundamental resource-efficiency issues, and running bulky applications with increased function sizes will only result in more resource wastage.
First, today's serverless systems allocate all resources for a function when it starts; this amount stays the same during the function's execution.
%\notemohammad{"until the function finishes" -> it is also common for those resources to be kept alive after execution to mitigate cold starts.}
However, bulky applications usually have different resource consumption phases during their execution (\eg, reading compressed images, decompressing them, and detecting faces in them). 
%\noteyiying{is this a good example? if so, we should say which phase in this pipeline is more or less resource hunger.}
%\notemohammad{"(\eg, decoding a video, detecting faces in it, and then encoding it)" > This is not a great example, and someone who has not worked with that specific benchmark would have a hard time grasping this.}
%With today's serverless, users have to provision functions for peak usages but end up not using the peak resources all the time.
Second, a function's size is fixed across invocations in today's serverless offerings. Yet, different inputs to a function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}, which is more likely to happen with bulky applications.
This lack of elasticity results in resource wastage or, in the worst case, function failure if an invocation exceeds the resource reservation.
%Finally, providers offer fixed, limited sets of function CPU-to-memory ratios. Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}, and these issues are more severe as applications become larger.


%\notezhiyuan{Maybe no effort part? just focus on the limit and inefficient. mention inefficient not only caused by uers but also }
On the other hand, manually porting applications into DAGs of functions heavily burdens developers, as they need to split existing programs manually and repeatedly test that each split piece fits within a function's resource limit. Moreover, manually generated DAGs could be resource-inefficient, as programmer-determined application splitting could be too fine-grained, resulting in huge function-communication/startup overhead, or too coarse-grained, resulting in resource wastage within a function.
\zhiyuan{To be presented as a single DAG}
\fi
%Because of these benefits, efforts have been made to port large-scale applications such as data analytics~\cite{XXX} and machine learning~\cite{XXX} to serverless computing, even though serverless computing is designed and optimized for running short, small-scale functions. These prior efforts demonstrate the feasibility and benefits of running large-scale applications in a serverless manner, but they have two major issues.

\if 0
Despite many benefits, today's FaaS-based serverless computing still has several key limitations.
%and we believe that they are major reasons that prevent serverless computing from enabling a richer set of applications.
First, function CPU-to-memory ratios are fixed by providers. 
Because workloads can have arbitrary CPU-to-memory ratios, fixed ratios result in either CPU/memory wastage (when provisioning for peaks) or performance degradation (when under-provisioned)~\cite{bilal2021}.
Second, a function's resource reservation is fixed across invocations, but different inputs to the same function could result in different resource requirements~\cite{bilal2021,mvondo2021ofc}.
This lack of elasticity would result in resource waste or, in the worst case, function failure if an invocation exceeds the resource reservation.
%, \eg, Google Cloud Functions offer six combinations of CPU frequency and memory sizes
%\zhiyuan{maybe add: in a single execution}
Third, all resources are allocated from the provider at the beginning of a function and kept as long as the function lives.
Thus, users have to provision functions for peak usages but end up not using the peak resources all the time.
%As a result, either the cloud provider~\cite{azure_functions_pricing} or the user needs to pay for the unused resources~\cite{aws_lambda_pricing,google_functions_pricing}. %, because cloud providers cannot easily exploit the unused resources.
Meanwhile, data generated during function execution cannot live after execution ends, 
which makes sharing such data across functions difficult and slow~\cite{klimovic2018pocket,sreekanti2020cloudburst}.
Finally, the maximum amount of resources a function can use is limited, which can force users to rewrite their large-scale applications like machine-learning inference~\cite{lambda-ml-inf} as smaller pieces that can fit in functions. 
%and/or to use an external service to host its extra resource needs. 
\fi

%These limitations are caused by today's \textit{function-centric} serverless model, where a function is the unit of resource allocation and scaling. This model works well when applications are small but would cause significant resource waste when applications become larger and bulkier.
%To work around FaaS's limitations, programmers today have to rewrite existing medium- to large-scale applications to run on FaaS, usually by manually splitting a program into functions, by using a storage layer like S3 or in-memory storage~\cite{klimovic2018pocket,} to share data across functions, and by expressing functions in an application as a DAG with an orchestration layer~\cite{AWS-Step-Functions,azure_durable_functions}. 
%We argue that larger serverless applications call for more fine-grained resource allocation and scaling.

%\notezhiyuan{resource flexibility}
The root cause of these issues is today's \textit{function-centric} serverless model, where the size and boundary of a function do not adapt to application workloads or the underlying cluster resource availability.
To address their issues, we propose an \textbf{\textit{adaptive, resource-centric}} serverless model.

%As applications get bulkier, we believe their resource allocation and scaling granularity should be made smaller than an application. Moreover, instead of having fixed granularity, the granularity should follow and adapt to each execution run of a bulky application. With this fine-grained, internal resource scaling and execution idea, we propose a \textbf{\textit{resource-centric}} serverless model for bulky applications and build \textbf{\textit{\sys}}, a new framework for efficiently executing bulky applications in a serverless style. Figure~\ref{fig-faasraas} and Figure~\ref{fig-overall} illustrate \sys's overall idea and architecture.
%\sys\ includes a profiler, a compiler, and a runtime system, as shown in Figure~\ref{fig-overall}. 


%Users deploy their applications as original programs with optional annotations; they do not need to set any resource size but can optionally cap the maximum they are willing to pay.
% \notezhiyuan{may delete the limitation part. I think its a patch not our main point}
%\sys\ sets no resource limit to an application but allows users to set a constraint on the maximum amount of resources they are willing to pay for.
%Event-triggered applications with different resource and scaling requirements within the same invocation or across invocations would benefit particularly from \sys, but \sys\ still supports other types of serverless applications, such as those currently run on FaaS. 
%\sys\ still supports small serverless applications and large applications with constant resource needs. For the former, \sys\ works similarly to FaaS; for the latter, \sys\ works similarly to traditional VMs. \noteyiying{instead of defining bulky applications, I'm just saying what types of applications would benefit from us and what we can support}
%\notezhiyuan{we now have no evaluation of this. Still I think its a patch, should not be in the intro}

\if 0
At the core of \sys\ is the concept of resource-centric computing graph, or {\em resource graph}, which captures the internal resource requirements and their relationships of an application.
%\notezhiyuan{should not be stable? we are missing that the component could scale based on across different inputs. which is not connected to later part.}
%\noteyiying{I can't think of a better word than stable. Stable CPU doesn't mean same CPU across invocations. It just means that the utilization stays the same in one execution. I think this should be fine.}
Nodes in a resource graph represent either a piece of application code with stable CPU usage (\ie, a {\em compute component}) or one or more data objects with similar lifetime (\ie, a {\em data component}).
%\notezhiyuan{A reousrce graph could outline the resource requirements and sharing relatinship of in an application}
%A user application can be viewed as a {\em resource graph}, 
%Each component has two associated resource features: %differs in at least one of the three resource features from other components: 
%\textit{resource type, resource amount, and lifetime}. At least one feature differs from other components for the code piece or data objects to be a unique component. %We expect one resource 
%We impose no limit on the amount or lifetime of a component (within user's budget cap), and these values can vary across invocations or even within an invocation (\eg, a memory component . 
% (\eg, when \sys\ auto-scales up a memory component).
%Under the hood, our compiler and libraries map user applications to a \textbf{\textit{resource graph}} that \sys\ executes. 
% One component can trigger other components, run in parallel with other ones, or communicate with other ones. 
A component can trigger, access, or communicate with other components, and these relationships form the edges of a resource graph.

\sys\ captures resource graphs based on an application's historical executions. 
%\notezhiyuan{maybe move the profiling part to later after we motivate why we need to capture history?}
%The resource graph is our model for capturing an application's historical resource features and is the basis of our runtime scheduling and auto-scaling.
%\notezhiyuan{detailed explaination. the reousrce sharing pattern and amount enables us to see components as estimate the resoource needs, instead of isolated executions, enabling our following key implementation.}
It performs lightweight profiling on sampled user invocations to capture the resource usage of code ranges and data object sizes, based on which we generate the resource graph of an application with the \sys\ program analyzer and compiler. 
\sys\ captures the per-component peak resource usage for all user runs, which we use to set the expected size of each component.
%Based on profiling results, \sys\ identifies compute and data components and generates compute-components' code using our compiler.
%samples user invocations of an application for performing our lightweight profiling. Based on profiled resource-usage patterns, \sys\ compiles user programs into resource graphs. %For example, we group large objects with similar lifetimes into a data object and then analyze programs to turn  
%When knowing the resource features of an application through its resource graph, a runtime system can proactively schedule and scale CPU and memory resources in the right amounts that meet the needs of an application's different execution phases.

%We argue that we should forgo the function-based execution model and 
 %To achieve fine-grained resource allocation and scaling, we 


%To obtain the resource graph for a user program, we first profile the program's execution with sampled inputs to acquire object sizes, per-code-block CPU usage, and memory access intensity. We then compile the code to separate out code pieces with different CPU consumption as different compute components and larger or shared objects as memory components.

%\notezhiyuan{maybe change the order and the key words. see slack msg.}
Executing captured resource graphs in a resource-efficient and performance-efficient way presents several challenges: 1) To provide generic support for bulky applications, we impose no size limit on any component in a resource graph. Thus, a component can exceed a server's available resources.
2) The best way to execute a resource graph depends on the cluster resource availability. For example, components can be co-scheduled on the same server when resources are ample.
3) As our profiling results are from past sampling runs, a future run can have inputs not profiled before. Thus, our generated resource graphs may diverge from the actual application resource needs.
\fi

%To confront these challenges, we propose the {\em adaptive materialization} of resource graphs by forming an {\em execution graph} based on an application's resource graph, the runtime resource availability, and each invocation's actual resource demands. %where \sys\ determines the location and execution methods of each component. 

%\notezhiyuan{Better definition focusing on transforming. Use three separate cases? cross-server, cross invocation, lifetime.}
%\notezhiyuan{Materialization is tightly coupled to performance? we could do all connected by IPC implementaion.}
%\notezhiyuan{This fine-grained approach may face the same problem as functions: high inter-communication overhead and scheduling overhead. An ideal case would be, when resoruces available on one machine, it should be executed as if its a single monolith function. If more resoruces are needed, it should be able to dymaically utilize the resoruce on other servers. }
%\notezhiyuan{This is a requirements from the innner-requirement of serverless.}

The main idea behind \sys\ is \textbf{\textit{adaptive serverless}}, where the resource allocation and execution of a bulky application adapts to its internal resource requirements and cluster resource availability.
As shown in Figure~\ref{fig-faasraas},
\sys\ first tries to execute a bulky application as one process in a single server. When no single server can host it, \sys\ executes it on multiple servers.
\notezhiyuan{How to execute on multiple servers?}
As the application's resource needs change throughout its execution, \sys\ decreases or increases the corresponding amount on the same server(s) if possible. However,
% as we do not reserve resources to minimize resource waste, 
increasing CPU or memory resources on a server is not always possible. In this case, \sys\ launches increased computing or memory resources on another server while maintaining the already launched resources at the initial server.
% to avoid migration costs.
If no single server can host the added resources, \sys\ allocates the needed resources from multiple servers.

Adaptive serverless executes bulky applications in a resource-efficient and, thus, cost-efficient way. 
Two key design in \sys{} brings adaptive serverless into practical.

%whenever possible and expresses all data accesses as native memory instructions. If the server has enough resources for running the subsequent compute components, these components will execute in the same process as the previous component, avoiding the overhead of any execution environment launch time. 
%If a compute and a data component can fit in a single server, \sys\ schedules them together, with data accessed through native memory instructions. 
%In resource-constraint scenarios, \sys\ would schedule data components away from compute components and transparently orchestrate data accesses via network communication. 
%For large data components, \sys\ may also allocate multiple memory regions from multiple servers. %We also apply adaptive materialization for triggering compute components, scheduling triggered components in the same container if the server has enough resources and on another server otherwise.
%\notezhiyuan{not underestimated, maybe just say runtime resource requirements}
%Furthermore, to handle resource demands that diverge from previous profiling results, \sys\ dynamically adds physical resources to a component on demand. 

%\input{tab-intro}
\input{fig-faasraas}

\notezhiyuan{Connecting to this? The challange of execution. (not adaptive?) => Requirement is fast response}


First, \sys autoscales resources using a \textbf{provisioned} approach.
Fine-grained and unpredictable auto-scaling could downgrade scheduling and execution performance.
Instead of purely on demand, our solution is to capture resource features prior to the execution with a combination of user hints and coarse-grained profiling history.
Users express where resource changes may happen by annotating their source programs.
Prior to execution,
\sys uses static analysis and profiling history to decide the resource amounts and scaling pattern within each annotated part.
Internally, \sys\ record the information as a {\em resource graph}, as shown in Figure~\ref{fig-overall}. At runtime, \sys\ makes {\em proactive} resource scheduling decisions, \eg{} preserving the resource based on history amount and future scaling when possible. \sys\ handles input variance or inaccurate prior knowledge by making on-demand resource adjustments following scaling patterns.
\notezhiyuan{How to autoscale?}
% Compared to a pure on-demand approach, \sys\ largely avoids the performance overhead of execution and network environment setup.


Second, \sys use \textbf{adaptive execution} to execute applications seamlessly in different forms, by decomposing the application into resource components following resource graph, and dynamically compose them at runtime.
\sys{} {\em compiles} actual component code to adapt to different compositions (\eg, local execution uses native memory accesses; remote accesses use RDMA). We pre-compile and cache the compilation results to allow \sys\ runtime to quickly choose from.
% that fits the runtime needs.
As a result, although resources are allocated and scheduled at fine granularity, \sys provides single binary like (for components on the same server) or hand-optimized distributed system level execution performance (for components on different servers).

%can scale cpu and memory separately if needed

\input{fig-overall}

Following the proactive and adaptive approach, good application performance requires proper runtime support at different layers.
At the scheduling layer, \sys\ employs a two-level scheduler architecture that performs coarse-grained scheduling at a global node and fine-grained allocation at the rack and server level. \sys\ adopts a {\em just-in-time} scheduling policy that makes scheduling and execution decisions just before the resources are needed. 
%of a component and launches it when its previous component is running. For compute components, \sys\ performs automatic CPU and memory scaling in an on-demand and transparent fashion. For data accesses and data components, \sys\ compiles a native and an API-based remote version for the \sys\ scheduler to choose between quickly, and we allocate local or remote memory space in an adaptive and auto-scaled way. 
% For memory accesses, \sys\ supports and dynamically chooses native local memory accesses, object-based remote memory accesses, and transparent remote memory swapping.
For communication, we propose a new control plane for fast connection establishment in a serverless style. Finally, \sys\ handles failure by partial re-execution of failed components and consistency by providing synchronization primitives.

\if 0
\notezhiyuan{I think we cannot implement the policy with this. maybe just remove the straight forward part.}
A straightforward way to implement the above policies is to determine an entire execution graph and reserve all resources needed. However, resource reservation causes significant wastage.
\notezhiyuan{The motivation should be 1) the resoruce avaliable 2) requirement for each input are both flexible. Should map to motivation point 2)3). The question should be When/How to do this adaptive materialization. }
Instead, we perform {\em just-in-time} materialization by scheduling the following component(s) in a resource graph when the current component executes. Just-in-time materialization avoids resource wastage, adapts execution plans based on real-time cluster resource utilization and component execution locations, and overlaps the start-up time of the next component's environment with the current component's execution.
\notezhiyuan{These are implementation detials, maybe not here or lead by a word saying this is an optimization. }
For \sys\ runtime to quickly choose a materialization way, we compile multiple versions of components in a resource graph offline (\eg, one compilation that co-locates a data and a compute component with native memory accesses and one non-colocated compilation with network accesses).
%A straightforward way of realizing adaptive materialization is to determine the entire execution graph when a user event triggers an application and reserve the resources for the execution graph. This approach has two issues. First, reserving resources for the entire application's duration causes significant resource wastage. Second, determining the resources needed by an entire execution graph before its execution is hard. 
\fi

%Altogether, resource graphs allow the \sys\ runtime to have prior knowledge of component relationships and their estimated sizes, with which it can make good locality-based scheduling decisions. Adaptive materialization allows for \sys\ to adjust to runtime cluster environment and application resource needs. Our designs at different layers of \sys\ enable the efficient execution of these ideas.
%\noteyiying{not sure where to best put the above sentences. having them here for now}
%Altogether, \sys\ adapt run-time resource allocation based on profiled application resource patterns and cluster resource availability, thereby achieving both resource efficiency and performance efficiency.

We evaluate \sys\ with a set of microbenchmarks and three real-world applications: a machine-learning task, data analytics queries from the TPC-DS benchmark, and video processing pipelines.
We compared \sys\ to two FaaS frameworks (OpenWhisk~\cite{OpenWhisk}, AWS Lambda~\cite{AWS-Lambda}), four serverless DAG frameworks (AWS Step Functions~\cite{AWS-Step-Functions}, PyWren~\cite{jonas2017occupy_pywren}, ExCamera~\cite{excamera}, gg~\cite{fouladi2019laptop}), one serverless resource tuning system (Orion~\cite{Orion-osdi22}), and two VM-based execution methods (remote-memory swapping~\cite{FastSwap}, VM migration~\cite{XXX}).
Our machine-learning results show that \sys\ reduces resource consumption by 40\% to 84\% compared to OpenWhisk while only adding 1.3\% performance overhead.
Our TPC-DS results show that \sys\ reduces resource consumption by 73\% to 85\% and improves performance by 54\% to 64\% compared to PyWren.
Our video process results show that \sys\ reduces resource consumption by 33\% to 90\% and improves performance by 33\% to 47\% compared to gg on Openwhisk.

We will make \sys\ publicly available upon acceptance.
%Our results demonstrate that \sys\ reduces application resource consumption by  up to 6.1\X\ while improving application run time by up to 28\% compared to existing systems.  \notegeoff{since Scad uses remote memory, a reviewer might be surprised that the system improves performance.  so you might couch it in terms of something like, "Even though ... remote memory ..., Scad is able to improve performance because data does not need to be serialiazed/unserialized between components..."}
%\yiying{Zhiyuan, what exactly is the 28\% number? Total run time of an application?} \zhiyuan{Yes its execution time}
%In addition, \sys\ enabled workloads that are larger than today's FaaS limits without any developer involvement.




\if 0
Our resource disaggregation and physical component materialization ideas solve the resource stranding problem, but they bring two challenges: performance overhead caused by network delays between physical components and system scalability to handle decomposed components. %When optimizing for low cost, our goal is to retain the performance of today's serverless computing.
%\notehx{Doesn't this problem already exist? as long as you disaggregated memory/cpu, you would suffer from network delays?}
We solve these problem from several perspectives.
First, we use a hierachical scheduling system with locality-aware scheduling policy to improve scheduler scalability and to reduce communication delay. %perform locality-aware scheduling to place frequently communicating components close to each other. 
%as close to each other as possible, in addition to cold-start-aware scheduling and pre-warming techniques.
Second, we separate control-path operations like network connection establishment from performance critical paths. %\noteryan{The idea of hiding operations behind critical path sounds odd in my head. I would probably say separate control path operations from performance-critical path.}
%Second, we build an efficient RDMA-based communication system that judiciously exploits an indirect channel for fast connection setup, while allowing direct component-to-component communication after the setup.
Third, we %compile user programs to directly access memory components with 
use a memory-like internal interface to directly access memory components and avoid serialization/de-serialization. 
Fourth, we cache/buffer read/write data in a small local cache, and we batch network accesses.
\fi

%In the worst case where performance overhead is still high after the above optimizations, we propose to merge, or {\em aggregate}, components that have high communication overhead and run them together in one execution environment in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources. We dynamically aggregate and disaggregate components to tune the tradeoff between performance and efficient resource utilization.

%In addition to enabling new long-running, resource-intensive serverless workloads, Scad maintains or improves the efficiency of today's short-lived workloads that are not split. 
%For these, Scad is equivalent to today’s stateful serverless systems, but with added support for autoscaling state. 
% Thus, Scad’s scheduling overhead and overall performance are also similar to today’s serverless systems for short-lived workloads.
%To demonstrate these, 









\if 0

To enable this vision, we judiciously exploit two ideas, {\em disaggregation} and {\em aggregation}.

\boldunderpara{Disaggregation.} Our first idea is based on resource disaggregation, a popular data-center architecture which separates resources into different pools.
Today's disaggregation systems disaggregate user applications based on their resource types (\eg, separating compute from memory)~\cite{Shan18-OSDI,semeru-osdi20,AIFM}.
%The criteria for disaggregation in a serverless computing setting, however, should not just be resource type as in traditional disaggregation systems.
To fit the elasticity of serverless computing, we propose to also disaggregate based on (1) resource amount and (2) span of execution (\ie, phases or relative time windows within an application's execution time).
%\yiying{Shall we give an example here? It's a bit hard to talk in abstract terms, but I don't know how to properly give a (short) example here.}
Specifically, we disaggregate a serverless application into {\em component}s, each representing either a piece of application code (\ie, compute component) or a data structure (\ie, memory component) with a distinct triad, \textit{$<$resource type, resource amount, span$>$}.
%\yiying{not sure if we should still keep the triad here.}
Components with different resource types run on different disaggregated resource pools. %\textcolor{red}{\sout{(\eg, a memory component runs in a memory pool)}}.
A user application can be described as a {\em resource graph}, where one component can communicate with or trigger other ones.
%An component is the unit of scheduling, execution, and auto-scaling. 
%For example, a compute component runs in a compute pool, and a memory component runs in a memory pool.
%Users supply a graph of components to \sys\ for their application, with an easy-to-use interface \sys\ provides.
%components of an application form a graph, which represents both the task flow and the data flow. 
%One component can trigger one or more components (\ie, task flow) and multiple components running at the same time can communicate with each other (\ie, data flow). 
%Users supply resource graphs to \sys, with an easy-to-use interface \sys\ provides.

%Resource disaggregation has the potential of fulfilling both these two required changes, as it allows users to separately define execution units with different resource features and allows providers to easily manage and execute such units.
%Disaggregation allows users to precisely and freely define the resources they deem fit for their applications, thereby 
Serverless-specific disaggregation has several key benefits. 
First, it enables the independent scaling of different resource types, thereby allowing arbitrary resource ratios (\eg, CPU-to-memory ratio). 
Second, instead of provisioning for the peak resource usage, we can use multiple components to capture resource consumption changes in a user application.
Third, when pooling resources, applications can allocate and use resources beyond what a single node can provide. 
%Users however can specify cost rate limits to prevent incurring unexpected charges.
Finally, when serverless applications want to access or share data that cannot fit into the local environment, allowing them to use a memory interface to access disaggregated memory could potentially yield better performance than accessing a storage layer via a storage interface as in today's serverless systems.
% \zhiyuan{Tightly connected components can avoid communication and computational overhead introduced by restructuring application into resource limited functions.}
Together, the first two features improve {\em resource efficiency}, and the latter two improve {\em performance}.
% \zhiyuan{Together improves {\em resource efficiency}, and {\em performance}.}
%essentially lifting today's FaaS function resource limits.
%, thereby saving the total cost to run the application.
%Right-sizing resources for different phases of an application results in less total resources and thus lower cost.
%For example, if the initial phase of an application uses a huge data structure, the next phase uses only a few variables, and the last phase uses a median-sized data structure, we could use a huge memory component, no memory component, and a median-sized component for these phases while using a single compute component for the entire duration.
%In contrast, today's FaaS would use one function with huge memory for the entire duration.
%As a result, disaggregation reduces the total resource consumption and thus user costs.
%Finally, because components can have different lifetimes, applications can decouple the lifetime of data (memory components) from computation (compute components). %and use the memory component interface to easily manage intermediate data. 
%For example, a memory component representing intermediate data can live from the start of its first producer to the end of its last consumer.

\zhiyuan{Merge this part to execution. should we follow the same structure here? (profiling, compiling, execution)}
\boldunderpara{Aggregation.} Despite its benefits,
disaggregation inevitably incurs increased network communication.
% network communication is intrinsic to disaggregation can affect performance.
%This problem could become more severe when users unnecessarily split their applications into very fine-grained pieces. 
Moreover, when disaggregating an application into smaller units, each of them could potentially incur scheduling and startup overhead.
%The overhead of both items could be significant in a serverless setting.
To reduce or eliminate these overheads, our second idea is to merge, or {\em aggregate}, components and when possible, run them together in a {\em balanced pool}, where each server is equipped with similar amounts of CPU and memory resources.
Aggregated components can run locally
% in one execution environment
in one environment on one server, avoiding the network communication overhead, startup time, and scheduling burden.
%Aggregation can go beyond even what today's single-function limit, allowing the merging of potentially several functions in a DAG.
%They can also be scheduled and launched as one unit, reducing the system overhead.

%Overall, disaggregation allows an serverless application to be executed in fine granularity thereby being \textbf{more resource efficient \zhiyuan{and solve resource-related performance problem}} than today's serverless solutions. Aggregation allows an application to go beyond the limit of today's FaaS functions thereby avoiding the otherwise needed network communication and \textbf{improving performance}. \zhiyuan{improve performance overhead introduced by disaggregation?}

\fi

\if 0
Both disaggregation and aggregation bring new challenges under the serverless computing setting.
First, disaggregation inevitably introduces more inter-component communication. Such communication needs to sustain much higher load and achieve much lower latency than today's function-to-function communication.
Second, an component should be elastic and auto-scaled.
Third, the startup time of components could have a bigger impact on application performance when components run shorter than typical traditional functions.
Unfortunately, none of today's serverless computing platforms are designed or can properly handle disaggregation and aggregation.

\boldunderpara{\sys.} We built {\em \sys} ({\em Serverless Computing with Aggregation and Disaggregation}), a resource-centric serverless computing framework that dynamically aggregates and disaggregates components based on resource utilization and application behavior. 
Users can port their applications to \sys by annotating the original programs %(\eg, adding split points in a program) 
or by using libraries that \sys provides. %(\eg, a remote-memory-based NumPy library). 
Under the hood, our compiler and libraries map user applications to a component-based interface that \sys\ executes.
\sys\ can run all applications supported by today's serverless platforms and many that are not. %\yiying{not very sure if this is the best way to say it..}
Applications whose resource usage patterns vary during the execution
% whose usage patterns are input-dependent,
and/or use vast amounts of resources can especially benefit from \sys.
% \zhiyuan{Changed here}
%\yiying{give some example applications here?} \zhiyuan{i'd say do not emphysis on phases here? Programs suffers limited, coupled and variance resource usage patterns can especially benefit from \sys.}

Despite these many benefits, disaggregation and aggregation in a serverless setting bring two major challenges.
%in resource scaling and component management, as elaborated below: 

%Different from traditional disaggregation systems, in the serverless setting, \sys\ needs to not only disaggregate resources based on new criteria but also efficiently start and automatically scale the disaggregated components.
%Moreover, \sys\ should dynamically disaggregate and aggregate components in an efficient and adaptive manner.
%Making disaggregation and aggregation work in a serverless setting is not easy, as every disaggregated component needs to start up quickly and automatically adapt to changes in resource demands (\ie, auto-scaling).
%Moreover, disaggregated components need to communicate efficiently. 
%Moreover, as \sys\ allows users to define components, inevitably user definitions can be imprecise or even wrong. 
%For example, a user may split their application into too fine-grained components. 
%Often times an application’s resource features are highly
%dependent on input and cannot be pre-determined. Thus, \sys\ should be able to {\em morph} an resource graph into different shapes by disaggregating and aggregating different components dynamically.
%To achieve these goals, \sys\ follows two design principles.
%Although resource disaggregation and serverless computing are each fairly well understood, it is 
%\hx{The following two paragraphs need more work; they do not read smoothly along the flow. How is it related to disaggregation/aggregation?  We shouldn't create another branch that is off of the main presentation flow.  Can we not talk about ``ideas'' again? We already talked two main ideas before.  All we need to do in this paragraph is to show how \sys instantiates these two ideas rather than introducing new ideas. }
%\hx{Relate each of these principles to the big picture of aggregation/disaggregation. For example, ``to efficiently implement aggregation/disaggregation, \sys uses two design principles'' or something like that. It is hard for me to see the transitioning/relationship. }

First, \emph{how to deal with dynamic resource scaling and aggregation that components must undertake} at the run time to achieve our targeted performance and resource benefits. For instance, a memory component may contain an array that grows dynamically, possibly requiring space beyond what the server that hosts it can offer. As another example, \sys\ may need to aggregate a compute and a memory component to improve their communication performance. To enable flexible resource adjustment, we decouple {\em virtual} and {\em physical} components. Virtual components, which capture application features and are generated statically by compilers, remain unchanged throughout the execution. Physical components, on the contrary, are dynamically added, released, or merged at run time in response to load changes. As a result, there can be one-to-one, one-to-many, or many-to-one relationships between virtual and physical components. These relationships are managed dynamically by \sys, enabling elasticity in a straightforward manner. 
%A virtual component can be {\em materialized} to one or more physical components at runtime.
%These physical components can be dynamically added or removed based on load changes, and they can exist on different servers.
%Meanwhile, multiple virtual components could also be aggregated and executed as one physical unit.
%The location, amount, and even the existence of physical components are hidden from the user.
%For example, a virtual memory component could be materialized as multiple physical memory components that potentially sit on different servers,
%while multiple virtual components could also be aggregated and executed as one physical memory.
%This decoupling allows \sys's runtime system to make different scheduling and execution choices while preserving application-specific features. 
%Moreover, it enables the dynamic elasticity of components.
%This decoupling is possible due to the serverless computing model: users supply application code and leave the provisioning and execution to providers.

Second, \emph{how to efficiently handle the two relationships in resource graphs: data communication and task triggering}.
Different from traditional disaggregation systems which focus on optimizing the run-time communication performance (data plane),
in a serverless setting, we also need to efficiently start up the communication across {\em dynamically instantiated} components (control plane).
We build an RDMA-based communication system that judiciously exploits an indirect channel for connection setup, while allowing direct component-to-component communication after the setup.
Different from today's serverless task-flow systems, our resource graph can contain many more components, demanding efficient scheduling and failure handling.
We propose a two-level scheduling system that launches components in a just-in-time, asynchronous, and reliable manner.
%\sys's second design principle is to decouple the {\em data flow} from the {\em task flow}.
%A data flow captures how data is accessed or transferred across components, while a task flow captures how components trigger the start of other components.
%\sys\ separates the design of data flow and task flow, with the former targeting fast, direct communication and the latter targeting fast startup and fault tolerance.
%For example, we implemented an RDMA-based component-to-component communication system for the data flow
%and a two-level scheduling system that launches components in a pre-warmed, asynchronous, and reliable manner. 
\fi


\if 0
Overall, this paper makes the following contributions:

\vspace{-\topsep}
\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
    \myitemit{The identification of various resource-related limitations of today's FaaS-based serverless computing.}
    \myitemit{The proposal of resource-centric serverless computing.}
    \myitemit{The first system that integrates serverless computing with resource disaggregation, with solutions like aggregation to make the integration practical.}
    \myitemit{A demonstration of how to decouple data and task flows.}
%    \myitemit{Solutions like aggregation to make disaggregation practical.}
%    \myitemit{The implementation and evaluation of \sys.}
     \myitemit{New scheduling and component launching mechanisms and policies designed for resource-centric serverless computing.}
     \myitemit{An RDMA-based, transparently virtualized, direct communication system that could be used in serverless settings beyond resource-centric serverless computing.}
    \myitemit{A demonstration of how to make applications written in managed languages like Python performant in a disaggregated serverless environment.}
    \myitemit{Three serverless computing applications ported to \sys.}
\end{itemize}

%We will make \sys\ publicly available upon the publication of this paper.
\fi


==> intro-zhiyuan2.tex <==
\section{Introduction}
\label{sec:intro}

Serverless computing, commonly offered as Function-as-a-Service (FaaS), is a cloud service that allows users to deploy and execute their applications without managing servers.
Serverless computing has gained tremendous popularity in the past few years thanks to its benefit of minimal IT burdens, pay-per-use pricing, and automatic scaling (auto-scaling)~\cite{serverless-growth-1,serverless-growth-2}.

Initially, serverless computing was designed for running short, small-scale functions like simple HTML serving. 
In recent years, there has been an increasing desire to run large, complex applications such as video processing~\cite{excamera,ao2018sprocket},
scientific computing~\cite{numpywren,serverlessseqcompar19}, machine-learning tasks~\cite{carreira2019cirrus,AWS-SageMaker-Serverless,Azure-ML-Training-Serverless}, data analytics~\cite{Databricks-SQL-Serverless,AWS-Redshift-Serverless}, and relational databases~\cite{AWS-Aurora-Serverless,Azure-SQL-Serverless-Announce} in a serverless style, as these applications are also event-triggered and can benefit from pay-per-use pricing, auto-scaling, and reduced IT burdens. These applications 1) run longer or consume more memory than typical FaaS function size limits, 2) exhibit resource usage variations across different phases of computation, 3) require different amounts of resources with different inputs.
We call serverless applications with one or more of these features {\em bulky serverless applications}, or bulky applications for short.

Today's practice of running bulky applications in a serverless style is function DAGs~\cite{AWS-Step-Functions,jonas2017occupy_pywren,excamera,azure_durable_functions,OpenWhisk-composer,zhang2020kappa,gg}, where users construct a DAG of functions and set the size of each function in the DAG. This approach creates several resource-waste and performance issues.
First, a function's size is fixed across invocations. Yet, under different inputs,
%to a bulky application often have different resource requirements~\cite{bilal2021,mvondo2021ofc}, resulting in 
there will be resource waste if provisioning for peak input usage or application failure if under-provisioning.
Second, different functions in a DAG execute in different environments (\eg, containers on one server or different servers). \noteyiying{need ref for this}
Communicating between and setting up the environments can become a major performance overhead, especially when breaking a bulky application into many functions.
On the other hand, reducing the number of environments by making functions bigger would cause resource waste, as a function has the same resource allocation throughout its execution; resources allocated for the peak execution needs are wasted during non-peak time of the function.
Finally, functions in a DAG store intermediate and shared data in a disaggregated layer, usually over a key-value-like interface~\cite{klimovic2018pocket,XXX}.
Accessing such a layer causes performance overhead due to network communication and data serialization.
The root cause of these issues is today's \textit{function-centric} serverless model, where the size and boundary of a function do not adapt to application workloads or hardware resource availability.


\input{fig-faasraas}

\input{fig-overall}

To address these issues, we propose an \textbf{\textit{adaptive, resource-centric}} serverless model,
%The main idea behind \sys\ is \textbf{\textit{adaptive serverless}}, 
where the resource allocation and execution of a bulky application adapts to its {\em internal} resource requirements and cluster resource availability (Figure~\ref{fig-faasraas}).
\notezhiyuan{detailed approach?}
For example, an application can execute in its entirety in one container process if a server can meet all its resource needs throughout one invocation. When its memory need increases, it could autoscale memory only and utilize free memory resource on another server.
For another invocation, it can be executed as two containers on two servers accessing memory on a third server followed by ten parallel executions of a task on five servers. Such adaptation is fully automated with the goal of minimizing resource waste and performance overhead. \noteyiying{last sentence can be improved}
\notezhiyuan{Auto scale at runtime}

Following this model, we build \textbf{\textit{\sys}}, a serverless platform designed for bulky applications. \sys several key challenges to bring the model into reality:

The first one is \textit{identified the resources that have unique features.}
Instead of imposing runtime monitoring overhead and reacting to every resource change in an on-demand way, our solution is to capture as many resource features prior to the execution as possible, with a combination of user hints and coarse-grained profiling history.
Users submit monolithic programs to \sys\ instead of function DAGs,
and express where resource changes may happen by annotating their source programs and using \sys's library; profiling history guides the resource amounts within each unchanged phase.
Internally, \sys\ records these pieces of prior information in an intermediate representation we propose called {\em resource graph}, as shown in Figure~\ref{fig-overall}.

The second one is \textit{how to adaptively schedule and execute a program in different forms.}
\sys achieves this by decomposing the program into components and dynamically generating and composing them at runtime. In this process, the communication of each piece is transformed adaptively using a compiler.
When \sys\ schedules a part of or the whole application in one execution environment, all computation and memory accesses are native (\eg, unmodified memory instructions). \sys\ may also schedule data objects apart from the computation (when memory resources on a server are limited) on a different server. In this case, memory accesses are automatically transferred into network communication. Similarly, \sys\ may schedule different parts of an application's computation as parallel instances or subsequent invocations on one or multiple servers, and it automatically determines the total CPU cores to use. Different computation parts could communicate as normal function calls or as \sys remote invocations, depending on their locations.
\sys\ uses a locality-based, greedy policy: it tries to co-locate computation and memory as much as possible, first in one server, multiple servers within a rack, and finally across racks. The scheduling policy is also used when resource features change during an application's invocation.

The last one is \textit{how to reduce the overhead of fine-grained, resource-level scalng.}
\sys's solution is to proactively schedule and execution even before the resource change happens. By knowing the allocation and scaling patterns from a combination of user hints and coarse-grained profiling history, \sys apply proactive scheduling decisions (\eg best effort resource reservation for future scaling and execution) and execution optimizations (\eg just-in-time prestart), \sys\ largely reduces the difficulty of runtime scaling and avoids the performance overhead.

% An immediate question that follows is how to capture resource features and their changes within an application's invocation and across invocations.
% Instead of imposing runtime monitoring overhead and reacting to every resource change in an on-demand way, our solution is to capture as many resource features prior to the execution as possible, with a combination of user hints and coarse-grained profiling history.
% Users express where resource changes may happen by annotating their source programs and using \sys's library; profiling history guides the resource amounts within each unchanged phase.
% Internally, \sys\ record these pieces of prior information as a {\em resource graph}, as shown in Figure~\ref{fig-overall}. At runtime, \sys\ makes {\em proactive} resource scheduling decisions based on an application's resource graph and cluster resource availability. \sys\ handles inaccurate prior knowledge by making on-demand resource adjustments. Compared to a pure on-demand approach, \sys\ largely avoids the performance overhead of execution- and network-environment setup.

On top of the above adaptive and proactive approaches, \sys\ further reduces performance overhead by asynchronously setting up execution and network communication environments before they are needed; it improves scalability with a two-level scheduling mechanism; and it handles failure by partial re-execution of failed components and consistency by providing synchronization primitives.
%\sys\ first tries to execute a bulky application as one process in a single server. When no single server can host it, \sys\ executes it on multiple servers. As the application's resource needs change throughout its execution, \sys\ decreases or increases the corresponding amount on the same server(s) if possible. However, increasing CPU or memory resources on a server is not always possible. In this case, \sys\ launches increased computing or memory resources on another server while maintaining the already launched resources at the initial server to avoid migration costs. If no single server can host the added resources, \sys\ allocates the needed resources from multiple servers.

%Adaptive serverless executes bulky applications in a resource-efficient and, thus, cost-efficient way. However, several key technical challenges must be solved to make this approach viable. 


%Finally, good application performance requires proper run-time support at different layers. At the scheduling layer, \sys\ employs a two-level scheduler architecture that performs coarse-grained scheduling at a global node and fine-grained allocation at the rack and server level. \sys\ adopts a {\em just-in-time} scheduling policy that makes scheduling and execution decisions just before the resources are needed. 
%of a component and launches it when its previous component is running. For compute components, \sys\ performs automatic CPU and memory scaling in an on-demand and transparent fashion. For data accesses and data components, \sys\ compiles a native and an API-based remote version for the \sys\ scheduler to choose between quickly, and we allocate local or remote memory space in an adaptive and auto-scaled way. 
%For memory accesses, \sys\ supports and dynamically chooses native local memory accesses, object-based remote memory accesses, and transparent remote memory swapping.
%For network communication, we propose a new control plane for fast connection establishment in a serverless style. Finally, \sys\ handles failure by partial re-execution of failed components and consistency by providing synchronization primitives.

We evaluate \sys\ with a set of microbenchmarks and three real-world applications: data analytics queries from the TPC-DS benchmark, video processing pipelines, and a machine-learning task,
We compared \sys\ to two FaaS frameworks (OpenWhisk~\cite{OpenWhisk}, AWS Lambda~\cite{AWS-Lambda}), four serverless DAG frameworks (AWS Step Functions~\cite{AWS-Step-Functions}, PyWren~\cite{jonas2017occupy_pywren}, ExCamera~\cite{excamera}, gg~\cite{fouladi2019laptop}), one serverless resource tuning system (Orion~\cite{Orion-osdi22}), and two VM-based execution methods (remote-memory swapping~\cite{FastSwap}, VM migration~\cite{XXX}).
Our machine-learning results show that \sys\ reduces resource consumption by 40\% to 84\% compared to OpenWhisk while only adding 1.3\% performance overhead.
Our TPC-DS results show that \sys\ reduces resource consumption by 73\% to 85\% and improves performance by 54\% to 64\% compared to PyWren.
Our video process results show that \sys\ reduces resource consumption by 33\% to 90\% and improves performance by 33\% to 47\% compared to gg on Openwhisk.

We will make \sys\ publicly available upon acceptance.


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Serverless computing, commonly offered in the form of FaaS (Function-as-a-Service), is a type of cloud service that allows users to deploy and execute their application programs (\ie, functions) without managing servers.
%(or more specifically, any software or hardware infrastructures beneath their applications).
%Initially introduced for cloud providers to exploit unused data-center resources, 
Serverless computing has quickly gained huge popularity in recent years because of its benefits to cloud users: minimal IT burdens 
%to focus on their core business products 
and paying for only when their applications are triggered.

Despite the many benefits, today's FaaS-based serverless computing still has several key limitations.
%and we believe that they are major reasons that prevent serverless computing from enabling a richer set of applications.
First, there are only few fixed CPU-to-memory ratios that users can choose, but user workloads can have many different CPU and memory usages.
As a result, either some CPU or some memory resource is wasted~\cite{arxiv}.
Second, a function's resource amount is fixed across invocations, but different input to a function could result in different resource needs~\cite{arxiv}.
This lack of elasticity would result in function failure in the worst case when some invocations exceed the preset per-function resource amount.
%, \eg, Google Cloud Functions offer six combinations of CPU frequency and memory sizes
Third, all resources must be allocated and deallocated at the same time even if they exhibit different lifetimes.
On one hand, a function needs to be provisioned with the peak resource use, but not the entire function needs to use the peak amount. 
As a result, either the cloud provider~\cite{azure_functions_pricing} or the user needs to pay for the unused resources~\cite{aws_lambda_pricing,google_functions_pricing}. %, because cloud providers cannot easily exploit the unused resources.
On the other hand, certain resources such as intermediate data cannot live beyond the execution of a function, 
which makes sharing them across functions harder~\cite{klimovic2018pocket,sreekanti2020cloudburst}.
Finally, the amount of resources a function can use is limited.
%For example, AWS Lambda~\cite{XXX} limits each function to use at most 10\GB\ of memory and run for at most 15 minutes.
Resource limits force users to rewrite their large-scale applications like data analytics as smaller pieces that are small enough to fit in a function
and/or to use an external service to host its extra resource need. 


Our observation is that the root cause of these limitations is today's ``function-centric'' serverless model.
%A function is a fix-sized box defined by the cloud provider,
%and cloud users have to adapt their applications into these provider-defined functions, 
%usually with performance loss, increased cost, and developmental cost.
%We argue that a better serverless computing model should work towards user applications, not the other way round.
%
A function is a rigid, fix-sized box that couples CPU and memory resources and is allocated, scheduled, terminated, and billed as an inseparable unit.
Meanwhile, different functions are completely separated from each other, and their communication has to resort to another service like S3 or Redis.
This function-based model leaves users with a dilemma:
either pack more functionalities in a large ``function box'' to avoid function communication cost but pay for unused resources 
or split functionalities into small boxes to achieve more fine-grained resource utilization but incur high function-communication performance overhead.
Moreover, neither option is always possible, as even the largest function size will not be able to host large applications in their entirety,
and many applications cannot be properly split into small pieces as a task flow (which is what today's serverless orchestration cloud services take).

To solve the above dilemma and many issues of today's function-based serverless computing, a natural solution is to get rid of the rigid function model.
\textit{How can we then represent and execute user applications in a serverless manner?}

In this paper, we explore two ideas, {\em disaggregation} and {\em aggregation}, and build a system called {\em \sys} as a demonstration of how next-generation serverless computing could be ``resource centric''.

Our first idea is to disaggregate serverless applications into {\em element}s, each representing a piece of application code or data structure and 
has a distinct triad, \textit{$<$resource type, resource amount, lifetime$>$}.
An element is the unit of scheduling, execution, and auto-scaling, and elements with different resource types run on different disaggregated resource pools. For example, a CPU (compute) element runs in a CPU (compute) pool, and a memory element runs in a memory pool.
In this paper, we focus on the serverless system layer and assume that disaggregated pools are built and managed by the cloud provider; 
they could use physically separate server pools~\cite{FACEBOOK-BRYCECANYON,XXX}, virtual pools that physically live on the same set of servers~\cite{FaRM}, or dedicated hardware device pools~\cite{Clio}. \zacb{I think the last few sentences focus too much on implementation details and could be left to a later section in the paper}
Elements of an application form a graph, which represents both the task flow and the data flow. 
One element can trigger one or more elements (\ie, task flow) and multiple elements running at the same time can communicate with each other (\ie, data flow). 
Users supply element graphs to \sys, with an easy-to-use interface \sys\ provides (we discuss how users could potentially generate elements, with some of \sys's compiler support in \S\ref{XXX}).

The disaggregation scheme has several key benefits to serverless computing. 
First, it enables the independent scaling of different resource types, thereby allowing arbitrary resource ratio (\eg, CPU-to-memory size ratio). 
Second, when pooling resources together, applications can allocate as much resource as needed for any element, essentially lifting today's FaaS function resource limits.
Third, multiple elements can be used to capture resource consumption changes in a user application.
For example, if the initial phase of an application uses a huge data structure, the next phase uses only a few variables, and the last phase uses a medium-sized data structure, we could use a huge memory element, no memory element, and a median-sized element for these phases while using a single compute element for the entire duration.
In contrast, today's FaaS would use one function with huge memory for the entire duration.
As a result, disaggregation reduces the total resource consumption and thus user costs.
Finally, because different elements can have different lifetimes, applications can decouple the lifetime of data (memory elements) from computation (compute elements) and use the memory element interface to easily manage intermediate data. 
For example, a memory element representing intermediate data could live from its first producer starts until its consumers have all finished.

Despite its benefits, disaggregation raises several key technical challenges. 
First, elements could be smaller than typical serverless functions today, resulting in huge amounts of (small) elements in an element graph and putting scalability and performance pressure on the scheduling and element-launching system.
Second, the startup time of elements could have a bigger impact on application performance when elements run shorter than typical traditional functions.
Second, an element could be larger than today's per-function quota and potentially exceeding the capacity of the server it runs on.
Finally, inter-element communication could be a lot more intensive and demand much lower latency than today's serverless systems.
For example, a compute element could frequently access a memory element and expect such accesses to be close to native memory performance.

We propose a set of techniques to confront these challenges from several perspectives.
For the scheduling system, we propose a locality-aware and resource-pool-aware scheduling system that schedules elements as close to each other as possible if they have high communication need.
%We organize the scheduler itself as a two-level distributed system to make the scheduling more scalable. \zacb{As discussed in previous meetings, it's not really more "scalable" than other schedulers, so we can probably leave this sentence out.}
In addition, to launch elements as fast as possible, we propose a pre-warming mechanism that warms up the execution environment for each element in an ``almost just-in-time'' manner.

For the run-time system, we develop an RDMA-based direct element-to-element communication system.
On top of it, we build a library that transparently caches remote memory data locally and performs serialization and deserialization. 
To efficiently launch and execute memory elements, we propose to use a single execution environment for all memory elements on a physical server and to isolate them into different RDMA protection domains. \yiying{Zhiyuan, true about RDMA PD?}
We auto-scale memory elements by allocating more {\em physical} memory chunks for a remote memory element when its size grows.
The allocation and accessing of multiple memory chunks are all transparent to user applications, and different memory chunks can sit on different physical servers, thereby allowing user applications to use as large memory as they want.
We also transparently track the lifetime of elements and terminate them when their lifetime end.
\yiying{Zhiyuan, need to talk to you to see what exactly you did in the runtime system.}

Despite disaggregation's various benefits and our solutions to its technical challenges, certain performance loss is still inevitable when there are many elements that communicate with each other frequently.
To solve this problem, our second idea is to merge, or {\em aggregate}, elements.
Specifically, we transparently merge compute and memory elements that suffer from high communication performance overhead into one execution environment that run on a \textit{server pool}.
The server pool does not disaggregate different types of resources, and each server has both beefy CPU and ample memory.

To fully exploit the benefits of element aggregation while hiding its complexity from user applications, we developed new run-time and compiler support.
The run-time system transparently executes two elements in a single container and converts remote accesses to local ones, while the compiler merges multiple elements' code into one which is then executed as any other elements.

To decide when and what to aggregate/disaggregate, we design a policy based on the utilization of each resource pool, the performance overhead of element communication, and element resource utilization.
%merge same lifetime
We also developed a monitoring system to collect per-element run-time profiles.
We design our policy and monitoring to be simple and lightweight. 
As a tradeoff, at runtime, an element could use more resources than the prediction.
In worst case, an element can use more memory than what the server hosting it has.
To handle such cases, we developed a user-space swap system to transparently swap not-recently-used local memory to the remote memory pool.

We implemented \sys\ on top of OpenWhisk~\cite{OpenWhisk}.
%Currently, \sys\ only supports Python, but our approach could be easily extended to other languages.
We evaluated \sys\ with a set of microbenchmarks and three real-world applications: simple machine-learning training, distributed query with the TPC-DS benchmark, and video processing.
We compared \sys\ with vanilla OpenWhisk, AWS Lambda, AWS Step Functions~\cite{AWS-Step-Functions}, and PyWren~\cite{jonas2017occupy_pywren}.
Our real-workload evaluation results demonstrate that \sys\ could save memory of up to 1.96\X\ while improving performance by up to 28\% compared to existing systems.
In addition, \sys\ enables workloads that are larger than today's FaaS limits without any developer involvement.
We will make \sys\ publicly available upon the publication of this paper.
% Serverless computing is a new type of cloud service that has gained a lot of traction recently. The main idea of serverless computing is to free cloud users from managing servers so that they could focus on their core business logic. Because of this, more types of (non-IT) users could now enjoy cloud computing.

%Serverless computing is a recent computing paradigm introduced and now supported by most major public cloud providers. Serverless computing, as the name suggests, removes the need for cloud users to manage virtualized operating systems infrastructure. This allows companies to focus less on the infrastructure challenge of operating their services and more on the features that they provide to the users. Another positive consequence of serverless computing is more efficient billing and resource utilization. Instead of needing to allocate computing cores and memory which may go unused due to patterns in user activity \cite{liu2011measurement} serverless users are billed only when requests to applications are received and for the resources used while processing the request. One more benefit of serverless computing is the ability for cloud providers to have more efficient scheduling and placement policies of applications which can more effectively use the resources within the data center.

%As promising as the serverless paradigm may seem it is not without its drawbacks. There are a few main limitations which prevent more users from shifting their applications to serverless infrastructure. First is that current serverless offerings from cloud providers such as AWS, Google Cloud, and Microsoft Azure all limit serverless application functions to relatively small amounts of computing resources. Typically no more than a few cores and generally less than 15GiB of memory. These values are far less than what is available in traditional reserved virtual machine offerings. Second is that serverless functions are not designed for storing state between function invocations. They are supposed to be designed in a stateless way to offer easy horizontal scaling, but this places limits on the types of applications which may be converted to serverless workloads. Lastly, serverless functions are not designed to communicate directly between one another. This results in high communication latencies between chains of serverless functions that may make up larger processing pipelines.

%In this work we aim to solve the hardware resource limitation and communication latency issues of serverless computing by proposing a new end-to-end architecture for serverless functions to run on disaggregated hardware. This work presents the system and performs an in-depth performance analysis to show the feasibility of such an architecture and why serverless is a good fit for disaggregated platforms.

==> network.tex <==
\subsection{Component Network Communication}
\label{sec:communication}

As communicating or accessing components in a resource graph can sit on different servers especially in a highly utilized rack, it is crucial to ensure that both the actual communication (data plane) and the connection set up (control plane) are fast.
We suppport both RDMA and TCP communication, with several optimizations at the control path and the data path. %Below, we explain these optimizations, with the Appendix present our detailed RDMA implementation. Most of the optimizations except for zero copy apply to TCP as well.
Similar to existing remote-memory works~\cite{Mira}, we optimize the data path by batching small network requests and by caching fetched data locally. For RDMA, we perform one-sided, zero-copy communication\noteyiying{true?}.

The communication control-path optimization is unique to serverless computing, as we need to minimize network connection set up time, while allowing the direct communication between components in the data plane. 
The general challenge in serverless communication is that a function cannot easily know where other functions are.
Prior serverless communication systems rely on an overlay network to build connections~\cite{thomas2020particle}) or pre-establishes connections between all pairs of endpoints~\cite{copik2021rfaas,wei2022booting,wei2021krcore,mohan2019agile}. The former is slow while the latter does not meet our resource elasticity goal. Both try to establish connections via {\em direct} channels between two nodes.

Our idea is to leverage {\em non-direct but already established} connections to assist the initial location discovery.
Our observation is that a component has always established a connection with its rack-level scheduler by the time when it starts up.
Moreover, the scheduler is the one that decides and thus knows the physical locations of the two components that will be communicating. % (\ie, communicating relationship in the component graph).
We let the scheduler send one component's physical location (in the form of executor ID) to its communicating component's {\em network virtualization controller} when initiating the two components.
With the location information, the two components can easily establish a datapath connection (\eg, RDMA QP).
To further optimize the startup performance, we initiate the location exchange process as soon as the execution environment is ready, while user code is loaded in parallel. Doing so hides the location-exchange overhead behind the performance-critical path (Figure~\ref{fig-launch}).


==> offline.tex <==
\subsection{\sys\ Offline Component}

The offline component of \sys\ consists of a fine-grained profiler (\S\ref{sec:dryrun}) and a compiler (\S\ref{sec:compiler}). 
The top half of Figure~\ref{fig-workflow} illustrates the workflow of the offline component.

Given a user program, our offline analysis first attempts to perform \emph{vertical partitioning}, which turns \emph{thread-level} parallelism into \emph{element-level} parallelism. 
Next, \sys\ uses a dry run, where the user program is executed with representative inputs provided by the online component, to profile the program and understand how memory utilization changes as the execution progresses. The profiling results are analyzed to identify a set of \emph{stages}. 
Within each stage, memory utilization is \emph{relatively stable}, but different stages may use drastically different amounts of memory.  
\sys\ feeds these stages to our compiler, which automatically performs \emph{horizontal partitioning} of the program by generating a new logical element for each stage. While vertical partitioning focuses on parallelism (\ie, better utilize CPU resources), horizontal partitioning is done with respect to memory utilization, enabling a precise understanding of the amount of memory to allocate for each stage and making each stage amenable to fine-grained resource allocation and management. 

Note that the entire offline component of \sys\ is pluggable and optional.
Users could also manually insert cut points (by annotating their programs) for \sys\ to generate elements to be used by the \sys\ online system. Users could also follow the same idea to develop  offline components for other languages.

\zhiyuan{Profiling and Identification of Logical Elements}

\subsubsection{Dry Run Profiling and Adaptive Repartitioning}
\label{sec:dryrun}

\zhiyuan{\textbf{1. identifying resource usage stages using dry run}}
\rcsc's benefits rely on the knowledge of resource utilization at different stages of a user program.
Fine-grained profiling tools like \fixme{XXX} are able to generate detailed (\eg, per program statement) resource usages.
However, they all add significant performance overhead to the program execution.
Our idea is to perform offline {\em dry runs} to collect fine-grained profiles.
These dry runs execute on bare-metal (beefy) servers\footnote{In the rare case where a user program's vertical partition requires more resources than what a single server can provide, we run it with memory swap enabled.} and are completely separate from real (online) program execution.

\sys\ performs the initial dry run in the deployment phase (\ie, when users ship their programs to the provider) using input that users supply (\eg, input that users use when testing the program). If no input is provided, \sys\ will skip the initial dry run. \yiying{Harry: is this what we want to say about the initial dry run and its input?}
After real execution starts, \sys\ performs more dry runs on a need base.
We will discuss the criteria \sys's online component uses to trigger dry runs in \S\ref{sec:profiling}.
%\harry{The only thing missing here is when to redo a dry run. I'll write it later once we have a more concrete idea. }


For each dry run, we execute the user program on top of a fine-grained profiler~\cite{XXX}, which reports CPU and memory utilization per line of source code. 
We analyze these profiles to identify lines that contribute to a significant change in memory consumption. 
 For example, if the memory usage at Line \texttt{i+1} is $> N\times$ (or $< \frac{1}{N}$) of that at Line \texttt{i} (where $N$ is a system parameter), a new stage starts at Line \texttt{i+1}. At the end of the dry run, a set of \emph{stage-defining code lines} (\ie, stage delimiters) is collected. 

Next, we instrument the program by inserting, at each stage-defining line, a function call that dumps the call stack when that line is executed (\eg, \texttt{main}$\rightarrow$\texttt{foo}$\rightarrow$\texttt{bar}). We run the instrumented program again and collect a set of \emph{stack traces}, each (together with the line number) defining the boundary of a stage.  Since a function can be invoked in multiple contexts (\eg, \texttt{bar} can be invoked by \texttt{foo} or another function), a stack trace can \emph{uniquely} identify an execution point, which provides a basis for the compiler to perform horizontal partitioning (\S\ref{sec:compiler}). 
%Given a stack trace, the compiler inlines all functions in the user program, find the program location corresponding to the stack trace (\ie, breaking point), and split the program at the location; details of this process can be found in \S\ref{subsec:compiler}.  

A major challenge here is that program behavior and resource utilization depend on inputs, which may, however, drastically change as the execution progresses, thereby invalidating the initial partitioning. 
%Consequently, running the initially generated elements can lead to inferior performance. For example, if the memory consumption of a compute element grows beyond its memory capacity, frequent swaps would result and performance would degrade significantly.  
To make matters worse, the requirement of high efficiency in real executions precludes any heavyweight profiling (such as the dry run), making it hard for us to collect new stack traces and repartition the program.  

To solve the problem, we leverage  dry runs to generate more breaking points (and stack traces) than we use to partition the program, so that these additional stack traces can be used for repartitioning during real executions. In particular, we use two system parameters $N_1$ and $N_2$ in our dry run (where $N_1 < N_2$) to identify breaking points (stages). The first set of breaking points, which we refer to as \emph{logical points}, is identified with $N_1$, while the second set, referred to as \emph{physical points}, is identified with $N_2$. It is clear that the first set is a \emph{superset} of the second due to $N_1 < N_2$; each physical point is also a logical point but not vice versa. We use the same instrumentation approach to collect a stack trace at each logical point. 

Our idea is to partition the program initially based on physical points (representing coarser-grained stages) while leveraging logical points (representing finer-grained stages) for repartitioning during the execution (because stack traces for all logical points have been generated during the dry run and are available to use throughout the execution). In particular, at the time our compiler splits the program using the stack traces corresponding to physical points, it inserts an API call, \texttt{pull\_stat}, to an internal library function at each (non-physical) logical point. This function is used by the online system to determine its strategy to repartition physical elements (\S\ref{sec:profiling}).

\zhiyuan{\textbf{2.identifying dynamic resource usages }}
\zhiyuan{\textbf{3.identifying parallel computes from threads} form next section \textit{Vertical partitioning}}

\zhiyuan{Generating Physical Elements }

\subsubsection{Compiler}
\label{sec:compiler}

\zhiyuan{Our compiler takes the user input programs, and a set of logical elements with estimated }

Our compiler takes as input a DAG of program(s) (or a single program) and a set of stack traces collected by the dry run, turning the program into a DAG of physical elements via vertical and horizontal partitioning. 

\zhiyuan{\textbf{Selecting Physical elements based on resource estimation} <- Move 4.2.6 here} 
\zhiyuan{\textbf{Code Generation} Generate interface code to utilize runtime element apis}

\boldpara{Vertical partitioning} happens before the dry run.
%is done by turning the body of each parallel loop into a separate program. New edges are then added into the DAG to model the new dependence relationships (\ie, this new program is invoked automatically once its input becomes available). 
In particular, if the user program uses parallel loops (which run iterations in parallel), we generate code that turns each iteration of such a loop into a separate program, which is subject to scheduling and resource allocation. However, we do not identify further parallelization opportunities in the user programs\textemdash 
there exists a large body of work~\cite{bondhugula-pldi08,pouchet-popl11,holewinski-pldi13} (mostly in the PL/HPC communities) on parallelizing sequential programs; such techniques are not the focus of this paper and applying them to identify further parallelism opportunities is left to future work. 

\boldpara{Horizontal partitioning.}
After the dry run, with the stack traces, the compiler performs horizontal partitioning. The compiler first \emph{inlines} all functions into the \texttt{main} function. For each stack trace corresponding to a physical cut point, it maps the trace to a unique program location in the inlined program
and generates two sub-programs (\ie, elements), one representing the part before the location and one representing the part after.  

\boldpara{Memory objects.}
Breaking a program introduces cross-element dependencies\textemdash a variable is defined in one element and accessed in multiple elements. 
To safely handle dependencies, we package shared variables as {\em memory object}s which our online system places in shared, remote memory.
%is placed in shared, remote memory to enable accesses from both sides. 
To properly access memory objects, our compiler generates a \emph{prologue} at the beginning of each element and an \emph{epilogue} at the end.  The prologue contains a set of code statements that read values from the memory element for the element to access.
%for variables that are used but not defined in the element. 
Conversely, the epilogue contains statements that write values to remote for variables that are modified in this element and used by other elements. 

In addition to memory objects created to handle physical element dependencies, \sys\ identifies data structures that are fit for placing into memory objects running remotely.
For example, a large data structure that is not accessed frequently (\eg, the results of mappers in a MapReduce-style program) could be placed into a memory object to reduce the memory consumption of the element accessing it.
%Findings from recent works in disaggregated memory~\cite{AIFM,Aguilera-FarMemory} could also be used for generating memory objects, and we leave it for future work.
We discuss other use cases of memory objects in \S\ref{sec:memoryelement} and \S\ref{sec:swap}.
Users could also annotate their programs to identify memory objects.
%Such data structures can be \yiying{Zhiyuan, Zerui, Isshan: what's the criteria used by the PL side to generate these memory elements?}
%These read/write statements invoke calls provided by the low-level system to access remote memory via RDMA. Such cross-element dependencies introduce new DAG edges. We add them appropriately to model the input-output relationship between the elements. 


\zhiyuan{\textbf{2. Generating memory elements for swapping to handle memory variance}}

\zhiyuan{\textbf{3. Generating More efficient elements using specialized generator} With access to user code, Specialized code generator can take better utilization of elements. When we detect that we build physical element on a numpy array, we are generating special code to make it zero-copy. Further, for pandas data analysis applications, we will be able to generate code with out-of-core algorithm (ref dask \cite{???})  and utilize the memory object as fast out-of-code memory.

We expected more specialized profilers and code generated to be implemented to make full utilization of elements.}

\boldpara{Final product.}
At the end of the compiler analysis, we generate a new DAG whose nodes are physical elements or memory elements
and whose edges represent dependency relationships (\ie, one element triggering another element) or access relationship (\eg, one element accesses a memory element). We also attach a {\em resource estimation} at each node to represent the estimated resources (CPU cores, memory size) needed by the element at this node. This DAG is then fed to \sys's online system.

%stack trace cut
%inlining
%inserting remote access APIs
%inserting logical cut points library calls
%third-party APIs (\eg, to storage)



==> overview-old.tex <==
\input{fig-workflow}

\input{fig-api}
\input{fig-architecture}


\section{\sys\ Overview}
\label{sec:overview}

This section gives an overview of \sys's usage model and overall design.
Figure~\ref{fig-workflow} illustrates the overall workflow of \sys\ with a simple example.


\subsection{Resource-Based Elements}
\label{sec:elements}

\sys's abstraction and implementation center around the concept of {\em resource-based element}s, or simply, {\em element}s.
Each element has a distinct triad of $<$\textit{resource type, resource amount, lifetime}$>$. 
An element can be a piece of code or a data structure, and our current implementation supports three resource types: compute, memory, and mixed.
A {\em memory element} has no processing (\ie, no instructions) and is usually just one or few data structures. 
A {\em compute element} or a {\em mixed element} is a code piece.
Compute elements are intended to capture compute-heavy program phases that can work with small internal memory. It could and often does access large memory objects (as memory elements), but with less frequency.
Differently, mixed elements frequently access large amounts of memory during their computation and thus are hard to be disaggregated further.
Similar to compute elements, a mixed element can still access other memory elements.
Elements can relate to each other in two ways:
1) one element sends its result to another element, what we call the {\em triggering} relationship,
and 2) two elements have overlapped lifetime and communicate with each other during that time, what we call the {\em communicating} relationship.

\zhiyuan {Scad automatically infers lifetime of elements based on its type and relationship with other elements. The lifetime of a computational element continues to its execution's end. The lifetime of a memory element is controlled with reference counting. All communicating compute elements will hold an reference to a memory element instance. Compute elements will automatically release the reference when its lifetime ends or release it earlier. Memory element starts when any computational elements accessing it start executing and ends when its reference counts goes to zero.

Or we just say "when all communicating elements finishing accessing it", and introducing referencing counting in later sections.
}

\zhiyuan {
\subsection{Programming Model}

Currently, \sys\ can execute Python and Node.js programs, which are the two most commonly used languages in serverless. %Extending \sys\ to other languages is mostly straightforward and we leave it to future work. 
2\sys uses different elements to capture the different resource requirements for a program. Programs are defined as a graph of elements in \sys, whose nodes are different elements and edges are relationships (either communicating or triggering).

Scad’s native interface is a DAG of elements with Scad’s template (written as a JSON file). The template has different fields for computational (compute or mixed) and memory elements (e.g., compute elements have a field to specify location of the code; memory elements don’t have this). The template also lets users specify the relationship between elements (triggering or communicating). A DAG is formed from these relationships. Within each computational element, the user can open a memory element and read/write to it with an offset and a size using APIs \sys\ provide (Figure~\ref{fig-api}).
Different code pieces sharing a memory element simply by opening the same name (memory element name is unique in an element graph).
One computational element can also communicate to other computational elements, via a send/recv interface. 
%Optionally, users could give hints about the initial resource amount of an element (the only hint in Scad’s interface). All our experiments except for Figure13 run without any user hints and use the default resource amount. Figure13 uses hints to set the initial and incremental memory sizes (S4.1.1), which are smaller than the default.

% user programs are not executed.

execution on next section?
}

%To use \sys, users supply a connected graph (Step 1 in Figure~\ref{fig-workflow}) called {\em element graph}, whose vertices are compute, mixed, or memory elements. All the elements users specify and are aware of are virtual elements, and they define the resource type of these elements. 
%Optionally, users can provide hints of resource amount (\eg, CPU cores, memory size) of an element, which \sys\ will use as the initial resource assignment. % and specify its lifetime.
%If no hints are given, \sys\ will automatically scale an element. % and monitoring references for lifetime.
%Directed edges in a graph represent triggering relationship, and undirected edges represent communication relationship. 
%Figure~\ref{fig-api} lists \sys's core memory-accessing APIs.
%On top of the direct memory accessing interface, we provide compiler support for several common high-level language-specific data structures like NumPy arrays.
%Programs written with these data structures can directly work with \sys\ after a few user annotations such as the hint of where to split the code and what data structures to put into remote memory.
%\sys\ compiles such programs into an element graph (Step 1' in Figure~\ref{fig-workflow}). 

\zhiyuan{
\if 0
An easy way to write programs on \sys\ is to separate different stages of an application into different elements.
%(\eg, data loading, data pre-processing, mapping data, reducing data, writing data back).
If a stage is compute heavy, then it should be a compute element. If a stage accesses memory that cannot be easily separated, then it can be a mixed element.
Programmers can then define data that is shared among these elements, large data structures that are infrequently accessed, and data that should live longer than tasks  as memory elements.
\fi
}

\zhiyuan {
On top of the native interface, compiler and tool support could be added to offer a high-level interface that can handle elements generation and accessing based on user semantic, which we expect most users to use. As this work focuses on systems building, we only offer primitive, proof-of-concept compiler and tool support and leave developing comprehensive support to future work.

% annotations are not the most important thing here, we can also do libs?

Compiler support for decomposing an application: We currently support user insertion of ## split to their code (not arbitrary locations, with some restrictions). Scad compiler then splits the program at these split-points into multiple code pieces, each representing a compute element. We turn variables that are shared across split-points into memory elements. There are also other ways to port an application, for example, by mapping a workflow DAG to a Scad element DAG.

Compiler and library support for remote memory accesses: Users can mark a data structure with ## rMem. Scad creates a memory element for it. For these memory elements and for memory elements created in 1, our compiler translates their accesses to Scad remote-memory APIs. We add library support for NumPy arrays and Dataframes to efficiently fetch remote memory to local cache. With these extensions, users do not need to write any of the Scad APIs in Fig4.

Profiling and predicting resource usages: At runtime, Scad captures resource usages which are used to predict future invocations’ usages. These predictions serve as user hints in the native interface.

We believe that writing/porting applications with our high-level interface has similar or lower complexity than writing/porting applications to today’s FaaS interface, as users will also split code into functions and convert local-variable accesses to remote storage accesses.

All our experiments use some of the above extended support. We use split annotations to convert the Logistic-Regression program to a Scad DAG. We convert an original Pywren workflow of TPC-DS to Scad DAG by converting each stage to one compute element and each externalized state (a Dataframe) to a memory element. At runtime, our library translates Dataframe APIs into Scad’s remote-memory APIs.
}

\if 0
\subsection{Design Principles}
\label{sec:principle}

There are several key challenges \sys\ faces. 
First, disaggregation raises new performance challenges both at the data plane (network communication across disaggregated units) and at the control plane (start up multiple disaggregated units), as discussed in \S\ref{sec:disaggregation}.
Second, by letting users define their own element graphs, there is the potential issue of wrong user estimation of their applications' resource features.
For example, a user may split their application into too fine-grained or coarse-grained elements.
They may also underestimate the resource consumption of an element.
Moreover, often times an application's resource features are highly dependent on input and cannot be pre-determined.
Thus, \sys\ needs to dynamically adjust the size and the scope of a user-defined element.

To solve these challenges, we design \sys\ by following two design principles.
The first principle is to decouple users' element view from the materialization of elements.
The abstraction exposed to \sys\ users is {\em virtual elements} (defined in \S\ref{sec:elements}), which users use to capture their applications resource features.
The internal abstraction \sys\ uses for scheduling and execution is {\em physical elements}, which are optimized for run time execution.
The location, amount, and even the existence of physical elements are hidden from the user.
For example, a virtual memory element could be materialized as multiple physical memory elements that potentially sit on different servers,
while multiple virtual elements could also be aggregated and executed as one physical memory.
This decoupling %is the key enabling factor of our disaggregation and aggregation approach, as it 
allows \sys\ run-time system to easily make different materialization choices for an element without the need to involve other elements even when they have communication or dependency relationships.
Moreover, it enables the dynamic elasticity of elements, which is required to solve the second challenge.
We are able to do this decoupling because of the serverless computing service model: users supply application code and allow the providers to execute in any way they want (as long as some performance and cost guarantees are delivered).

The second principle is to separate the data flow from the task flow.
Task flow captures how different computational tasks (\ie, compute elements) trigger each other.
Data flow captures how data is generated, accessed by tasks, and transferred over time.
%Today's serverless computing only allows users to define a task flow and only handles the transmission of task output/input (\eg, AWS Step Functions, Azure Durable Functions).
%As such, users have to use another service such as S3 or Redis for the data flow (\eg, when two functions need to frequently access some data or when some data lives beyond a task's lifetime).  
%\fixme{Need to double check whether or not Durable Functions support some sort of data flow}
\sys\ separates the data flow and the task flow, with the implementation of the former targeting fast, direct communication and the implementation of the latter targeting fast startup and failure handling.
\fi


\subsection{Overall System Architecture}

Figure~\ref{fig-arch} illustrates the overall architecture of \sys.
\sys\ is a data-center-wide solution, with multiple racks working together under a \textit{global monitor} which monitors the resource consumption of each rack and a \textit{global scheduler} which performs coarse-grained scheduling based on per-rack monitored resources.
A global database stores user programs and various \sys\ metadata. %, monitoring and profiling results, and billing information.
Each rack has its own \textit{rack-level scheduler} that performs fine-grained scheduling decisions and orchestrates the execution of user element graphs.

\sys\ supports different types of resource disaggregation implementation.
For example, resource pools could be physically separated where each node in a pool only serves one type of resources (Node 1 and Node 3 in Figure~\ref{fig-arch} only serve for the compute and the memory pool respectively).
Resource pools could also be virtual, in that one node can be part of multiple (virtual) pools, \eg, Node 4 is in a virtual compute pool and a virtual memory pool.
The compute/memory pool executes compute/memory elements respectively.
Different from traditional resource disaggregation architectures, \sys\ also includes a {\em balanced pool}, which runs aggregated elements and mixed elements.
Nodes in this pool (\eg, Node 2) have balanced (similar) amounts of CPU cores and memory.
%By design, a node could be a regular server or a specialized device~\cite{Clio}, although our current implementation is based on regular servers.

\input{tbl-techniques-single-col}

Each node runs an executor that launches and manages elements (\ie, the control plane). 
We build a compute element controller to manage compute and mixed elements and a memory element controller to manage memory elements.
A node can have both compute and memory controllers or either one of them, depending on where the node belongs to one physical pool or two virtual pools.
In addition, we build a thin network virtualization unit to orchestrate the connection establishment of communicating elements.
Each compute/mixed element executes in its own sandbox (\eg, Docker) and sits on top of a \sys\ runtime and a language runtime (for managed languages).
The \sys\ runtime orchestrates remote memory accesses and performs various monitoring tasks.
Memory elements do not have any computation and thus only need access isolation. 
They do not live in traditional sandboxes like containers.
We currently use RDMA memory regions (MRs) for this isolation purpose. 
A memory element is a virtual concept and can include multiple \textit{memory chunks} that may be physically at different nodes.




==> overview-zhiyuan.tex <==
\section{Design Overview}
\label{sec:overview}

This section gives an overview of \sys, centered around the concept, generation, and execution of resource graphs.
Overall, \sys\ contains two parts as shown in Figure~\ref{fig-workflow}: an offline part that profiles application behind user-perceived execution and compiles unmodified user programs into resource graphs, and an online part that executes resource graphs when triggered by user events.
Connecting the two parts is our proposed resource graph model, which we will introduce first in this section before presenting the high-level ideas of offline and online systems.
%In the offline mode, \sys\ performs program analysis and fine-grained profiling {\em dry runs} to generate a DAG of elements and an estimation of how much resource each element needs. In the online mode, triggered by user events, \sys\ executes this DAG by scheduling and running its elements, with resources allocated according to the offline mode's estimation. 

%\input{fig-example-stack}
\input{fig-workflow}

%\subsection{Resource-Based View of Applications}
%\label{sec:components}
% (why we need components)
%As program organized with control-flow functions couples the resource usages, we need a resource-centirc representation for programs. 
%Before presenting \sys's abstractions, we first  introduce \sys's view of serverless applications.
%\zhiyuan{remove}
%Different from FaaS-based serverless, \sys's view of a serverless application is based on its resource features.


\if 0
A major challenge here is that it is infeasible for the offline component to generate a DAG of elements that can {\em always} work well at the run time, since program behavior and resource utilization depend on inputs, which may, however, drastically change as the execution progresses, thereby invalidating the DAG that the offline component produces (with an initial input). 
This implies that a one-time generation of elements is not enough, and we need to keep monitoring resource usages in real executions and adjust the element DAG (and the corresponding resource estimation) accordingly.
However, it is infeasible to perform the offline mode's fine-grained profiling in the online mode, since doing so would largely impact real executions' performance.
%To make matters worse, the requirement of high efficiency in real executions precludes any heavyweight profiling (such as the dry run), making it hard for us to collect new stack traces and repartition the program.  

To solve this problem, our idea is to let the offline component generate more elements at a time than what the online system actually uses.
We call the former {\em logical element}s and the latter {\em physical element}s\footnote{We use physical elements and elements interchangeably throughout the paper.}.
Each physical element is the combination of one or more logical elements.
With more logical elements, we can change physical elements in the online mode without incurring high profiling performance overhead. 
To know real runs' resource usages, \sys\ periodically sets an execution as the {\em measurement run} (\eg, one out of 1000 executions).
\sys\ performs {\em lightweight, coarse-grained} profiling at measurement runs by measuring the resource consumption {\em only at the boundary of every logical element}. 
Based on the real resource usage measurement, \sys\ chooses new physical elements (\eg, from $[L1+L2, L3]$ to $[L1, L2+L3]$).
\fi


%\input{fig-example}


\boldunderpara{Component materialization.}
%\label{sec:materialize}
%\notezhiyuan{Allocation and executing based on resource graph will reduce resource waste }
The resource graph described above is intended to follow application resource features to minimize resource wastage. As such, a component in a graph can have arbitrary size and duration. If a system directly schedules and executes them, it would be hard to achieve high utilization of server resources.
To solve this problem, we propose to instantiate an arbitrary-sized component as several fixed-size internal components. We call this process {\em materialization}, the former component {\em virtual}, the latter {\em physical}.
%The components in the resource graph as defined in \S\ref{sec:components} are {\em virtual}.

\sys\ materializes virtual components to physical ones at the run time in an on-demand and auto-scaled fashion that is optimized for run-time scheduling and execution.
One virtual component could be materialized as multiple physical components potentially on different servers, and \sys\ transparently maps an access of a virtual component to one or more accesses of the corresponding physical component(s).
Multiple virtual components could also be materialized as one physical component that runs on one server. \sys\ dynamically adds more physical component on demand, e.g., when a virtual memory component's size grows. It can also create multiple parallel instances of a virtual compute component %\noteryan{By compute memory does it mean like multiple copies of the read-only sections of the binary or does it just mean arbitrary virtual memory component} 

Decoupling virtual components from physical components allows \sys's runtime to 1) avoid resource fragmentation because physical components are all of fixed sizes, %\notewill{I'm confused as to why physical components are cited here as the cause of resource stranding. Isn't resource stranding in current serverless due to fixed-sized/fixed-ratio functions? The improvement made by Scad is that now a function is no longer required to map exclusively to one server: the virtual to physical component abstraction eliminates the resource fragmentation caused by fixed-sized allocations.} 
2) transparently and dynamically {\em scale} a virtual component, 3) have a virtual component's {\em size} go beyond what a single machine can hold, and 4) transparently {\em aggregate} multiple virtual components or {\em disaggregate} an aggregated component.
%to avoid network communication, and 4) transparently {\em disaggregate} an aggregated component when resources in the balanced pool is scarce.
% 1) and 4) improve resource efficiency, while 2) and 3) improve performance.
%easily make different materialization choices for a component without the need to involve other components even when they have communication or dependency relationships.
%We are able to do this decoupling because of the serverless computing service model: users supply application code and allow the providers to execute in any way they want (as long as some performance and cost guarantees are delivered).
% Users can specify a maximum hourly cost rate or the maximum level of parallelism



==> policy.tex <==
%\notezhiyuan{materialization plan or materialzation allocation adjustment?}
\subsection{Component Resource Adjustment}
% \subsection{Component Adjustment}
\label{sec:policy}


To improve the overall performance of executing applications in a \sys\ cluster, we dynamically %set the default resource plan and 
"morph" the resource graph for new invocations of each application if needed. %To adjust the resource plan based on historical usage patterns, we collect usage data for each component and report it to the global scheduler, which decides on how to change resource plan as discussed below. Rather than adjusting components based solely on current metrics, we incorporate historical usage to avoid over-adjusting for one-time input changes.


\if 0
% the text version without equations starts here
As mentioned earlier, each component is composed of one or more logical components. For component $i$ of the DAG with $n_{i}$ logical components, the corresponding resource usage vectors of CPU, memory (including remote swap), and network bandwidth are as follows:
\begin{equation}
C_{i} = [c_{1}, ..., c_{n_{i}}], M_{i} = [m_{1}, ..., m_{n_{i}}], B_{i} = [b_{1}, ..., b_{n_{i}}]
\end{equation}
Storing all resource usage measurements as time series is costly. 
To keep the metadata overhead low, we only store the exponential moving average (EMA) of measurements. 
Upon receiving the $t^{th}$ measurements, we update the C vector in the following way (similarly for $M$ and $B$):
\begin{equation}
C_{i}^{t}=\begin{cases}
    [c_{1}^{t}, ..., c_{n_{i}}^{t}], t=0\\
    \alpha ([c_{1}^{t}, ..., c_{n_{i}}^{t}]) + (1-\alpha)C_{i}^{(t-1)}, t>0
\end{cases}
\end{equation}
$\alpha$ is a coefficient between 0 and 1 and controls the decay speed of old observations. We use $\alpha=0.5$ by default.
\fi

%\zhiyuan {selection of memory component steps need to briefly mention here.}

\if 0
\subsubsection{Per-component Resource Adjustment}
%\notezhiyuan{need to say not runtime scale, we still do per-instance scale, but select the right resource amount at materialization time}
\label{sec-policy-component}
As shown later in \S\ref{subsubsec:component_adjustment}, it is critical to right-size components to hit a balance between performance and resource efficiency. 
To do this, \sys\ readjusts each component's resource allocation periodically after $K$ (\eg, 1000) invocations of an application.
%\notegeoff{what is an invocation here?  is it the invocation of the entire application, or of the component?  (I'm assuming component)  how many component invocations are there in the apps in the evaluation (e.g., can you give an intuition on how many resource adjustments might be made during the execution of an application?)}
%This adjustment uses the per-component resource usage distribution and is different for compute and memory components.
For a compute component, if the total memory usage (including swap) is below a preset threshold (256MB by default), we leave the component in the compute pool.
If the swap frequency of the compute component in the compute pool is consistently high and total memory footprint exceeds this limit, \sys\ places it in the balanced pool for future invocations and sets its local memory size to the measured swap space size plus the prior local memory size.
For a memory component, the adjustment is its initial and incremental memory allocation sizes (\ref{sec:memorycomponent}).
We set these sizes based on historical memory usage patterns.
%on the other hand, can only be kept in the memory pool. 
%Thus, the only adjustment required is setting its initial and incremental memory allocation sizes based on profiled memory usage pattern.
% \mohammad{We need to talk about vCPUs too. Apparently its currently set by the user and is not adjusted by the system. Any ideas Yiying?}
% Based on the per-component resource profile, \sys\ adjusts the component's resource allocation periodically (\eg, after every 1000 invocations), which could avoid over-reacting to small load spikes.
%As this paper focuses on demonstrating the overall idea of adaptive resource-based components, we do not claim our current policy to be the best, and it can easily be replaced by other policies.
%After updating the resource usage vector with the latest profiling data, the optimization algorithm decides whether the following changes are necessary:
% \zhiyuan{policy balances the execution performance and overhead of runtime scaling and fine grained physical elements.}
% For compute components, we increment or decrement the vCPU count if its peak CPU utilization is above a high watermark or below a low watermark.
% \zhiyuan{when a compute memory shows increasing demand of memory, as swap frequency of a compute component in the compute pool is high, our policy will adjust its intial memory and swap object size, and move it to compute/balanced pool based on adjustment results.}
% If the swap frequency of a compute component in the compute pool is high, we move it to the balanced pool and set its initial local memory size to the measured swap space size.
% \yiying{Zhiyuan/Mohammad, fill what's the criteria for moving a compute component back to the compute pool}
% We adjust memory components' initial and incremental sizes based on profiled memory usage patterns.
% \yiying{Zhiyuan/Mohammad, shall we include more details on how exactly we do this?}
%increase its initial size if our profiling finds it to be quickly scaled up after initialization and decrease the initial size if \fixme{what?}.
%We also adjust the incremental size (\S\ref{sec:memorycomponent}) based on the profiled scaling pattern.
\fi

\if 0

\vspace{-\topsep}
\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
    \myitemit{Increasing resource allocation:}
    If the peak CPU utilization of an component is higher than a threshold, we increment the vCPU count of this component.
    If there are large amounts of swapping activity, we increase the memory size to the current memory size plus the swap component size.
    %We only increase resource allocation if doing so would not exceed the maximum container size (\eg, a cluster-wide configuration set by the provider).
   % If the vCPUs allocated to an component are below the allocation limit and the peak CPU utilization is high ($\max(C_i)>c_{th}^{high}$), the optimizer increments the vCPU count for the component. Similarly, if heavy swapping is measured ($\frac{\max(M_i)}{Mem_i}>m_{th}^{high})$), the allocated memory size for the component should increase, if possible. Changing the resource limits is a lightweight operation and immediately goes into effect for the next invocations without the need to rebuild docker images.
    \myitemit{Decreasing resource allocation}:
    When not all allocated resources are used in an component, the provider would waste resources, and it is incentive to reduce the resource allocation to more closely match the used amount.
    If the peak CPU utilization is lower than a threshold, we decrement the vCPU count, and similarly for memory reduction.
    %If the maximum memory usage is lower than the allocated amount, we reduce the memory allocation to the actual usage (plus some slack space).
    %Decreasing the allocation limits is needed to minimize the cost for the users and to increase the packing density.
    %If the peak CPU utilization is too low $(\max(C_i)<c_{th}^{low})$, the optimizer decrements the vCPU count for the component. Similarly, if the peak memory usage is low ($\frac{\max(M_i)}{Mem_i}<m_{th}^{low})$), the memory allocation is shrank. 
\end{itemize}
\vspace{-\topsep}
\fi

\input{fig-exp12-merged}


\subsubsection{Component Aggregation}
\label{sec:aggregation}

Aggregating disaggregated components and running them in a balanced pool eliminates network communication overhead. However, the balanced pool has limited space, and \sys must decide which sets of components to aggregate. We frame the problem as a zero-one integer linear program where each candidate is decided to be aggregated (1) or not (0). The ILP solver assigns binary decision variables to minimize network communication overhead while respecting the available resources in the pool.

When two or more components are aggregated, they become a new physical component that runs in a single sandbox. For example, merging a compute component with one or more memory components involves allocating \sys-managed memory spaces inside the merged sandbox. During execution, \sys handles memory access calls by copying to/from the local memory space. Additionally, the \sys runtime starts K processes in one sandbox when merging K compute components and handles communication API calls by sending/receiving inter-process messages. Giving each merged component its own space allows \sys to monitor the communication load between the original components, while having merged components run in one sandbox improves performance~\cite{Dukic_2020}. 



\subsubsection{Component Disaggregation}
\label{subsec:diagg_pol}
When the balanced pool gets overloaded, \sys\ needs to disaggregate to free up resources.
Determining which disaggregation candidate to chose is also done using a zero-one ILP solver.
Here the goal is to incur minimum increase in network communication overhead (optimization function), while respecting the resources available in memory and compute pools (hard constraints) and freeing up a minimum amount of resources from the balanced pool (soft constraint). 
Our aggregation mechanism discussed in \S\ref{sec:aggregation} is what enables us to still capture the communication load between components after they are aggregated.
To prevent thrashing, we use a smaller watermark for aggregation than for disaggregation.
% , creating a hysteresis behavior that acts as a buffer.


% The policy for disaggregating components is the opposite to the aggregation policy, \ie, choosing the component that could fit to the compute and memory pools and would add the {\em minimal} network communication overhead after disaggregation.
% We also form a zero-one ILP similar to the ILP for aggregation.

\if 0
Depending on the pressure on the balanced pool aggregation or disaggregation decisions need to be made:

\vspace{-\topsep}
\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
    \myitemit{Disaggregating components}:
    Ideally, if there is capacity available in the balanced pool, keeping co-running components aggregated guaranties minimum communication latency. 
    However, as the utilization of the balanced pool gets high (e.g., beyond 85\%), disaggregation into CPU and memory pools is required. 
    \sys has a splitting policy that decides which components should be disaggregated to incur minimum overhead. 
    This optimization problem is solved using as a zero–one integer linear program.
    The objective function to be minimized is the sum of communication bandwidth ($\sum b_i$) for disaggregated components. 
    The constraints include resources available in the CPU and memory pools as well as the minimum amount of resources to be reclaimed from the balanced pool~\footnote{If reclamation request cannot be met, the optimizer re-tries with a smaller limit (20\% less each time).}.
    %%% old text below  
    % %Finally, the last optimization decision is splitting an component to two or more components. 
    % If different logical components in an component have significantly different resource usages (\eg, more than 2\x\ different), we split the component at where resource usage changes.
    % %more than one logical component and % a cut-point can be selected such that the peak memory usage before and after the cut-point are significantly different (e.g., $\geq 2$x), it makes sense to split the component to two dependent components. 
    % The other case is when the allocated container memory is at its max, but heavy swapping is observed.
    % Splitting this component to concurrent or dependent components can help reduce the performance overhead caused by swapping.
    \myitemit{Aggregating components}:
    If the balanced pool has enough available capacity, disaggregated co-running components can be aggregated to reduce communication overhead. 
    \sys's merging policy is in charge of determining the best candidates to merge. 
    Here also we use a zero–one integer linear program to solve the optimization problem. 
    The objective function to be maximized is the sum of communication bandwidth for aggregated components.
    The only constraint is for respecting the available resources in the balanced pool.
    %%% old text below
    % There are two scenarios that require the merging of components.
    % First, when the resource usages of two or more co-running or dependent components are similar (for all types of resources), we merge them, as doing so would not cause resource under- or over-provisioning and would avoid the network communication overhead.
    % %First is when there exist concurrent or dependant components that are underutilized, even with the smallest allocations sizes (e.g., 1 vCPU). 
    % % In such cases, merging those can improve resource efficiency and reduce unnecessary communication or cold start latency. 
    % Second, if two or more co-running components have high communication overhead that significantly impacted the entire application's performance, we merge them (as long as the merged component fits in the maximum container size) even though doing so would result in potential resource wastage.
    % %The second case is to mitigate high communication bandwidth between two concurrent components. 
    % %We profile the point-to-point communication between components and if it exceeds a threshold (\fixme{XXX}), it makes sense to merge these components.
    % %Note that such merging is possible only when the sum of resources required by those components is lower than the cluster-wide container maximum size.
\end{itemize}
\vspace{-\topsep}
\fi
%%% old text below
% Finally, to avoid oscillating between adjustment decisions (\eg, increasing resource $\Rightarrow{}$ splitting components $\Rightarrow{}$ merging components $\Rightarrow{}$ increasing resource), we separate the thresholds used for different decisions with a big enough gap and keep a short history of past adjustment decisions (to avoid going back).


==> porting.tex <==
\section{Porting Applications to \sys}
\label{sec:porting}
%\notezhiyuan{Should focus on 3.1 and 3.3? This section introduces Scad’s core abstraction, resource graph. We with a complete workflow example, we demo the interface and and how to map componet graph to servers.}

This section introduces how we port applications to \sys's internal resource-graph interface. Our current two approaches serve more as a proof of concept. Future extensions such as profiling-guided resource-graph generation and other compiler optimizations are all possible.
%and then to execution units. 
Figure~\ref{fig-workflow} illustrates the workflow of \sys\ and Figure~\ref{fig-example} shows a code example. %\ with a simple example.
%\notezhiyuan{Details should go appandix}

%\subsection{\sys\ Programming Model, Compiler, and Libraries }
%\label{sec:program-model}

\boldunderpara{User annotation.}~~
The first way to use \sys\ is by adding two annotations to original user code: \textbf{\textit{\xsplit}} which indicates a location to separate code into two triggering compute components and \textbf{\textit{\remote}} which indicates a data structure that is intended to be placed as a memory component.
\sys\ compiles user annotated code to an internal representation. 
This internal representation includes a JSON file that describes the construction of a resource graph, with each compute node being a code snippet that is compiled from the original user code.
When compiling, \sys\ can identify the relationship between components and the time span (life time) of a component.
It also finds the variables that are shared across a \xsplit annotation and puts them in a memory component. The compiler then converts the original accesses of these shared variables into \sys's internal remote-memory accessing APIs.
%Figure~\ref{fig-example} illustrates this process with a simple example code snippet.
The \textbf{Appendix} describes all the internal APIs.
%\zhiyuan { I'd say annotation is not the essential thing here. Calling a library & adding annotations takes the same efforts. As the essential of high-level things is the two major tasks (1) without changing the programming model, identification of components from code snippets and generating the components. 2) generating high-performance interaction code using \sys native APIs between components.)}

\boldunderpara{\sys\ libraries.}~~
The second way to use \sys\ is by replacing existing libraries with \sys's corresponding libraries. 
\sys libraries implement certain library calls as remote accesses using the internal interface discussed above.
As a proof of concept, our current implementation includes two libraries.
The \textbf{\textit{NumPy array}} library places a Numpy array annotated with \remote\ as a memory component and implements Numpy array operations to it using \sys's internal remote memory accesses.
The \textbf{\textit{DataFrame}} library and our compiler convert programs written with pandas~\cite{mckinney-proc-scipy-2010} to a resource graph.
Our compiler generates one memory component per DataFrame and one compute component for each operator such as \texttt{map}, \texttt{join}, \texttt{shuffle}, and \texttt{reduce}. 
%We also apply an optimization to generate one compute component from multiple operators of the same nature (\eg, multiple filters working on the same data). The compiler generates one memory component per DataFrame that a compute component accesses.
The library implements each DataFrame operator using \sys's internal remote-memory accesses.
This compiler-library combination demonstrates the possibility of transparently porting programs that are well encapsulated into computation stages.


\boldunderpara{Application porting.}
%\harry{I think it would benefit from discussing why it is easy to split existing applications.. something along the line of serverless applications commonly having multiple phases, each phase with it unique resource profile; the boundary of phases is often an API call that can be easily identified.. give a few examples. }
%\zhiyuan{I think we should including both identifying memory and compute. Example: Video processing pipeline may including multiple tasks (decompressing, preprocess, filtering, detection. ). In many of this tasks they also know the time span of objects: e.g, after decompression the original input is released.}
Application developers can leverage their understanding of an application to add annotations or use \sys\ libraries.
Our simple annotations and proof-of-concept libraries can already support a wide range of programs. New compilers and libraries could be built to support more programs.
%For example, existing serverless programs with stages, such as a video processing pipeline may include a decompression, a pre-processing, and a face-detection phase.
%Each phase could process and generate a distinct data structure (\eg, a set of frames).
%Those stages and data structures with distinct resource requirements can be identified as components leveraging our annotations.
Application developers can also analyze their applications using profilers like Scalene~\cite{scalene, scalene_arxiv}, pprofile~\cite{pprofile}, or Memray~\cite{memray} to capture how resource consumption changes and annotate their code accordingly. 
Future tools and compilers could potentially automate the above steps.
%Using native interface requires programmer to re-organize programs to components and work with low-level communication interfaces of components, which could be a complex job for programmers that are not familiar with the concept and lead to low performance due to wrong decomposition of programs. As we observed most of the information needed to decomposition the program is already embedded in the source code, we introduce the add-on compiler and high-level interface to application builders.
%
%Furthermore, it is possible to convert certain types of unmodified and unannotated programs to \sys\ with the right compilers and profiling tools; we show an initial exploration in this direction with our DataFrame compiler to be discussed soon and leave full exploration to future work. Finally, unmodified and unannotated programs can also run on \sys, by simply being treated as a single mixed component and benefiting from \sys's transparent swap system. 
%

After compiling, users deploy their application to \sys\ by submitting the generated JSON file and code pieces.
The user also specifies the events which trigger the application.
Users can keep adding more or changing existing annotations and library uses to incrementally port their applications to \sys. 
%\notegeoff{can application porting to Scad be done incrementally?  e.g., first use the libraries, but leave the application as one big component, then do a coarse-grained component partitioning, etc.  the more porting the better the benefits, but it can ease the transition. zhiyuan: yes. We allow compute elements with large memory resources}


==> references.tex <==
\pagestyle{empty}

\bibliographystyle{ieeetr}
\bibliography{references}

==> results.tex <==
\section{Evaluation}
\label{sec:results}

\boldunderpara{Implementation.}
We implemented \sys's compiler and program analysis on top of Mira~\cite{Mira}.
We implemented \sys's runtime system on top of Apache OpenWhisk~\cite{OpenWhisk}.
In total, \sys\ includes $\mathtt{\sim}$17K SLOC: 1.4K lines of change on Mira, 9K lines of Scala to extend Openwhisk's scheduler and executor, and 4.6K lines of C together with 1.8K lines of Python for runtime and libraries.
Currently, \sys supports programs written in Python, the second most commonly used programming language in serverless~\cite{Datadog_2023}, and in C++, a common language used for bulky applications.

\boldunderpara{Environment.}
We evaluated \sys\ on a local rack of a Dell PowerEdge R740 servers each equipped with two 16 core Intel Xeon Gold 5128 CPU, 64\GB\ of memory, and a 100\gbps\ Mellanox Connect-X5 NIC. 
We use eight servers for running \sys\ and systems in comparison and four additional servers to run Redis.
All the servers are connected to a 100\gbps\ FS N8560-32C 32-port switch. All servers run Ubuntu v20.04 with Linux v5.4.0. We use Docker v24.0.7 for containers.


\subsection{Application Performance and Resource Consumption}
\label{sec:eval-app}


We first present the high-level results of running three bulky applications on \sys: 1) data analytics on TPC-DS, analytical queries with different stages of parallelism and resource consumption, 2) video processing pipeline, with computation and data dependency defined by graph, 3) logistic regression training, a single-threaded application with different resource-consumption phases.

\boldunderpara{Distributed Queries with TPC-DS}
First application we evaluate is distributed data analytics on PyWren running the TPC-DS benchmark~\cite{tpcds:sigmod02}.
We compare \sys\ with Pywren~\cite{jonas2017occupy_pywren} running on OpenWhisk on our local cluster.

We use a database size of 100\GB\ and evaluated three TPC-DS workloads with different performance characteristics and varying resource requirements: queries 1, 16, and 95.
They read 2.5\GB, 20\GB, and 19\GB\ of data respectively and have peak memory usage of 240\GB\ and peak CPU of 120 vCPUs.

PyWren splits each TPC-DS query into several stages. For each stage, PyWren generates static number of workers to perform the computation, and we use Orion~\cite{Orion-osdi22} to set the resource for each worker. Intermediate data storage for PyWren uses Redis servers in the cluster. 
In \sys, We implement each query as a single Python program and annotate related memory and compute components.
\sys infers data components when converting each query to a resource graph.

% \boldunderpara{Overall cost and performance.}
Figure~\ref{fig-tpcds-resource} shows \sys's and PyWren's total memory consumption. PyWren failed to scale efficiently with multiple isolated functions. \sys\ reduces memory consumption by 72.5\% to 84.8\%.
% PyWren provisions each stage for its peak memory usage. Moreover, each worker in PyWren fetches all the data it will access from Redis before the computation starts and stores the data back after all its computation finishes. Essentially, PyWren pays for the same amount of memory consumption twice. In contrast, \sys\ right-sizes each of its components by auto-scaling on demand. Moreover, \sys\ does not incur the double-memory-consumption problem, as it only fetches data when accessed.

% Comparing across queries, Q16 has the largest resource consumption reduction and performance improvement because it has a higher degree of parallelism and a more complex sharing pattern, which \sys\ handles a lot better than PyWren.

Figure~\ref{fig-tpcds-time} plots the total run time of the three queries.
\sys\ outperforms PyWren by 54.2\% to 63.5\%, primarily due to \sys\ adaptively schedules and access data components locally. Over 84\%, 78\%, 82\% shared memory accesses are local for Q1, Q16, and Q95.
% Moreover, PyWren incurs significant I/O performance overhead because of its serialization/deserialization. In comparison, \sys's accesses to a remote data component is via zero-copy RDMA with no need for serialization. 


\boldunderpara{Video Processing.} 
Our Second application is video processing, where we perform video transcoding using the encoding/decoding operators developed by ExCamera~\cite{excamera}. ExCamera divides video frames into batches and uses one parallel worker to encode a batch.
Our version is a single program with 11 annotations, where input video are sliced into parallel segments and each segment are processed with up to 16 parallel compute units. We use ExCamera's set up of six frames as a single encoding unit and a batch size of 16 units. 
\sys\ generates a resource graph with 37 compute and 33 data components.

We compare \sys\ to ExCamera running on the gg~\cite{fouladi2019laptop} serverless frameworks. gg offers several backends, and we use the OpenWhisk backend. The gg implementation represents the encoding of each frame batch with 80 functions, each reading from and writing to a Redis intermediate storage pool. 
We also compare with a local $vpxenc$ encoder~\cite{vpxenc} that runs everything natively on one server in our cluster.

Figure~\ref{fig-excamera-time} plots the total execution time of the three systems processing a 1-minute slice of the movie "Sintel" (2010) ~\cite{sintel2010} in three resolutions: 240P, 720P, and 4K. The peak resource usage hits the cluster resource limit of 120 CPUs and 174GB of peak memory in both Openwhisk and \sys. \sys\ achieves the best performance for all three resolutions. \sys\ performs adaptive materialization and launches \81.3\% of components in same batch on the same server. In contrast, even when servers used for the gg experiments have the same amount of free resources, gg's functions share data that always lives on separate Redis servers.
$vpxenc$ runs in one server, but it is limited by the amount of parallelism it can achieve: only 18 out of 32 allocated cores and 14 out of 16GB allocated memory are actually used.
This difference is more apparent with larger videos that benefit from larger parallelism.

However gg fails to achieve resource- and performance-efficiency as it scales up.
Figure~\ref{fig-excamera-mem} and Figure~\ref{fig-excamera-cpu} plot the total memory and CPU consumption. 
\sys\ consumes the least amount of memory, and gg consumes the most.
As a function-based framework, gg sets the same function size for all inputs. Thus, it has to make provisions for the largest anticipated inputs, causing significant unused resources for the smaller 240P and 720P videos.
For the largest 4K video, gg incurs significant execution-time overhead and memory overhead for reading/writing data to Redis, which putting together, causes high memory consumption. 
$vpxenc$ has similar or lower used memory as \sys, but its unused memory amount is much larger. As a single-unit execution, its size needs to be set to the peak memory size.

Similar to memory, gg and $vpxenc$ also incurs high CPU resource wastage because of their peak-based static provisioning. Unlike memory, their used CPU resource is also much higher than \sys\ with 720P and 4K resolutions, mainly because of their longer execution time. \noteyiying{I don't get why longer execution time doesn't result in larger used memory for them, esp. gg 720P}
\notezhiyuan{give it one core it will run forever but have less CPU-time, as cpu is not wasted}


\subsubsection{Performance Breakdown}
\input{fig-breakdown}

As shown in Figure~\ref{fig:eval:breakdown-tpc} and Figure~\ref{fig:eval:breakdown-excamera}, we \sys's three key approach supporting adaptive serverless, including resource graph, adaptive execution and proactive execution, and how it would affect the performance.

Going from function-centric to resource centric allows resource to be shared between multiple computation segments and scale independently. This greatly improves the computation efficiency, especially reduces the allocated but not used resource caused by resource bundling. However, on execution time, this may introduce the extra scheduling overhead and pay for inefficient remote access. Whether the execution time larger or smaller than function-centric depends on whether the remote access overhead is larger.
Adding adaptive execution allows resource access to be native and efficient, greatly reduce the execution time.
Further, adding proactive scheduling and execution tunes the scaling patterns based on history, reduces the scheduling effort, setup time and chance of remote accesses, further improve the performance.



\subsubsection{Comparing with Other Systems}
\label{sec:eval-lr}

% \zhiyuan{I'll try to write key ideas of each experiment. First one is application level, compare with serverless DAG and Reactive disaggregation}

Our first application is a machine learning training task using logistic regression (LR) ported from Cirrus~\cite{carreira2019cirrus}.
It first loads the input data set and separates it into a training set and a validation set.
Then, it performs the regression on the training set.
Finally, it validates the trained model with a validation set.
%
%We annotate the original code with 3 \xsplit\ annotation points where tasks change. 
\sys\ compiler generates a resource graph of four compute components (loading, data-set splitting, training, and validation) and three data components (training set, validation set, and learned weights).
Figures~\ref{fig-lr-resource-mid} and \ref{fig-lr-resource-large} plot the total memory consumption of these schemes when processing two input dataset sizes, 12\MB\ and 44\MB, which result in peak memory usage of 0.78\GB\ and 2.4\GB\ respectively. 
%We separate consumption accounting between the compute side (Lambda, \sys\ compute components, FastSwap's local node) and the memory side (S3, Redis, \sys\ data components, FastSwap's remote memory).
%\notezhiyuan{need to explain colors. May be "resource wastage" first? }
As all schemes use the same number of vCPUs in this experiment, CPU consumption comparison directly translates to comparing execution time, which we show in Figure~\ref{fig-lr-time} for the 44\MB\ input.
Overall, \sys\ consistently achieves the lowest resource consumption, highest resource utilization, and best performance. Comparing the two inputs, the smaller wastes more resources for the baseline systems but not \sys.

\boldunderpara{System comparison on local cluster.}
We compare \sys\ (RDMA and TCP) with executing the original program on vanilla OpenWhisk and on FastSwap~\cite{FastSwap}, a system optimized for remote-memory swapping. OpenWhisk executes the application as one function sized to the peak memory size. FastSwap uses the same amount of local memory as \sys's compute component and remote memory of the peak memory size. We run these systems on our local cluster to have controlled network environments. 
For the two inputs, \sys\ (when running on RDMA) reduces resource consumption by 40\% and 84\% compared to OpenWhisk while only adding 1.3\% performance overhead. Even when running on TCP, \sys\ still largely reduces resource consumption with small performance overhead.
Moreover, \sys\ only has 0.9\%-3\% unused resources, while OpenWhisk wastes 9\%-70\%.
FastSwap has the highest resource consumption and performance overhead among the three, because it wastes a significant amount of remote memory by allocating for the peak (no autoscaling) and its swap-based coarse-grained remote memory access overhead. 

\input{fig-exp12}
\input{fig-exp346}


\boldunderpara{Running on AWS services. }
We also ran a set of configurations on AWS: 1) running the entire program as one Lambda function, 2) running the same four code pieces as \sys\ compute components in four Lambdas orchestrated by AWS Step Functions~\cite{AWS-Step-Functions} and storing data components in S3 or Redis~\cite{REDIS}. %running on an EC2 t3.medium instance. 
%As Redis is faster than all existing serverless computing frameworks with intermediate storage pool~\cite{klimovic2018pocket,sreekanti2020cloudburst}, we only evaluate Redis here.
For Step Functions,  we use two settings: %\textit{{SF-PO} (performance optimized)}: size Lambda functions to achieve the optimal performance; 
\textit{{SF-CO} (cost optimized)}: size Lambda to achieve the lowest cost~\cite{power-tuning,Eismann_2021,COSE} with Redis used for intermediate state; %(in GB$\times$second, which is proportional to AWS's billing of Lambda but does not use dollar price); 
and \textit{{SF-Orion}}: size each Lambda function using Orion~\cite{Orion-osdi22}.
%Although we only compare with AWS, the problems we show prevail in other clouds.

Running the resource graph on Step Functions only reduces 2\%-5\% memory resource consumption with SF-CO and 3\%-3.5\% with SF-Orion compared to single Lambda, far from how much \sys\ reduces over OpenWhisk.
Digging deeper, we found that splitting a program into Lambda functions introduces both performance and resource overhead, as seen in Figure~\ref{fig-lr-time}.
Each function needs extra time to read/write data from S3 or Redis and serialize/deserialize the data. Serialization and deserialization also requires extra memory space. 
%Moreover, the communication between Lambda and S3 is slow.
%However, communication speed to S3 is not the main performance overhead, as can be seen from the only-slightly-better run time when running on Redis, an in-memory key-value store. 
These results demonstrate that simply writing an application as function DAGs on today's serverless platforms is not enough. % for achieving cost and performance goals.
%\notezhiyuan{splitting into components cannot achieve performance and resource efficient at the same time}

%\boldunderpara{Resource wastage on AWS.}
%Figures~\ref{fig-lr-resource-mid} and \ref{fig-lr-resource-large} also report allocated but unused resources (\ie, resource wastage). 
Additionally, all schemes have huge resource wastage, especially with the small input, for several reasons. %There are multiple causes of resource wastage on AWS.
As discussed in \S\ref{sec:serverless}, FaaS services only allows one function size for all invocations and throughout an invocation's execution.
Moreover, AWS fixes the CPU-to-memory size ratio, causing wastage of CPU or memory.
%memory is wasted when a function reads/writes data from storage and serialize/deserialize them.
%Fourth, CPU and memory sizes have fixed ratio. When optimizing for performance, the CPU size fits the needs but memory will be over-provisioned, causing more resource wastage in SF-PO. In contrast, when we set the size to be minimal memory, execution time increases significantly (not shown in the figures).
Finally, the Redis instance is provisioned for the peak resource usage and wastes huge amounts of resources at non-peak times.


%\zhiyuan{\sys\ schedules at local server and converting data sharing to both shared memory access or remote memory access,} \fixme{then need to talk about how much is local vs remote} incurs negligible I/O and scheduling overhead.


%\yiying{Zhiyuan, how many times did we run each experiment?}
%\zhiyuan{Average of several runs, did not remember the details, should be less than 5 times. maybe not mention this?}
% (zac)[removed for brevity] Unlike PyWren whose scaling unit is a FaaS function, 
%\sys\ can both increase the memory size of a compute/memory component and invoke more parallel instances of a compute component.
%Moreover, we use an efficient data-object implementation (zero copy and batching), which makes \sys\ efficient.



\input{fig-exp789}

\subsubsection{Video Processing}
\label{sec:video}


\input{fig-cluster-level}



\subsection{Closer Looks}
\label{sec:eval-micro}

To further understand \sys, we performed a set of additional evaluations to focus on various features of \sys.

\input{fig-exp-add}

% New figure about cluster level utilization
\boldunderpara{Cluster level resource utilization.} \sys's resource saving reflects at cluster level. We evaluate \sys and Openwhisk with same amount of limited resources as shown in Figure~\ref{fig:eval:cluster-mem} and~\ref{fig:eval:cluster-cpu}.

First, \sys achieves better \textit{resource allocation ratio}, because of adaptive materialization reduces resource stranding and utilizes resources across server; Second, most of allocated resources are utilized in \sys, due to the runtime on-demand resource scaling. As a result, given same amount of resources, \sys could utilize more resources in real computing, results in a  \fixme{xxx} performance gain compared to Openwhisk.

\boldunderpara{Alternative resource adjustment methods.}
As discussed in \S\ref{sec:disagg}, resource disaggregation and migration are two possible ways of adjusting resources and avoiding wastage.
We compare \sys\ with 1) swap-based disaggregation (to be fair, we run all \sys's systems except that we perform swapping for all accesses beyond local memory), 2) a best case for live migration by only counting pure data movement time using full 100\gbps\ network bandwidth, 3) migration with MigrOS~\cite{migros}, and 4) vanilla OpenWhisk.
For a fair comparison, we let all systems use the same amount of total resources (not counting unused resources).

As shown in Figure~\ref{fig-tpcds-flex}, for different inputs, the size of $Join$ stage varies from 267\MB\ to 14.7\GB.
with \sys's adaptive materialization, all components run locally with the scaling factor 100, and 34\% of data components' memory regions are scheduled at remote servers with the scaling factor 1000.
Disaggregation solutions like the swap results we show always place data in remote servers, causing high application-execution performance overhead because of network communication.
With migration-based solutions, the application execution runs natively and has no overhead. However, migrations cause significant overhead even with an optimal best case, because bulky applications' memory consumption is high (SF 1000).
Finally, OpenWhisk incurs significant performance overhead for the reasons covered before.

%To compare with disaggregation, we 
% \zhiyuan{In this exmaple we focus on the scaling of the `JOIN` operator in TPCDS-16 quries, which joins three different tables. Depends on the input size, the required memory from a single worker in this operator could go from 176MB to 14.6GB.}
%fig-eval\_tpcds\_same\_resource\_flexibility: Compare with different resource-scaling policy. we use the same allowed resource amount, and same runtime scaling policy (memory), means that no over-allocated is allowed. \sys executes the memory as a.
%Note that migration cannot scale resoruce lively, it will migrate from one fixed size to another. In this case we simulate migrate 
%\zhiyuan{More comments on the migration: migration is not designed for scale multiple times. The figure show one time scale up cost, but in real application the scale up can happen more than one time, along with the program execution. Under this senario our system still pays similar overhead, but a migration-based appeaoch need to migrate multiple times.}


\boldunderpara{Adaptation to different inputs.}
To understand how \sys\ adapts to different inputs, we use the TPC-DS Query 1 with five input sizes (5, 10, 20, 100, and 200\GB) to compare \sys\ with PyWren. 
Figure~\ref{fig-tpcds-input} shows the memory consumption comparison in relative terms, with absolute numbers reported on the top (CPU consumption is similar and not included).
\sys's memory consumption is consistently lower than PyWren. \sys\ adapts its component sizes at the run time according to inputs, thus resulting in negligible resource wastage. PyWren uses one function size across inputs, resulting in significant resource wastage, especially when inputs are small. Its used memory is also higher than \sys\ because of the reasons discussed in \S\ref{sec:eval-tpc}.

Figure~\ref{fig-tpcds-input-time} plots the corresponding execution time. \sys\ achieves good performance, especially with small input sizes, thanks to its adaptive-materialization. \sys\ is able to schedule everything locally for scale factors 5 and 10, 96\% local for SF 20, and 95\% of parallel compute components distributed evenly across four servers. \sys\ is able to pack most non-shared data components local to the compute components, with the shared data components accessed remotely.
%During the execution, most memory accesses goes into one scalable data component (for example, in stage 2, randomlly accessed, scales from 62M to 1.32G) that are placed in the local node, and only data compoentns sharing between computes (scaling from 12MB to 46MB) are accessed remotely. 

%eval\_tpcds\_scale\_resource and eval\_tpcds\_scale\_data shows how \sys adapts to different inputs. on TPCDS-1 Query. With resource-scaling, it keeps a high resource usage for all input size; With adaptive materialization, it keeps high performance for all cases. It could be divided into 3 phases, full local, partial local and divided.

%On performance side, with adaptive materialization, Mira \cite{} identifies the access to memory elements and generate the best case memory access.

\boldunderpara{Effect of adaptive placement.}
To compare different adaptive-materialization placements of \sys, we run the $ReduceBy$ operator within TPC-DS Q16. It involves a set (3 to 120) of parallel compute components passing their result to a single compute component (fan-in), with one data component used for data sharing for each sending compute component (total data size from 730\MB\ to 113\GB). 
Figure~\ref{fig-tpcds-adaptive} shows three cases: local runs everything in one machine, remote-scale scales up data components to a remote machine (with 46\% being local), and disagg runs all components on different machines. Application execution time increases with more components being remote, and most of the overhead comes from pure I/O movement. The system overhead of setting up execution environments and network connections is small.

%Each each worker have one randomly accessed data comp and another data comp for sharing data with reducer. 
%Dependes on the input, the number of parallel workers ranging from 3 to 120 and size of memory component ranging from 730MB to 113GB.
%eval\_tpcds\_adaptive\_materialization. local: All-in-one machine.
%remote access : The randomally accessed data comp is scaled onto the other machine.
%disaggregation of components. almost all physical elements are disaggregated.


\boldunderpara{Resource graph and resource adjustment.}
We compare \sys\ when enabling both resource graph capturing and component size capturing (\S\ref{sec:offline}), when only enabling resource graph capturing (with default component size), and following application task flow (no resource graph generation). 
Figure~\ref{fig-excamera-graph} shows the memory consumption and execution time of these three schemes running transcoding of the 4K video. When directly using the task flow, there is significant resource wastage.
Resource graphs group similar resource usages into components and outlines their lifetime and sharing relationships, which helps reduce resource wastage greatly. 
History-based component sizing further reduces wastage by setting the right initial and incremental sizes and protect provisioned resource for all components.

Figure~\ref{fig-policy-adjustment} plots the performance and memory utilization with three schemes: fixing initial and incremental sizes to 256\MB\ and 64\MB, provision data components to the highest usage (peak-provision), and \sys's history-based size setting. 
We use real-world serverless application memory usage profiles from Azure~\cite{shahrad2020serverless}.
%This dataset contains a set of real-world applications, each being invoked many times with different user inputs.
In addition to the average of all the datasets, we choose a few representative applications to highlight.
% Figure~\ref{fig-micro-adjust-data} plots the CDF of memory usage across invocations of these representative applications and the average memory usage of all applications in the trace.
%The representative applications are 
\textit{Small}: most invocations' memory usages are small, \textit{Large}: most invocations used a lot of memory, and \textit{Varying}: different invocations' memory usages vary largely.
Figure~\ref{fig-dataset-dist} shows their invocation distributions. 
Overall, \sys\ achieves high utilization and good performance.
Peak provisioning achieves the best performance since no auto-scaling or swapping is needed, but has low memory utilization. 
%\zhiyuan{A fixed configuration only works well when an application's usage pattern happens to be close to the configuration. actually this cannot process variance data. Maybe just remove this} 
A fixed size configuration can lead to both poor resource utilization %(when real usage is below the configuration) 
and poor performance. % (when frequently adding many physical memory components). % at runtime).

\if 0
What's the benefit of using a resource graph and offline compiling? 
Resource graph adds the support for lifetime of memory elements, reduces the lifetime of memory elements, enable better scaling and data sharing. enable resource-based scaling. AS \sys will be able to schedule things together, execution time is also reduced. Downside is with default scaling, the resource usage is low esp the inital requirement is small. Also without provisioning the scale-up part would be scheduled on other machine - in this cases, over 7.7\% of data components are scheudled apart from its accessing compute.

Graph-History bsaed provision add scaling capalibity. (faster resource scaling, more accurate allocation, better cpu scaling, better scheduling). In this cases as reported in ExCamera, only 1.3\% of components are accessed remotely.

We need to focus on two things in this process: Task graph to resoruce graph highlights the resource relationship and instruct us how to scale the resoruce, so adaaptive materialization could use it to reduce both runtime (as access to redis is merged back) and 
\fi



\if 0 
\sys\ also achieves a much higher speedup than OpenWhisk when scaling out, because it avoids function performance overheads such as serialization and data partitioning.
Because of the high speedup and minimal memory consumption, \sys's total memory consumption (GB$\times$min) {\em decreases} by 81\% when scaling up,
while OpenWhisk's provisioned memory increased by 4.57x, and used memory increased by 21.6\% as shown in Figure~\ref{fig-tpcds-computescale-resource}.

Finally, \sys\ automatically and transparently scales a compute component up with memory swapping when the component is low on memory. 
Our results as detailed in \textbf{Appendix} shows that our swap system only adds 1\% to 26\% performance overhead compared to when the entire compute component's memory can fit in the local server. This baseline however makes resource packing hard.
\fi
% % To measure our swap system performance, we use a simple microbenchmark of sequentially or randomly reading an array that is configured to be from 100\MB\ to 1000\MB.
% Figure~\ref{fig-micro-swap} plots the total run time of the microbenchmark with increasing array size. 
% We test two local cache sizes: 200\MB\ and 400\MB, and compare the swap performance against the case where the local memory is larger than the whole array size (\ie, no swapping and the ideal performance but impossible with the compute pool configuration).
% Overall, swapping adds 1\% to 26\% performance overhead. The overhead is higher when the array size is bigger and when the local memory size is smaller.


% We include results of auto-scaling compute components with swapping in the \textbf{Appendix}.
%\zhiyuan{We use a microbench mark which have variance memory footprint dependents on the input size, similar to our motivating example in \ref{fig-micro-elastic}. We load an compressed dataframe dataset and perform random sampling on data set, and return our sampled results. For openwhisk components we prealloc the maximum possible memory usage while utlize \sys's elastic Memory. With nearlly same execution time, we can achieve memory utilization xx-xx compared to fixed resource xx-xx}. 

\boldunderpara{Scheduler scalability.}
Our evaluation shows that \sys's global scheduler can process 50k application invocations per second, 2.5 times faster than OpenWhisk's cluster scheduler. The rack-level scheduler can schedule 20k components per second. We further analyze the component processing rate a rack can execute. Our evaluated applications have an average of around 1 second duration per component; each (compute) component consumes one core on average. A rack typically has less than 1,000 cores. This means a rack’s computation rate is 1,000 components per second. Applying the same type of calculation using today's serverless function duration and resource consumption~\cite{shahrad2020serverless}, we get 9,804 functions per second to be a rack's computation rate.
%If we use today’s serverless functions to model components, according to~\cite{shahrad2020serverless}, each function’s average duration is around 0.6 seconds; each function consumes avg 128MB memory which translates to 0.17 cores using AWS Lambda’s ratio. This means a rack’s processing rate is 9804. 
Both computation rates are much smaller than our scheduler’s 20,000/s request rate. This analysis is robust regardless of the number of components in an application. %, as the more components there are in an application, the more processing needed (fewer applications but same amount of components to schedule).
Overall, \sys\ can sustain a cluster of around 100 to 1000 racks and is more scalable than OpenWhisk. As enable resource sharing between clusters already achieves high resource utilization, future implementations could deploy multiple global level scheduler to achieve better scalability. 
% To scale further, one could change our current single-threaded implementation of the global and rack schedulers to be multithreaded and/or deploy multiple global schedulers.

\boldunderpara{Network communication.}
Figure~\ref{fig-launch} shows the impact of \sys's communication techniques on a workload with one compute component accessing one data component in warm started environments with no established connections. The first bar represents OpenWhisk without an overlay network, while the second bar adds the overlay network to enable direct component-to-component communication. The third bar replaces the TCP stack in the second bar with \sys's RDMA stack, improving component execution time. The fourth bar removes the overlay network and uses \sys's network virtualization module, reducing initialization time. Finally, the fifth bar includes \sys's asynchronous messaging optimization, hiding network connection setup time.





\if 0
\subsubsection{Data Component Autoscaling}
%\boldunderpara{Auto-scaled memory components.}
To demonstrate how \sys\ dynamically scales data components, we build a simple video processing workload 
%inspired by the video processing example in \S\ref{sec:serverless}.
that loads a compressed DataFrame dataset, performs random sampling on the dataset, and returns the sampling results.
Figure~\ref{fig-micro-elastic} shows the amount of memory actually used by the workload, memory allocated by \sys, and memory allocated by OpenWhisk.
When calculating \sys's memory consumption, we also include the local memory used by compute components, which is a fixed but small amount (shown at the bottom of the figure).
\sys\ adapts to memory usage by adding physical data components. 
In contrast, OpenWhisk containers (and public cloud services like AWS) have a fixed memory size throughout the execution, provisioned for peak usage.
In this case, the nearest OpenWhisk can provision is 1.5\GB.

To demonstrate \sys's memory scaling with different inputs, we take a closer look at the \texttt{Reduce-By-Key} stage in TPC-DS.
Figure~\ref{fig-tpcds-memoryscale} plots the memory consumption of computational function when we change the input dataset size, while fixing the compute resources to 20 vCPUs.
%\sys\ uses 20 CPU cores for all the dataset sizes and easily achieves different CPU-memory ratios thanks to memory disaggregation.
%By fully decouple the compute from memory, \sys allows independent scale of memory independent of memory. 
When input data size increases from 64\MB\ to 1\GB, \sys's memory size increases by 1.1\GB, while OpenWhisk's increases by 3.6\GB.
Both systems can use different amounts of memory with the same number of vCPUs (\ie, scaling memory without scaling compute).
OpenWhisk's memory consumption is higher than \sys\ because OpenWhisk requires more memory and execution time to load/store data for each function, and the loaded data occupies memory for the entire duration of a function. \sys\ directly accesses data in memory nodes at the time when the data is needed.
\noteyiying{add why scad is better than scad-unopt, and the difference is much bigger than in Fig13}
\fi

\if 0

\subsubsection{Compute Component Autoscaling}
We evaluate \sys's ability to independently scale compute resources also with the \texttt{Reduce-By-Key} stage. For this experiment, we use an input data of 1\GB\ for all the configurations. 
%Compared to function-centric approach, which means scale by launching parallel functions, \sys's element programming model, share memory elements and optimizations (Section <opt>) allows launching parallel compute elements and..
Figure~\ref{fig-tpcds-computescale} plots the memory usage and run-time speedup when increasing compute resources (in vCPUs).
To model AWS's resource configuration, we set each OpenWhisk function's CPU and memory to have a fixed ratio of 1 vCPU to 1,769\MB\ memory. OpenWhisk scales out by triggering more parallel instances of a function. Because of the fixed-coupling of CPU and memory, this scaling results in 20\X\ provisioned memory when the amount of vCPUs increases by 20\X. In contrast, \sys\ scales only its compute component by invoking 1 to 20 instances of it, while using the same number of data components.
As a result, \sys's total memory size only increases by 67.4\% when its CPU resources increase by 20\X.
For OpenWhisk, in addition to provisioned memory size, we also measure the amount of memory that is used during function execution. 
Its used memory increases by 2.05\X, which is much lower than the 20\X\ increase in its provisioned memory.
This is because the total amount of processed data is the same when scaling out. %, and we shard the data across all the functions, resulting in each processing only a shard. 
%Worth noticing is that even when removing the fixed-ratio limitation, OpenWhisk's used memory is still much higher than \sys's total memory (2.05\X\ vs. 67.4\%). 
%This is because OpenWhisk requires extra memory in each function for data loading (\eg, data structures for serialization/de-serialization).
\fi

\if 0
\subsubsection{Independent Scaling}

To demonstrate its benefit over the fixed CPU-to-memory ratio design of today's FaaS offerings, we perform a micro-benchmark of processing input data of different sizes with {\em reduce by key}.



Figure~\ref{fig-exp6} plots the memory consumption of this micro-benchmark when changing the input size.
Our baseline is using Redis to store the input data and reading the entire data into the local component before performing the computation and writing it back at the end. This is the practice taken by today's serverless computing that uses an intermediate layer to store data~\cite{wang2020infinicache,klimovic2018pocket}.
\sys\ uses a data component to store the data and batches accesses of small reads/writes.
We also include results of \sys\ when batching is not used.

Compared to \sys, using Redis consumes huge amounts of memory, growing with the input data size.
Without batching, \sys's memory consumption also grows as input data size grows, since \sys\ also reads the entire data object.
It is lower than Redis because of our zero-copy design, where the network stack directly uses application data objects without copying.
With batching, \sys\ consumes stable and tiny amount of memory even with growing input size,
because we always read the same size of batch at a time. This result demonstrates the benefit of segregating data components.
\fi

\if 0
\subsubsection{Component Communication}

Figure~\ref{fig-micro-launch} shows the impact of \sys's communication techniques on a workload with one compute component accessing one data component in warm started environments with no established connections. The first bar represents OpenWhisk without an overlay network, while the second bar adds the overlay network to enable direct component-to-component communication. The third bar replaces the TCP stack in the second bar with \sys's RDMA stack, improving component execution time. The fourth bar removes the overlay network and uses \sys's network virtualization module, reducing initialization time. Finally, the fifth bar includes \sys's asynchronous messaging optimization, hiding network connection setup time.
\fi
%\boldunderpara{component Launch Time}
%\zhiyuan{In fig \ref{fig-micro-launch}, we run a small DAG with single memory and compute component to measure the optimizations we introduced in Section \ref{}. Compared to our TCP implementation we can launch and execute compute and memory containers to 2.8x and 23x speedup compared to unoptimized implementation. Our launch and communication setup process even xx faster than openwhisk with a pre-setup redis server.}

% Also, compared to communicate with Redis cluster with fixed bandwidth, our locality based scheduling policy will also enables co-running components to take advantage of lower in-cluster latency.
%In this experiment we show the communication performance between compute and memory components in \sys using the built-in library, compared to other serverless methods for passing or storing information from functions. To run these experiments we launched large number of pairs of compute and memory components concurrently where each pair had direct communication with one another. We show in \fixme{fig} that the latency and overall variance experienced by components in our system is smaller in both respects than using \fixme{xxx} or \fixme{xxx} to communicate.
% 


%\subsubsection{Component Scheduling}

%When applications are split, they will contain more individual components that must be invoked by \sys. In serverless systems, this causes two outcomes: (1) more load is placed on the scheduler and (2) more individual components in the execution DAG are created, leading to a potential for more cold starts. We evaluate \sys cold start performance and measured the scheduler's throughput.

\if 0
\boldunderpara{Startup time.}
To measure startup time, we create an application graph with 10 distinct compute components in a chain, each sleeping for 100\ms. %Table~\ref{fig-micro-coldstart} shows the warm and cold startup time. All the rows except for AWS run on our local cluster. Similar to Figure~\ref{fig-micro-launch}, the overlay network adds significant overhead to the cold startup time for both OpenWhisk and \sys.
\sys's pre-warming mechanism and asynchronous control plane reduces the cold start time by 76\% and is on par with AWS. 
%AWS in general has better cold start performance than OpenWhisk-based systems including \sys\ because of its lightweight virtualization mechanism~\cite{Firecracker}. %Optimizing virtualization for serverless computing has been well studied and is out of scope for this paper.
\sys's warm startup time is only 10\ms, with an improvement of more than 90\% over AWS and 71\% over OpenWhisk, because \sys\ moves scheduling operations off the performance critical path.
\fi

\if 0
\boldunderpara{component chaining and fan-out.}
With disaggregation, component graphs could contain many components, with long chains of components and/or many components running in parallel (\ie, high fan-out). To demonstrate \sys' performance with chains and its almost just-in-time warm up, we use a microbenchmark of a sequence of components, each {\em sleep}s for 10\ms, 100\ms, or 1 second, and the chain lengths are 2 and 8. These lengths are representative of today's serverless workloads~\cite{shahrad2020serverless}.
Figure~\ref{fig-chain} plots the overhead of running this micro-benchmark on \sys, OpenWhisk Composer~\cite{OpenWhisk-composer}, and AWS Step Functions~\cite{AWS-Step-Functions}.
When running on OpenWhisk and AWS, each node is a function.
To measure the per-component overhead, we capture the end-to-end latency, deduct the execution (sleep) time from that, and calculate the average.
Thus, the overhead includes both scheduling and container preparation time.
Overall, \sys's overhead is much lower than OpenWhisk and AWS for both chain lengths.
The benefit comes from our almost just-in-time design, which hides the scheduling overhead.
The remaining overhead of \sys\ comes from Kafka, a tradeoff for faster failure recovery.
%In this experiment shown in figure \ref{fig-exp1} we demonstrate the \sys scheduler's just-in-time scheduling ability to reduce overhead coordinating multiple objects together which execute in a direct sequence. To carry out this experiment, we launched sequences of functions which were lengths of 2 and 8. Each function in the sequence was designed to run for an equal amount of time (10, 100, 1000ms) to represent realistic serverless function runtimes as in ~\cite{shahrad2020serverless}. The results show that regardless of the length of the sequence, \sys has approximately the same overhead induced per-object in the sequence which is lower than the overhead of both OpenWhisk and AWS Step Functions regardless of sequence length.

%\boldunderpara{Cold Starts}

When components are in sequences or in parallel within a DAG, there is an opportunity to reduce cold start times because when a DAG is processing, the next component is known ahead of time. \sys takes advantage of this by pre-warming components ahead-of-time in order to improve performance. To measure this we used sequences of components of length 2 and 10, with execution times between 100 and 10,000 ms to show the effect of \sys's cold-start prewarming capabilities. For DAGs that have longer chains of components, \sys is able to reduce the cold start overhead of the DAG by more than 50\% as shown in Figure~\ref{fig-exp9}


\boldunderpara{Locality-aware scheduling.}
\sys's locality-aware scheduling aims to put communicating components as close to each other as possible. % before resorting to aggregation.
Figure~\ref{fig-micro-locality} demonstrates the effect of our scheduling and puts it in perspective with running OpenWhisk and Redis on our local cluster and running on AWS Lambda with S3. 
We also evaluate \sys\ without using the locality-aware scheduling (\sys{}\_nolocal). %For this setting, we assign all memory component to a single executor. 
The workload launches 1 to 50 compute-memory-component pairs.
%The first effect of the locality-aware scheduling is on the communication throughput.
Since \sys\ always tries to put communicating components on the same server, its aggregated communication throughput is much higher and the average latency is lower than all other schemes.
\sys also scales better than Redis and \sys{}\_nolocal by utilizing local network bandwidth.
% Since we only have one rack, we cannot evaluate the effect of rack-level locality, but we believe the trend to be the same.
% We believe the trend to be the same at rack level.
As expected, S3's performance is the worst (almost invisible in the figure).
%The second effect is on the communication latency. With locality, the average latency is much lower.
\fi

%\input{fig-exp-extra-merged}

%\zhiyuan{In this experiment we launch multiple compute-memory object pairs and test the system under stress. While our RDMA based communication system already provide low latency and high er throughput, Our locality based scheduling system will always trys to put memory and compute on the same rack. which enables them to fully utilize the rack-local bandwidth in communication, result in higher accumulated bandwidth. This locality policy also ensures we do not have performance downgrade in larger racks.}

% We include scheduler scalability results in the \textbf{Appendix}.


%\boldunderpara{Scheduler performance and scalability.}

\if 0

\subsubsection{Component Communication}

Figure~\ref{fig-launch} shows the impact of \sys's communication techniques on a workload with one compute component accessing one data component in warm started environments with no established connections. The first bar represents OpenWhisk without an overlay network, while the second bar adds the overlay network to enable direct component-to-component communication. The third bar replaces the TCP stack in the second bar with \sys's RDMA stack, improving component execution time. The fourth bar removes the overlay network and uses \sys's network virtualization module, reducing initialization time. Finally, the fifth bar includes \sys's asynchronous messaging optimization, hiding network connection setup time.

\fi


%\subsubsection{Component Adjustment}
%\label{subsubsec:component_adjustment}

\if 0
\boldunderpara{Per-input component adjustment.}
% As discussed in \S\ref{sec-policy-component}, \sys\ automatically adjust the resource plans for each component based on history usage patterns.
% We evaluate the effect of our dynamic adjustment of the initial and incremental memory sizes of components (\S\ref{sec:memorycomponent}) using real-world serverless application memory usage profiles from Azure~\cite{shahrad2020serverless}.
We evaluate the effect of our dynamic adjustment of the initial and incremental data component sizes (\S\ref{sec-policy-component}) using real-world serverless application memory usage profiles from Azure~\cite{shahrad2020serverless}.
This dataset contains a set of real-world applications, each being invoked many times with different user inputs.
In addition to the average of all the dataset, we choose a few representative applications to highlight.
% Figure~\ref{fig-micro-adjust-data} plots the CDF of memory usage across invocations of these representative applications and the average memory usage of all applications in the trace.
%The representative applications are 
\textit{Small}: most invocations' memory usages are small, \textit{Large}: most invocations used a lot of memory, and \textit{Varying}: different invocations' memory usages vary largely.
\textbf{Appendix} shows their invocation distributions. It also contains results on performance of applications not split (Figures~\ref{fig-micro-time} and~\ref{fig-micro-resource}).

Figure~\ref{fig-micro-adjust} plots the performance and memory utilization with three schemes: fixing initial and incremental sizes to 256\MB\ and 64\MB, provision data components to the highest usage (peak-provision), and our dynamic adjustment policy. 
Overall, our dynamic policy achieves high utilization and good performance.
Peak provisioning achieves the best performance, since no auto-scaling or swapping is needed, but with low memory utilization. 
%\zhiyuan{A fixed configuration only works well when an application's usage pattern happens to be close to the configuration. actually this cannot process variance data. Maybe just remove this} 
A fixed configuration can lead to both poor resource utilization %(when real usage is below the configuration) 
and poor performance. % (when frequently adding many physical memory components). % at runtime).
%\zhiyuan{
%In figure \ref{fig-micro-adjust}, We evaluated our resource adjustment policy for single element using memory utilization traces collected from Azure Functions \cite{shahrad2020serverless}.
%We launch single computation element, and use Scad's runtime to scale its memory resources.
%We test our default policy, and our adjustment policy together with peak-provisioned resource allocation policy used in current serverless computing. We use average memory distribution from the dataset, together with 4 application with different distribution to set the policy.
%Our dynamic adjustment policy can successfully balanced the resource utilization and performance overhead introduced by disaggregation.
%}
\fi





==> runtime.tex <==
\section{\sys\ Runtime System}
\label{sec:online}

This section discusses how the \sys\ runtime system schedules and executes an application's invocation by adaptively materializing its resource graph based on the cluster resource availability using pre-compiled binaries. 
%\boldunderpara{Online system architecture.}
Figure~\ref{fig-arch} illustrates the overall architecture of \sys's runtime system.
Each rack has a {\em rack-level scheduler} for scheduling tasks within a rack, and the entire cluster has one global scheduler for assigning coarse-grained tasks to rack-level schedulers.
Each server has a {\em memory controller} for data component allocation and management, a {\em compute controller} for compute component execution,
%Controllers are responsible for creating, monitoring, and terminating their respective components. Additionally, each server has 
and a {\em network virtualization controller} for component communication orchestration. These three controllers sit in a user-space {\em executor} that interacts with the scheduler and other executors. 
A {\em \sys\ runtime} is inserted within the application execution sandbox (Docker container in our implementation) to handle \sys\ internal APIs and monitoring tasks.
%for communication, manage a local memory buffer, and monitor resources and performance.
%This section discusses these components and how \sys\ adaptively materializes and executes applications. 

%\input{fig-runtime}


%Once a component is scheduled, the \sys execution system is responsible for executing it in an efficient manner and for facilitating its communication with other components. 
%Below, we discuss how Scad executes its memory components and compute components and how it handles component communication and component triggering.

\input{schedule}
\input{scaling}
\input{network}
%\input{policy}
\input{failure}




==> scaling.tex <==
\subsection{Component Execution and Auto-Scaling}
\label{sec:execution}

We now discuss how \sys\ adaptively executes and scales data and compute components. 

\zhiyuan{At runtime, we treat them separately. They are managed by different components}

\subsubsection{Data Component Accessing and Autoscaling}
\label{sec:memorycomponent}

\sys\ automatically starts a data component when the first compute component accessing it in the resource graph starts. \noteyiying{when this compute component starts or when it first allocates memory?} The memory controller at the server chosen by the scheduler allocates a memory space with the size indicated in the resource graph. The data component ends when the last compute component accessing it ends or explicitly releases it. 

\zhiyuan{Adaptive execution? }

%\notezhiyuan{shared memory components are allocated in a shared memory pool} \noteyiying{think that's already implied in the current writing}
When a data component co-locates with a compute component accessing it on one server, the memory controller allocates a virtual memory space for the data component and mmaps it to the compute-component container.
When a data component is not co-located, the memory controller manages it as a virtual memory space in a reserved \sys\ process for a TCP cluster or an RDMA memory region for an RDMA cluster.
\noteyiying{how do we isolate different data components (local case and remote case)? need to talk about security and isolation here}

\notezhiyuan{should mention physical here}
As noted, a data component can grow beyond its initially allocated size. In this case, the \sys\ memory controller on the server picked by the scheduler allocates an additional memory space.
%we dynamically add more memory spaces to automatically scale up the data component. Specifically, the \sys\ memory controller first tries to allocate more memory space on the same server where the data component currently lives. If there is no more space there, the memory controller asks the rack-level scheduler to find a proper server to allocate the new memory space. 
When a compute component is currently accessing a data component natively, \sys\ mmaps the additional memory space on the same node or performs swapping if the additional memory space is on a different node (T3 in Figure~\ref{fig-materialize}).
When a compute component is currently accessing the data component via \sys\ APIs, the \sys\ library will transparently issue network requests to multiple servers for accesses spanning separated memory spaces.
%On the other hand, if a data component uses less memory than its initial allocation, we update the resource graph with the new size for future invocations.
%\zhiyuan{We do not do this simple update. need to bring back the selection feature.}

\if 0
We now explain how we implement a virtual memory component with dynamically added physical memory components.
%Memory components contain data and need to be elastic (both within an invocation and across invocations), as motivated in \S\ref{sec:background}.
%To execute a virtual memory component in a resource-efficient and performance-efficient way, we need to materialize it. We also need to proper isolation between memory components. 
%We design the execution of memory components to have proper isolation, runtime autoscaling, flexible scheduling, and fast startup. 
%Different from traditional disaggregated/remote memory systems, a unique need and challenge in the serverless setting is to quickly react to application resource changes by automatically and transparently adjusting the size of a memory component.
%We confront this challenge by materializing a virtual memory component with dynamically added physical components.

%\boldunderpara{Materialization and auto-scaling (cost, no resource limit).}
%Different from traditional disaggregated/remote memory systems, 
A unique need and challenge in the serverless setting is to quickly react to application resource changes by automatically and transparently adjusting the size of a memory component, while ensuring high resource utilization (\ie, minimal memory stranding).
To solve this, our main idea is to materialize each virtual memory component with dynamically added physical components and to use physical memory components as the unit of scheduling and execution environment.
%One virtual memory component can consist of multiple physical memory components potentially on different nodes.
Instead of making physical components all of the same size or of arbitrary sizes,
we choose from a small number of configurable sizes for each physical component based on an application's resource graph.
For example, a 2\GB\ virtual memory component can be internally represented as two 1\GB\ physical components or one 1\GB\ and eight 128\MB\ ones.
%\noteyiying{Zhiyuan, can you use some more realistic numbers for this example?}
This gives \sys flexibility to balance performance and memory utilization.
Currently, 64\MB\ and 1\GB\ are the smallest and largest physical memory component sizes in our evaluation, which means \sys\ can have at most 1\GB\ of stranded memory on any server and at most 64\MB\ for internal fragmentation. These numbers can be configured by system administrators.

%\boldunderpara{Auto-scale memory components.}
To support large, dynamic memory space needs without the upfront commitment of peak memory usage (\S\ref{sec:background}), \sys\ automatically scales up a virtual memory component in an on-demand fashion. When starting a virtual memory component, \sys\ first allocates and starts a physical memory component with {\em an initial size}, \eg, 1\GB.
As the application allocates more heap memory, %\noteryan{It's unclear if this is all dynamic heap allocation, or their is also a swap system reading from binary or cold storage}, 
\sys\ launches more physical components one at a time in an {\em on-demand} fashion. Each of these physical components is of the same size (what we call {\em the incremental size}, \eg, 128\MB).
\sys\ dynamically determines these sizes based on historical memory usage pattern (\S\ref{sec-policy-component}) and round them up to one of the small number of sizes we support.

%\boldunderpara{Execution environment (performance and safety).}
Different from traditional serverless functions, memory components only contain data and no computation. Their ``execution'' just need memory spaces on a server.
Thus, we do not use any virtualization environment or containers for them.
However, the memory spaces for different memory components should still be properly isolated to prevent one user access other's data. 
We rely on either a trusted party (the memory controller or the RDMA hardware) to allocate and manage physical memory component spaces. For example, for RDMA, we assign each physical memory component its own protection domain (PD).
%\textbf{Appendix} discussed the details of these isolation mechanisms.
\fi

\subsubsection{Compute Component Execution and Autoscaling}
\label{sec:computecomponent}

We execute compute components in containers (Docker in our current implementation) by initially sizing them according to profiling results. 
In the native access mode, compute components run directly on Docker. \sys\ only assists in mmap local data components and in forwarding the compute-component execution output to the rack-level scheduler. 
In the non-native mode, the \sys\ runtime executes access APIs as local memory copies (for local data components) or network requests (for remote data components). \sys\ waits for the reply from the rack-level scheduler before starting the subsequent compute components.

We set no limit to how much memory or CPU a compute component can use and thus need mechanisms to auto-scale compute components beyond the profiled configurations.
\sys\ detects when a compute component is under memory pressure and asks the rack-level scheduler to allocate additional memory space. The scheduler may schedule the additional space on the same or different server.
\sys\ performs local or remote memory swapping accordingly. \noteyiying{is this true for local?}
%The \textbf{Appendix} presents the details of our \ufd-based swap system. 
%\zhiyuan{this two seems to be the same for me?}
%We implemented our swap system in user space using Linux's \ufd.
%It swaps to a remote space that internally maps to one or more physical memory components.
%These physical components are scheduled and executed in the same way as physical memory components for regular virtual memory components.
%The same swapping method applies to a mixed component if its run-time memory consumption exceeds the allocated amount.
%Our resource adjustment policy (\S\ref{sec-policy-component}) ensures components' initial value is correct and swapping would not affect the performance.

\boldunderpara{Scaling CPU resources.} 
We scale CPU resources up and down by changing a container's vCPU. \sys\ periodically measures CPU utilization. If the utilization is 100\%, we increase vCPU by 1. The final usage will be logged and the initial number of vCPUs is decided by history, as described in Section~\ref{sec:offline}.

Note that we follow the application-specified level of parallelism defined with \xsplit$(par=K)$ (\eg, $K$ parallel threads each processing $1/K$ shard of data), as the level of parallelism is highly dependent on users' expectation of performance and cost tradeoff, and it is hard to automatically shard data for parallel execution without programmer hints.





==> schedule.tex <==
\subsection{Component Scheduling}
\label{sec:scheduling}

\zhiyuan{Start with runtime instead of scheudling? reorg this into adaptive materialization + Proactive scheduling}


We now discuss \sys's scheduling mechanism and policy.
%When a user-specified triggering event happens, our two-level scheduler is invoked with the triggered application's resource graph. The scheduler decides when and where to execute each physical component.
%We now present \sys's scheduler design.
 %It highlights the mechanism and efficiency of the \sys\ scheduling system.
%\notezhiyuan{need to mention figure 7 in detialed places? e.g. scheudling, communication setup}

\input{fig-materialization}

\subsubsection{Scheduling Mechanism}
\label{sec:schedulemechanism}
%\boldunderpara{Two-level scheduler architecture (scalability).}~~ 
%A bulky application can be complex and have many components in its resource graph. Moreover, with our auto-scaling support, one component can be materialized as multiple physical units (\S\ref{sec:schedulepolicy}). 
%We propose a two-level scheduler to achieve the scalability needed for bulky applications.
Our scheduling mechanisms aim to achieve scalability for launching components in a bulky application's resource graph while minimizing launching performance overhead.

For scalability, we propose a two-level scheduler architecture where a cluster has one {\em global scheduler}, and each rack within has a {\em rack-level scheduler}.
When a user event triggers an application, the request is sent to the global scheduler (possibly after a data-center load balancer directs requests across multiple clusters). The global scheduler maintains the rough amount of available resources in each rack. It uses this information to direct the application request to a rack by balancing loads across racks. It then looks up the application's compilations in the compilation database and sends the compilation and corresponding resource graph to the rack-level scheduler. 

The rack-level scheduler handles allocation requests for each component in a resource graph. It chooses a server to initially run the application based on policies in \S\ref{sec:schedulepolicy}. Upon completing a compute component, its result is sent to the rack-level scheduler via reliable messages (\S\ref{sec:failure}). The release of a data component or the need to scale it up are also sent to the rack-level scheduler. The rack-level scheduler increases the server's available resources accordingly and decides where to schedule the subsequent component or the scaled-up part of a component. It then updates the resource counting of the destination server and notifies that server's executor to start the component. Thus, the rack-level scheduler always has an accurate view of available resources in all the servers in the rack and what components currently run on each of them.
%maintains the available resources per server and what components currently run on each server. 
If a rack runs out of resources for a request, the rack-level scheduler sends the request back to the global scheduler to find another available rack.

To avoid applications being delayed by scheduling and container launching time, we pre-launch a subsequent component when the current component is running. With the help of resource graphs, our scheduler can set the proper size of the subsequent component before its execution. This {\em just-in-time} component launching mechanism utilizes application resource behavior history, adapts to the most up-to-date rack resource availability, and hides scheduling and start-up overhead behind foreground performance. Note that a recent work, Orion~\cite{Orion-osdi22}, also pre-warms functions in a FaaS DAG but does not incorporate resource patterns.
% To be resource efficient, we target to make a scheduling decision for each node just before it is triggered so as to utilize the most up-to-date cluster resource availability information . 
To further reduce start-up overhead, we pre-warm the first component in a resource graph based on historical invocation patterns, similar to previous works~\cite{roy_asplos22,shahrad2020serverless,singhvi2021atoll}.
Figure~\ref{fig-launch} plots a startup timeline with three dummy components, with latencies of different steps collected when running \sys.

\input{fig-launch}

\subsubsection{Scheduling Policy: Adaptive Materialization}
\label{sec:schedulepolicy}


Our scheduling policy aims to minimize network communication and execution environment startup time while being resource-efficient. When scheduling an application's invocation, the rack-level scheduler first tries to find servers that can fit the entire application in the hope that all components can run in one environment.
If there are such servers, the scheduler chooses the server with the smallest available resources among them to leave more spacious servers for future larger invocations (\eg, invocation 1 in Figure~\ref{fig-materialize}). The scheduler marks the chosen server's as having the potential need for more resources if its resource graph indicates so---no future resources are reserved, but the marked resources are given low priority when the scheduler allocates resources for other applications. The chosen server starts the application in a container whose size is set according to the {\em first} compute component's profiled resource needs. If this compute component accesses data components, the server also allocates the data components locally if possible. Afterward, if this server still has enough resources for the next components, the rack-level scheduler would still choose the same server. Its executor then continues the computation in the same container process but changes the container size to what the new components need. 
%\notezhiyuan{More on preserving. Basically we look ahead for whole memory usage (with a maxium step of n). each server have a preserved size. if this space is not take before scheduling next element, it will reduce the scheudle's job (just return the same machine). Or we will fall back to per-element scheduling}


If there is not enough resource to co-locate components, the rack-level scheduler will find a server with the smallest available resources to launch each of them. For instance, at invocation 2's T2, Server 1 runs out of resources, and \sys\ launches the blue component on Server 2. \sys\ then launches the compilation that issues \sys\ library APIs for data accesses, which our library executes as network requests (\S\ref{sec:communication}). If there is a need to scale up a component (\eg, in T3 of invocation 2, a memory allocation causes the data component's size to go beyond expected), the rack-level scheduler will first try to expand the data component on its current server. If that is not possible, the rack-level scheduler picks another server and prioritizes servers already running compute components that access the data component (\eg, Server 2).  
%co-locate compute components and their accessing data components as much as possible to avoid network communication. We also try to schedule a subsequent compute component in the  the triggering and the triggered compute components as much as possible, as the former avoids network communication and the latter avoids environment startup time.


Overall, our scheduling policy tries to co-locate compute components and their accessed data components, as doing so avoids remote data accesses. It also tries to co-locate triggered and triggering compute components to avoid environment startup overhead and output/input messaging overhead. Meanwhile, it sizes each component according to profiled history and adaptively scales it on demand.
%ensures locality whenever possible, avoids execution environment startup as much as possible, allocates resources to tightly fit different execution phases, and quckly scales up with on-demand load. 
Together with our component execution mechanism (\S\ref{sec:execution}), \sys\ achieves both resource efficiency and performance efficiency.

%To reduce the performance overhead of start-up containers and language runtimes for each function, there have been proposals to share these environments across functions.
Like \sys, some prior works also try to co-locate functions. \noteyiying{there should be some more papers on co-locating functions. fill more here}
A recent work, XFaaS~\cite{xFaaS}, proposes running multiple functions concurrently within one process and re-using runtime environments across invocations for serverless computing in the Meta private cloud. Differently, \sys\ does not co-run different applications, as our target environment is multi-tenant public clouds.
Moreover, unlike XFaaS, \sys\ is resource-centric instead of function-centric. 
%adjusts container sizes according to the needs of different components.

\if 0
Our policy takes the following steps when scheduling a physical component in an application:
1) For the {\em first} component in a resource graph, the rack-level scheduler chooses a server based on the hash of the application's and the component's unique ID to increase the probability of warm start, similar to OpenWhisk ({\em warm-start aware});
2) The rack-level scheduler schedules other {\em non-first} components in the same rack as previous components that trigger them unless this rack is out of resources, in which case another lightly loaded rack is chosen ({\em rack-level locality});
3) If a non-first component has other communicating component(s) that are already running, we schedule it on the same server as one of these other components if the server's resource permits to exploit {\em server-level locality}~\cite{zhang:shredder}. Otherwise, we fall back to warm-start aware and then to rack-level locality;
and 4) For compute components that fail the above steps and for all memory components, we choose a random server that has enough resources in the corresponding resource pool ({\em resource-pool aware}).
As will be seen in \S\ref{sec:memorycomponent}, memory components have no application-specific environments and can just be launched on arbitrary servers in the memory pool.
\fi


==> tab-intro.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{@{}l|ccc@{}}
\hline
Capability & \sys & Serverless & Reactive \\
\hline
\textbf{Auto Scaling} & & & \\
\quad Computation Scaling & yes & partial & partial \\
\quad Memory Scaling & yes & no & partial \\
\textbf{Resource Flexibility} & high & low & mid \\
\textbf{Performance} & high & low & mid \\
\hline
\end{tabular}
\mycaption{tab-intro}{System Comparison.}
{
}
\end{table}

==> tbl-system-comparison.tex <==
{
\begin{table}[h!]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|p{1.7cm}|p{1cm}|p{1.6cm}|p{1.2cm}|p{2cm}|}
\hline
\textbf{System} & \textbf{Memory Interface} & \textbf{Data Autoscale \& Mgmt} & \textbf{Compute Autoscale} & \textbf{Goals} \\ 
\hline
\textbf{Disagg Memory~\cite{Shan18-OSDI,AIFM,FastSwap}} & Y & N & N & resource saving \& larger memory \\
\hline
\textbf{Stateful Serverless~\cite{klimovic2018pocket,sreekanti2020cloudburst}} & N & Y & N & fast intermediate data access \\
\hline
\textbf{Scad} & Y & Y & Y & resource efficiency and performance \\
\hline
\end{tabular}
\vspace{-0.05in}
\mycaption{tbl-related}{Related Works Comparison.}
{
}
\end{table}
}

==> tbl-techniques-single-col.tex <==
{
\begin{table}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l | l | l |l |l}
\textbf{Technique}                              & \textbf{Sys.}             & \textbf{Purpose}                                                   & \textbf{Section}           & \textbf{Fig(s)}    \\
\hline
Mem. component auto-scaling    & C, S & Support memory elasticity                             & \S\ref{sec:memorycomponent}         &  \ref{fig-micro-elastic} \\
Native mem. comp. environment & C            & Fast memory component start up                          & \S\ref{sec:memorycomponent}         &  \ref{fig-micro-launch} \\
Transparent local mem. cache                           & R               & Cache remote memory                                      & \S\ref{sec:computecomponent}         & \ref{fig-tpcds-overhead} \\
User-space memory swapping                           & R               & Compute component elasticity                                       & \S\ref{sec:computecomponent}         & \ref{fig-micro-swap}  \\
RDMA network                           & C, R   & Fast component-to-component comm.                     & \S\ref{sec:communication}         & \ref{fig-micro-locality} \\
Network virtualization                 & C, S            & Connection between components & \S\ref{sec:communication}         & \ref{fig-launch} \\
Asynch. component initialization                        & C, R   & Fast memory component start up                          & \S\ref{sec:communication}               & \ref{fig-launch}, \ref{fig-micro-launch} \\
Pre-scheduling      & C, S             & Improving warm startup time                      & \S\ref{sec:failure}         &  \ref{fig-launch}, \ref{fig-micro-warmstart} \\
Language support                       & R               & Efficient language constructs         & \S\ref{sec:program-model}         & \ref{fig-tpcds-overhead} \\
Locality-aware scheduling              & S             & Fast component graph execution                          & \S\ref{sec:scheduling}         & \ref{fig-micro-locality} \\
Pre-warming components in graph          & S             & Improving cold startup time                      & \S\ref{sec:coldstart}         & \ref{fig-launch} \\
Component aggregation                       & C, S & Reduce execution time                             & \S\ref{sec:aggregation} & \ref{fig-policy}
\end{tabular}
}
\end{center}
\vspace{-0.15in}
\mycaption{tbl-techniques-single-col}{Summary of Techniques.}
{
The second column explains at which sub-system the technique is implemented (C: Controller, R: Runtime, and S: Scheduler). The last column points to corresponding result figures.
}
\end{table}
}

==> tbl-techniques.tex <==
{
\begin{table*}\scriptsize
\begin{center}
\begin{tabular}{l | l | l |l |l}
\textbf{Technique}                              & \textbf{Component}             & \textbf{Purpose}                                                   & \textbf{Description}           & \textbf{Results}    \\
\hline
Transparently scale memory elements    & Controller, Scheduler & Support for memory elasticity                             & \S\ref{sec:memoryelement}         & Figure \ref{fig-micro-elastic} \\
Native environment for memory elements & Controller            & Fast start up of memory elements                          & \S\ref{sec:memoryelement}         & Figures \ref{fig-micro-launch} \\
Transparent local memory cache                           & Runtime               & Cache remote memory for fast local accesses                                      & \S\ref{sec:computeelement}         & Figure \ref{fig-tpcds-overhead} \\
User-space memory swapping                           & Runtime               & Support for compute element elasticity                                       & \S\ref{sec:computeelement}         & Figure \ref{fig-micro-swap}  \\
RDMA network                           & Runtime, Controller   & Fast element-to-element communication                     & \S\ref{sec:communication}         & Figures \ref{fig-micro-locality} \\
Network virtualization                 & Controller, Scheduler            & Messaging between elements to set up connection & \S\ref{sec:communication}         & Figure~\ref{fig-launch} \\
Asynchronous element initialization                        & Controller, Runtime   & Fast start up of memory elements                          & \S\ref{sec:communication}               & Figures \ref{fig-launch} and \ref{fig-micro-launch} \\
Pre-scheduling off perf critical path      & Controller, Scheduler             & Improving warm startup time                      & \S\ref{sec:failure}         & Figures \ref{fig-launch} and \ref{fig-micro-dependent} \\
Language support                       & Runtime               & Efficiently support high-level language constructs         & \S\ref{sec:language}         & Figures \ref{fig-tpcds-overhead} \\
Locality-aware scheduling              & Scheduler             & Fast execution of element graphs                          & \S\ref{sec:scheduling}         & Figure~\ref{fig-micro-locality} \\
Pre-warming elements in graph          & Scheduler             & Improving cold startup time                      & \S\ref{sec:coldstart}         & Figure~\ref{fig-launch} \\
Element aggregation and disaggregation                       & Scheduler, Controller & Opportunistic reduction of execution time                             & \S\ref{sec:aggregation} and \S\ref{sec:policy} & Figures \ref{fig-policy}
\end{tabular}
\end{center}
\vspace{-0.15in}
\mycaption{tbl-technique}{Summary of Techniques.}
{
The second column explains at which component is the technique implemented. 
}
\end{table*}
}
